The subarcsecond mid-infrared view of local active galactic nuclei: I. The N- and Q-band imaging atlas

We present the first subarcsecond-resolution mid-infrared (MIR) atlas of local active galactic nuclei (AGN). Our atlas contains 253 AGN with a median redshift of z=0.016, and includes all publicly available MIR imaging performed to date with ground-based 8-m class telescopes, a total of 895 independent measurements. Of these, more than 60% are published here for the first time. We detect extended nuclear emission in at least 21% of the objects, while another 19% appear clearly point-like, and the remaining objects cannot be constrained. Where present, elongated nuclear emission aligns with the ionization cones in Seyferts. Subarcsecond resolution allows us to isolate the AGN emission on scales of a few tens of parsecs and to obtain nuclear photometry in multiple filters for the objects. Median spectral energy distributions (SEDs) for the different optical AGN types are constructed and individual MIR 12 and 18micron continuum luminosities are computed. These range over more than six orders of magnitude. In comparison to the arcsecond-scale MIR emission as probed by Spitzer, the continuum emission is much lower on subarcsecond scales in many cases. The silicate feature strength is similar on both scales and generally appears in emission (absorption) in type I (II) AGN. However, the polycyclic aromatic hydrocarbon emission appears weaker or absent on subarcsecond scales. The differences of the MIR SEDs on both scales are particularly large for AGN/starburst composites and close-by (and weak) AGN. The nucleus dominates over the total emission of the galaxy only at luminosities >=10^(44)erg/s. The AGN MIR atlas is well suited not only for detailed investigation of individual sources but also for statistical studies of AGN unification.

==> tab_obs.tex <==
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & NEII\_1 & 12.27 &  0.18 &      360 &  0.38 &  0.35 &      126 &  0.36 &  0.35 &      171 &     63.2 $\pm$     5.3 &     64.9 $\pm$     3.6\\
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & NEII\_2 & 13.04 &  0.22 &      543 &  0.36 &  0.36 &      128 &  0.40 &  0.36 &       23 &     62.1 $\pm$    10.2 &     53.5 $\pm$     4.3\\
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.33 &      108 &  0.36 &  0.33 &       80 &     67.2 $\pm$    13.0 &     70.7 $\pm$     8.2\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-01-26 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.56 &  0.48 &       95 &  0.51 &  0.41 &        2 &     39.0 $\pm$    15.1 &     53.8 $\pm$     7.2\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-03-23 & NEII\_2 & 13.04 &  0.22 &     1991 &  0.40 &  0.37 &       66 &  0.58 &  0.51 &      166 &     41.1 $\pm$     2.6 &     20.6 $\pm$     2.0\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-01-26 & PAH2 & 11.25 &  0.59 &      362 &  0.42 &  0.39 &       12 &  0.47 &  0.34 &      157 &     36.4 $\pm$     8.9 &     35.6 $\pm$     8.8\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_1 & 12.27 &  0.18 &      540 &  0.43 &  0.40 &       10 &  0.77 &  0.58 &      119 &     26.5 $\pm$    11.2 &     10.0 $\pm$    11.2\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_2 & 13.04 &  0.22 &      901 &  0.41 &  0.40 &       16 &  0.71 &  0.60 &       85 &     33.6 $\pm$     7.6 &     13.0 $\pm$     7.6\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV\_2 & 10.77 &  0.19 &      362 &  0.37 &  0.34 &      171 &  0.69 &  0.33 &      120 &     23.8 $\pm$     7.7 &     13.0 $\pm$     7.7\\
2MASXJ0918002 & VISIR &  084.B-0606(A)  & 10-01-05 & PAH2\_2 & 11.88 &  0.37 &     1986 &  0.34 &  0.31 &       94 &  0.42 &  0.31 &       97 &     16.6 $\pm$     0.6 &     13.4 $\pm$     0.7\\
3C029 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    11.1   &  $\le$    11.1  \\
3C033 & COMICS &  o09108  & 09-07-14 & N11.7 & 11.74 &  0.53 &     3208 &  0.71 &  0.52 &       72 &  1.00 &  0.85 &      121 &     47.4 $\pm$     5.0 &     20.8 $\pm$     3.0\\
3C078 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.5   &  $\le$    10.5  \\
3C093 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.5   &  $\le$    12.5  \\
3C098 & VISIR &  076.B-0194(A)  & 05-12-18 & SIC & 11.85 &  2.34 &     1973 &  0.55 &  0.45 &       69 &  0.49 &  0.45 &       74 &     25.2 $\pm$     6.8 &     31.0 $\pm$     5.8\\
3C105 & VISIR &  084.B-0606(A)  & 09-10-06 & NEII\_1 & 12.27 &  0.18 &      901 &  0.35 &  0.34 &       69 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.4   &      8.4 $\pm$     0.0\\
3C105 & VISIR &  084.B-0606(A)  & 09-10-08 & NEII\_2 & 13.04 &  0.22 &     1442 &  0.37 &  0.37 &      106 &  $\dots$  &  $\dots$  &  $\dots$  &     13.4 $\pm$     0.9 &     13.3 $\pm$     0.9\\
3C105 & VISIR &  084.B-0606(A)  & 09-11-19 & NEII\_2 & 13.04 &  0.22 &     1442 &  0.37 &  0.34 &       93 &  $\dots$  &  $\dots$  &  $\dots$  &      7.0 $\pm$     0.8 &      7.0 $\pm$     0.8\\
3C105 & VISIR &  076.B-0194(A)  & 05-12-18 & SIC & 11.85 &  2.34 &     4843 &  0.44 &  0.39 &       77 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     5.7   &  $\le$     5.7  \\
3C105 & VISIR &  084.B-0606(A)  & 09-10-06 & SIV\_2 & 10.77 &  0.19 &      543 &  0.35 &  0.34 &      107 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.7   &  $\le$    13.7  \\
3C120 & VISIR &  084.B-0606(A)  & 09-10-04 & NEII & 12.81 &  0.21 &      179 &  0.41 &  0.40 &       98 &  0.43 &  0.42 &      155 &    269.9 $\pm$     8.3 &    245.3 $\pm$    12.4\\
3C120 & VISIR &  084.B-0366(E)  & 10-03-14 & PAH1 &  8.59 &  0.42 &      181 &  0.30 &  0.27 &      103 &  0.57 &  0.44 &      126 &    123.9 $\pm$     9.8 &     38.8 $\pm$     7.3\\
3C120 & VISIR &  084.B-0606(A)  & 09-10-04 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.41 &  0.39 &      117 &  0.51 &  0.41 &        5 &    254.8 $\pm$    13.1 &    195.2 $\pm$    11.8\\
3C120 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  0.40 &  0.38 &      107 &    266.8 $\pm$     9.5 &    247.1 $\pm$    16.4\\
3C120 & VISIR &  084.B-0606(A)  & 09-10-04 & SIV & 10.49 &  0.16 &      176 &  0.34 &  0.32 &      113 &  0.42 &  0.38 &      134 &    231.0 $\pm$    12.1 &    158.6 $\pm$    16.0\\
3C135 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.37 &  0.31 &      113 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.3   &  $\le$     8.3  \\
3C227 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.37 &  0.31 &      113 &  0.35 &  0.33 &      148 &     31.7 $\pm$     8.2 &     31.3 $\pm$     7.1\\
3C264 & COMICS &  o09108  & 09-05-05 & N11.7 & 11.74 &  0.53 &     1804 &  0.40 &  0.38 &      112 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     3.9   &  $\le$     3.9  \\
3C264 & COMICS &  o09108  & 09-07-14 & N11.7 & 11.74 &  0.53 &     3208 &  0.44 &  0.40 &      120 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     4.7   &  $\le$     4.7  \\
3C273 & VISIR &  078.B-0255(B)  & 07-03-02 & PAH1 &  8.59 &  0.42 &      360 &  0.40 &  0.37 &      124 &  0.48 &  0.41 &      124 &    253.7 $\pm$    15.4 &    187.8 $\pm$    17.6\\
3C273 & VISIR &  086.B-0257(J)  & 11-03-22 & PAH1 &  8.59 &  0.42 &      118 &  0.53 &  0.36 &      110 &  0.39 &  0.30 &      132 &    251.3 $\pm$    13.1 &    370.1 $\pm$    36.9\\
3C273 & VISIR &  086.B-0257(I)  & 11-03-23 & PAH1 &  8.59 &  0.42 &      118 &  0.43 &  0.38 &       68 &  0.40 &  0.37 &       75 &    246.8 $\pm$    17.6 &    273.4 $\pm$    35.8\\
3C273 & VISIR &  086.B-0257(J)  & 11-03-22 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.43 &  0.36 &      105 &  0.46 &  0.32 &      126 &    297.0 $\pm$    19.9 &    313.5 $\pm$    16.5\\
3C273 & VISIR &  086.B-0257(I)  & 11-03-23 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.38 &  0.35 &       58 &  0.38 &  0.36 &       39 &    311.7 $\pm$    28.1 &    299.4 $\pm$    18.8\\
3C273 & VISIR &  078.B-0255(B)  & 07-03-02 & SIC & 11.85 &  2.34 &      358 &  0.39 &  0.37 &      111 &  0.43 &  0.37 &      132 &    345.4 $\pm$    16.4 &    298.6 $\pm$    12.6\\
3C285 & COMICS &  o09108  & 09-05-05 & N11.7 & 11.74 &  0.53 &     3609 &  0.40 &  0.38 &      112 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     4.3   &  $\le$     4.3  \\
3C293 & COMICS &  o09108  & 09-05-05 & N11.7 & 11.74 &  0.53 &     3609 &  0.40 &  0.38 &      112 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     3.8   &  $\le$     3.8  \\
3C305 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &     2406 &  0.38 &  0.37 &       69 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     3.1   &  $\le$     3.1  \\
3C317 & VISIR &  077.B-0135(A)  & 06-06-19 & SIC & 11.85 &  2.34 &     3588 &  0.43 &  0.39 &       94 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.9   &  $\le$    12.9  \\
3C321 & COMICS &  o09108  & 09-05-05 & N11.7 & 11.74 &  0.53 &     2005 &  0.42 &  0.39 &       27 &  0.92 &  0.61 &       89 &     43.6 $\pm$     7.4 &     12.2 $\pm$     1.4\\
3C327 & VISIR &  075.B-0621(A)  & 05-07-02 & SIC & 11.85 &  2.34 &     1794 &  0.56 &  0.47 &      119 &  0.66 &  0.61 &       97 &     58.4 $\pm$     7.6 &     40.3 $\pm$     1.8\\
3C353 & VISIR &  075.B-0621(A)  & 05-07-02 & SIC & 11.85 &  2.34 &     1794 &  0.51 &  0.44 &       96 &  0.46 &  0.31 &      161 &      8.0 $\pm$     2.2 &     12.4 $\pm$     2.2\\
3C382 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &      802 &  0.51 &  0.49 &      103 &  0.42 &  0.39 &      150 &    112.9 $\pm$     6.1 &    161.2 $\pm$    38.3\\
3C390-3 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &      802 &  0.38 &  0.37 &      159 &  0.51 &  0.48 &       92 &    152.4 $\pm$     5.3 &     87.1 $\pm$    15.6\\
3C403 & VISIR &  077.B-0135(A)  & 06-06-19 & SIC & 11.85 &  2.34 &     3588 &  0.54 &  0.44 &      104 &  0.41 &  0.37 &       60 &     80.6 $\pm$     4.4 &     97.0 $\pm$    10.8\\
3C424 & VISIR &  077.B-0135(A)  & 06-06-19 & SIC & 11.85 &  2.34 &     1794 &  0.42 &  0.34 &      104 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     9.4   &  $\le$     9.4  \\
3C445 & VISIR &  077.B-0137(A)  & 06-07-10 & NEII & 12.81 &  0.21 &      179 &  0.35 &  0.33 &      102 &  0.39 &  0.37 &       99 &    180.0 $\pm$     7.2 &    146.3 $\pm$    11.4\\
3C445 & VISIR &  077.B-0137(A)  & 06-07-10 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.31 &      128 &  0.37 &  0.32 &      107 &    190.9 $\pm$    10.4 &    160.6 $\pm$    12.0\\
3C445 & TRECS &  GS-2010A-Q-10  & 10-06-06 & Si2 &  8.74 &  0.39 &      144 &  0.39 &  0.36 &      152 &  0.46 &  0.41 &       26 &    102.4 $\pm$     2.9 &     76.3 $\pm$     2.8\\
3C445 & VISIR &  075.B-0621(A)  & 05-07-02 & SIC & 11.85 &  2.34 &     2691 &  0.59 &  0.48 &      111 &  0.56 &  0.50 &       96 &    189.9 $\pm$     7.3 &    169.6 $\pm$     6.4\\
3C445 & VISIR &  077.B-0137(A)  & 06-07-10 & SIV & 10.49 &  0.16 &      176 &  0.32 &  0.29 &      115 &  0.39 &  0.30 &      109 &    159.4 $\pm$     8.1 &    125.7 $\pm$    11.6\\
3C449 & COMICS &  o09108  & 09-07-14 & N11.7 & 11.74 &  0.53 &     2005 &  0.71 &  0.52 &      161 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.6   &  $\le$    10.6  \\
3C452 & COMICS &  o09108  & 09-05-05 & N11.7 & 11.74 &  0.53 &     3208 &  0.66 &  0.54 &       78 &  0.80 &  0.63 &      141 &     33.3 $\pm$     6.4 &     22.0 $\pm$     2.0\\
3C459 & VISIR &  385.B-0981(A)  & 10-07-21 & SIC & 11.85 &  2.34 &     3588 &  0.54 &  0.49 &      138 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.9   &  $\le$     8.9  \\
4C+73-08 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &      971 &  0.36 &  0.34 &      159 &  0.52 &  0.35 &      169 &     18.5 $\pm$     7.2 &     12.1 $\pm$     7.2\\
Ark120 & VISIR &  084.B-0606(A)  & 09-10-04 & NEII & 12.81 &  0.21 &      179 &  0.41 &  0.40 &       98 &  0.37 &  0.34 &       51 &    252.7 $\pm$    16.3 &    333.1 $\pm$    19.3\\
Ark120 & VISIR &  084.B-0366(E)  & 10-03-14 & PAH1 &  8.59 &  0.42 &      181 &  0.30 &  0.27 &      103 &  0.34 &  0.28 &      108 &    146.3 $\pm$     2.6 &    120.7 $\pm$     3.3\\
Ark120 & VISIR &  084.B-0606(A)  & 09-10-04 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.41 &  0.39 &      117 &  0.40 &  0.37 &       12 &    253.2 $\pm$    16.0 &    275.4 $\pm$    14.5\\
Ark120 & VISIR &  084.B-0366(E)  & 10-03-14 & PAH2\_2 & 11.88 &  0.37 &      181 &  0.34 &  0.33 &       74 &  0.39 &  0.34 &      113 &    226.9 $\pm$    19.9 &    193.2 $\pm$    18.0\\
Ark120 & VISIR &  084.B-0606(A)  & 09-10-04 & SIV & 10.49 &  0.16 &      176 &  0.34 &  0.32 &      113 &  0.32 &  0.31 &       34 &    269.3 $\pm$     9.6 &    293.4 $\pm$    23.1\\
CenA & VISIR &  076.B-0621(A)  & 06-02-02 & NEII & 12.81 &  0.21 &     1081 &  0.47 &  0.42 &      104 &  0.45 &  0.42 &      146 &   1723.2 $\pm$    61.3 &   1819.3 $\pm$    85.5\\
CenA & VISIR &  075.B-0631(A)  & 05-03-21 & NEII & 12.81 &  0.21 &     3622 &  0.39 &  0.37 &      136 &  0.48 &  0.44 &       79 &   2081.5 $\pm$    74.7 &   1461.7 $\pm$    58.3\\
CenA & VISIR &  077.B-0137(A)  & 06-04-09 & NEII\_1 & 12.27 &  0.18 &      180 &  0.37 &  0.33 &       83 &  0.36 &  0.34 &        9 &   1490.3 $\pm$    33.0 &   1425.9 $\pm$    30.0\\
CenA & VISIR &  076.B-0621(A)  & 06-02-02 & NEII\_2 & 13.04 &  0.22 &     1086 &  0.45 &  0.41 &      143 &  0.42 &  0.40 &      123 &   1464.1 $\pm$    56.5 &   1627.7 $\pm$    89.0\\
CenA & VISIR &  085.B-0639(C)  & 10-07-12 & PAH1 &  8.59 &  0.42 &       62 &  0.41 &  0.38 &       56 &  0.44 &  0.37 &       50 &    921.6 $\pm$    36.7 &    895.9 $\pm$    54.7\\
CenA & VISIR &  077.B-0137(A)  & 06-04-09 & PAH2 & 11.25 &  0.59 &      181 &  0.35 &  0.32 &       88 &  0.40 &  0.37 &       10 &    986.4 $\pm$    32.9 &    726.4 $\pm$    43.0\\
CenA & VISIR &  076.B-0599(A)  & 06-03-15 & PAH2\_2 & 11.88 &  0.37 &      543 &  0.33 &  0.32 &       26 &  0.34 &  0.33 &       67 &   1099.4 $\pm$    25.7 &   1019.9 $\pm$    24.2\\
CenA & VISIR &  076.B-0599(A)  & 06-03-22 & Q2 & 18.72 &  0.88 &     1539 &  0.52 &  0.49 &       81 &  0.54 &  0.52 &       27 &   2694.9 $\pm$    75.5 &   2440.9 $\pm$    71.0\\
CenA & TRECS &  GS-2004A-Q-41  & 04-05-03 & Qa & 18.30 &  0.76 &     2063 &  0.54 &  0.52 &      122 &  0.60 &  0.56 &        9 &   2401.9 $\pm$    92.5 &   2022.8 $\pm$    98.5\\
CenA & TRECS &  GS-2004A-Q-41  & 04-05-03 & Si2 &  8.74 &  0.39 &     2432 &  0.42 &  0.37 &      124 &  0.43 &  0.41 &       57 &    639.2 $\pm$    24.9 &    562.3 $\pm$    54.3\\
CenA & TRECS &  GS-2004A-Q-41  & 04-05-02 & Si6 & 12.33 &  0.59 &      608 &  0.65 &  0.44 &      113 &  0.52 &  0.48 &       89 &   1524.2 $\pm$    30.9 &   1689.2 $\pm$    81.3\\
CenA & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.37 &  0.31 &      113 &  0.46 &  0.38 &       96 &   1231.5 $\pm$    24.0 &    815.0 $\pm$    87.6\\
CenA & VISIR &  077.B-0137(A)  & 06-04-09 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.29 &       94 &  0.34 &  0.33 &      157 &    635.7 $\pm$    22.1 &    521.3 $\pm$    59.1\\
CenA & VISIR &  085.B-0639(C)  & 10-07-12 & SIV\_2 & 10.77 &  0.19 &       62 &  0.41 &  0.39 &      167 &  0.49 &  0.41 &       54 &   1086.3 $\pm$    77.2 &    881.6 $\pm$    80.3\\
Circinus & VISIR &  078.B-0255(A)  & 06-09-14 & NEII & 12.81 &  0.21 &      538 &  0.38 &  0.34 &      119 &  0.57 &  0.47 &       80 &  15964.2 $\pm$   482.6 &   7596.9 $\pm$   454.6\\
Circinus & VISIR &  078.B-0255(A)  & 06-09-15 & NEII\_2 & 13.04 &  0.22 &      540 &  0.38 &  0.35 &      119 &  0.58 &  0.49 &       86 &  15925.1 $\pm$   485.4 &   7332.5 $\pm$   307.6\\
Circinus & TRECS &  GS-2004A-C-2  & 04-05-06 & N & 10.36 &  2.64 &       32 &  $\dots$  &  $\dots$  &  $\dots$  &  0.56 &  0.49 &       34 &   8189.7 $\pm$  1429.9 &  $\le$ 12479.2  \\
Circinus & VISIR &  385.B-0896(A)  & 10-05-08 & PAH1 &  8.59 &  0.42 &      117 &  0.32 &  0.30 &       48 &  0.44 &  0.38 &      139 &   8349.8 $\pm$   371.8 &   4485.9 $\pm$   344.1\\
Circinus & VISIR &  385.B-0896(A)  & 10-08-17 & PAH1 &  8.59 &  0.42 &      117 &  0.30 &  0.26 &      110 &  0.37 &  0.32 &       46 &   6879.6 $\pm$   121.2 &   4578.2 $\pm$   188.5\\
Circinus & VISIR &  386.B-0026(A)  & 10-12-27 & PAH1 &  8.59 &  0.42 &      117 &  0.31 &  0.24 &       75 &  0.35 &  0.31 &      106 &   5843.5 $\pm$   133.8 &   3927.8 $\pm$   193.7\\
Circinus & VISIR &  386.B-0026(A)  & 10-12-29 & PAH1 &  8.59 &  0.42 &      117 &  0.28 &  0.27 &      110 &  0.35 &  0.31 &      117 &   7006.3 $\pm$   277.1 &   5009.1 $\pm$   469.4\\
Circinus & VISIR &  386.B-0026(A)  & 11-02-24 & PAH1 &  8.59 &  0.42 &      118 &  0.42 &  0.39 &       14 &  0.48 &  0.39 &      140 &   7623.4 $\pm$   431.2 &   6307.3 $\pm$  1161.8\\
Circinus & VISIR &  087.B-0746(A)  & 11-04-20 & PAH1 &  8.59 &  0.42 &      148 &  0.26 &  0.25 &      133 &  0.36 &  0.30 &       81 &   6694.3 $\pm$   158.8 &   4017.9 $\pm$   193.1\\
Circinus & VISIR &  087.B-0746(A)  & 11-06-15 & PAH1 &  8.59 &  0.42 &      148 &  0.29 &  0.29 &      149 &  0.35 &  0.32 &       32 &   6779.0 $\pm$   254.9 &   4961.6 $\pm$   403.3\\
Circinus & VISIR &  076.B-0599(A)  & 06-03-15 & PAH2\_2 & 11.88 &  0.37 &      543 &  0.33 &  0.32 &       26 &  0.36 &  0.36 &       97 &   9628.4 $\pm$   227.0 &   7768.4 $\pm$   190.8\\
Circinus & VISIR &  385.B-0896(A)  & 10-05-08 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.34 &  0.34 &      144 &  0.43 &  0.39 &      141 &  13655.8 $\pm$   601.4 &   9312.6 $\pm$   681.8\\
Circinus & VISIR &  385.B-0896(A)  & 10-08-17 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.33 &  0.32 &      116 &  0.38 &  0.35 &       38 &  12285.1 $\pm$   221.3 &   9916.7 $\pm$   766.0\\
Circinus & VISIR &  386.B-0026(A)  & 10-12-27 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.34 &  0.31 &       80 &  0.43 &  0.37 &       94 &  11605.1 $\pm$   237.2 &   7706.8 $\pm$   238.6\\
Circinus & VISIR &  386.B-0026(A)  & 10-12-29 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.34 &  0.33 &       93 &  0.41 &  0.35 &      104 &  11653.6 $\pm$   384.7 &   9210.7 $\pm$   722.9\\
Circinus & VISIR &  386.B-0026(A)  & 11-02-24 & PAH2\_2 & 11.88 &  0.37 &      118 &  0.50 &  0.44 &      169 &  0.53 &  0.47 &      134 &  13170.9 $\pm$   787.0 &  11059.9 $\pm$  1273.5\\
Circinus & VISIR &  087.B-0746(A)  & 11-04-20 & PAH2\_2 & 11.88 &  0.37 &      149 &  0.32 &  0.30 &        6 &  0.41 &  0.36 &       83 &  12492.9 $\pm$   224.5 &   8209.9 $\pm$   261.2\\
Circinus & VISIR &  087.B-0746(A)  & 11-06-15 & PAH2\_2 & 11.88 &  0.37 &      149 &  0.36 &  0.32 &      159 &  0.40 &  0.36 &       24 &  12425.0 $\pm$   480.6 &  10169.5 $\pm$   305.5\\
Circinus & VISIR &  382.B-0732(A)  & 08-08-09 & Q1 & 17.65 &  0.83 &      342 &  0.52 &  0.48 &      110 &  0.58 &  0.54 &       72 &  21409.9 $\pm$   348.8 &  18626.0 $\pm$  2649.0\\
Circinus & VISIR &  076.B-0599(A)  & 06-03-17 & Q2 & 18.72 &  0.88 &      993 &  0.49 &  0.47 &       96 &  0.53 &  0.52 &       74 &  18630.8 $\pm$   330.3 &  15365.6 $\pm$   292.9\\
Circinus & VISIR &  076.B-0599(A)  & 06-03-27 & Q2 & 18.72 &  0.88 &     1026 &  $\dots$  &  $\dots$  &  $\dots$  &  0.55 &  0.53 &      105 &  13642.5 $\pm$  5902.3 &  $\le$ 31349.5  \\
Circinus & VISIR &  382.B-0732(A)  & 08-08-10 & Q3 & 19.50 &  0.40 &      174 &  0.58 &  0.52 &      111 &  0.73 &  0.59 &       46 &  25364.6 $\pm$   817.2 &  18670.3 $\pm$  2361.5\\
Circinus & TRECS &  GS-2003B-DD-4  & 04-02-01 & Qa & 18.30 &  0.76 &      108 &  0.68 &  0.62 &      127 &  0.69 &  0.63 &      134 &  14039.0 $\pm$   219.0 &  13472.6 $\pm$   215.7\\
Circinus & TRECS &  GS-2003B-DD-4  & 04-02-01 & Si2 &  8.74 &  0.39 &      564 &  0.57 &  0.53 &      124 &  0.42 &  0.37 &      124 &   6421.0 $\pm$    70.1 &  12275.6 $\pm$  1285.3\\
Circinus & VISIR &  078.B-0255(A)  & 06-09-13 & SIV & 10.49 &  0.16 &      717 &  0.34 &  0.31 &      122 &  0.42 &  0.35 &       87 &   4497.7 $\pm$    72.9 &   3250.4 $\pm$   167.8\\
Circinus & VISIR &  078.B-0255(A)  & 06-09-13 & SIV\_2 & 10.77 &  0.19 &      722 &  0.36 &  0.32 &      140 &  0.48 &  0.39 &       78 &   5920.3 $\pm$   160.3 &   3606.7 $\pm$   119.1\\
CygnusA & COMICS &  o05107  & 05-04-28 & N11.7 & 11.74 &  0.53 &       49 &  0.56 &  0.51 &      110 &  0.81 &  0.62 &       94 &     80.6 $\pm$     7.5 &     48.0 $\pm$    11.8\\
ESO005-G004 & VISIR &  080.B-0860(A)  & 07-10-09 & NEII\_2 & 13.04 &  0.22 &      181 &  0.72 &  0.57 &       84 &  1.00 &  0.51 &       99 &    111.8 $\pm$    16.6 &     90.7 $\pm$    16.6\\
ESO005-G004 & VISIR &  080.B-0860(A)  & 07-10-09 & PAH1 &  8.59 &  0.42 &      181 &  0.88 &  0.70 &       73 &  0.67 &  0.39 &       99 &     14.1 $\pm$     8.2 &     32.9 $\pm$     8.2\\
ESO005-G004 & VISIR &  086.B-0349(C)  & 10-11-13 & PAH1 &  8.59 &  0.42 &      181 &  0.32 &  0.30 &       54 &  1.00 &  0.49 &       36 &     19.4 $\pm$     3.8 &      3.7 $\pm$     3.8\\
ESO005-G004 & VISIR &  086.B-0349(C)  & 10-11-22 & PAH2 & 11.25 &  0.59 &     1993 &  0.54 &  0.44 &       46 &  0.50 &  0.47 &       83 &     21.8 $\pm$     0.8 &     18.5 $\pm$     1.3\\
ESO005-G004 & VISIR &  086.B-0349(C)  & 10-11-22 & PAH2\_2 & 11.88 &  0.37 &     1986 &  0.49 &  0.40 &       57 &  0.52 &  0.47 &       95 &     28.8 $\pm$     1.9 &     22.3 $\pm$     3.0\\
ESO005-G004 & VISIR &  086.B-0349(D)  & 10-11-16 & Q2 & 18.72 &  0.88 &      496 &  0.59 &  0.51 &       76 &  0.49 &  0.43 &       69 &     68.6 $\pm$    24.9 &     97.5 $\pm$    24.9\\
ESO005-G004 & VISIR &  080.B-0860(A)  & 07-10-09 & SIV & 10.49 &  0.16 &      356 &  0.76 &  0.60 &       74 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    96.4   &  $\le$    96.4  \\
ESO005-G004 & VISIR &  086.B-0349(C)  & 10-11-08 & SIV\_2 & 10.77 &  0.19 &      362 &  0.46 &  0.39 &       32 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    36.7   &  $\le$    36.7  \\
ESO005-G004 & VISIR &  086.B-0349(C)  & 10-11-13 & SIV\_2 & 10.77 &  0.19 &      541 &  0.37 &  0.34 &      147 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    27.1   &  $\le$    27.1  \\
ESO033-G002 & TRECS &  GS-2004A-Q-14  & 04-10-24 & N & 10.36 &  2.64 &      716 &  0.72 &  0.62 &      176 &  0.89 &  0.79 &      133 &    168.9 $\pm$     3.3 &    104.9 $\pm$     3.0\\
ESO103-G035 & VISIR &  080.B-0860(A)  & 08-03-22 & NEII\_2 & 13.04 &  0.22 &       62 &  0.36 &  0.36 &       61 &  0.65 &  0.45 &       95 &    669.4 $\pm$    57.2 &    299.3 $\pm$    80.3\\
ESO103-G035 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH1 &  8.59 &  0.42 &       62 &  0.29 &  0.26 &      153 &  0.55 &  0.40 &      125 &    257.5 $\pm$    24.2 &     95.9 $\pm$    15.8\\
ESO103-G035 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH2 & 11.25 &  0.59 &       62 &  0.36 &  0.35 &       57 &  0.63 &  0.43 &      107 &    404.7 $\pm$    18.6 &    191.4 $\pm$    58.5\\
ESO103-G035 & VISIR &  080.B-0860(A)  & 08-03-22 & SIV & 10.49 &  0.16 &       62 &  0.31 &  0.30 &      132 &  0.75 &  0.45 &      101 &    300.0 $\pm$    21.2 &     84.5 $\pm$    14.5\\
ESO121-G028 & VISIR &  084.B-0606(A)  & 09-10-04 & NEII & 12.81 &  0.21 &      717 &  0.41 &  0.40 &       98 &  0.36 &  0.30 &       19 &     13.7 $\pm$     4.4 &     20.7 $\pm$     4.4\\
ESO121-G028 & VISIR &  084.B-0606(A)  & 09-10-04 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.41 &  0.39 &      117 &  0.39 &  0.34 &       32 &     10.6 $\pm$     3.2 &     13.0 $\pm$     3.2\\
ESO121-G028 & VISIR &  084.B-0606(A)  & 09-10-04 & SIV & 10.49 &  0.16 &      353 &  0.34 &  0.32 &      113 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     9.6   &  $\le$     9.6  \\
ESO138-G001 & VISIR &  085.B-0251(C)  & 10-07-16 & ARIII &  8.99 &  0.14 &      135 &  0.40 &  0.37 &       29 &  0.46 &  0.39 &      152 &    447.5 $\pm$    20.7 &    379.8 $\pm$    34.8\\
ESO138-G001 & VISIR &  080.B-0860(A)  & 08-03-14 & NEII\_2 & 13.04 &  0.22 &      543 &  0.36 &  0.34 &       99 &  0.40 &  0.37 &      127 &    809.8 $\pm$    18.2 &    655.2 $\pm$    16.3\\
ESO138-G001 & VISIR &  080.B-0860(A)  & 08-03-14 & PAH1 &  8.59 &  0.42 &      543 &  0.32 &  0.26 &       88 &  0.32 &  0.29 &      108 &    416.6 $\pm$    15.1 &    361.8 $\pm$    21.1\\
ESO138-G001 & VISIR &  080.B-0860(A)  & 08-03-14 & PAH2 & 11.25 &  0.59 &      543 &  0.34 &  0.29 &       75 &  0.34 &  0.32 &      111 &    747.4 $\pm$    12.1 &    683.4 $\pm$    29.0\\
ESO138-G001 & VISIR &  085.B-0251(C)  & 10-07-16 & PAH2\_2 & 11.88 &  0.37 &      141 &  0.41 &  0.38 &        3 &  0.48 &  0.39 &      167 &    746.1 $\pm$    38.7 &    605.0 $\pm$    39.0\\
ESO138-G001 & VISIR &  080.B-0860(A)  & 08-03-22 & SIC & 11.85 &  2.34 &      543 &  0.37 &  0.33 &      106 &  0.42 &  0.36 &      116 &    762.4 $\pm$    16.4 &    611.1 $\pm$    20.1\\
ESO138-G001 & VISIR &  080.B-0860(A)  & 08-03-22 & SIV & 10.49 &  0.16 &      540 &  0.31 &  0.30 &      132 &  0.41 &  0.34 &      104 &    623.8 $\pm$    14.8 &    436.8 $\pm$    31.7\\
ESO141-G055 & VISIR &  077.B-0137(A)  & 06-05-05 & NEII\_1 & 12.27 &  0.18 &      180 &  0.38 &  0.38 &      102 &  0.43 &  0.40 &      148 &    164.8 $\pm$     7.3 &    132.6 $\pm$    17.1\\
ESO141-G055 & VISIR &  077.B-0137(A)  & 06-05-05 & PAH2 & 11.25 &  0.59 &      181 &  0.39 &  0.38 &       80 &  0.45 &  0.42 &       81 &    158.7 $\pm$     8.2 &    122.8 $\pm$     3.9\\
ESO141-G055 & VISIR &  077.B-0137(A)  & 06-05-05 & SIV & 10.49 &  0.16 &      176 &  0.38 &  0.38 &      160 &  0.42 &  0.41 &      163 &    145.3 $\pm$     9.5 &    118.7 $\pm$    19.5\\
ESO198-G024 & VISIR &  084.B-0606(A)  & 09-09-28 & NEII & 12.81 &  0.21 &      358 &  0.46 &  0.43 &       82 &  0.43 &  0.37 &       33 &     39.7 $\pm$     6.6 &     48.6 $\pm$     6.6\\
ESO198-G024 & VISIR &  084.B-0606(A)  & 09-09-28 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.45 &  0.42 &       95 &  0.33 &  0.29 &      176 &     31.1 $\pm$     3.9 &     58.9 $\pm$     3.9\\
ESO198-G024 & VISIR &  084.B-0606(A)  & 09-09-17 & SIV & 10.49 &  0.16 &      353 &  0.33 &  0.33 &       55 &  0.39 &  0.36 &       32 &     36.9 $\pm$     3.1 &     31.5 $\pm$     5.5\\
ESO209-G012 & VISIR &  080.B-0860(A)  & 07-11-05 & NEII & 12.81 &  0.21 &       62 &  0.34 &  0.33 &      113 &  0.38 &  0.33 &       76 &    164.1 $\pm$    15.5 &    145.3 $\pm$     8.7\\
ESO209-G012 & VISIR &  080.B-0860(A)  & 07-11-05 & PAH1 &  8.59 &  0.42 &       62 &  0.31 &  0.27 &      117 &  0.30 &  0.28 &      178 &     98.0 $\pm$     5.6 &     96.5 $\pm$     2.8\\
ESO209-G012 & VISIR &  080.B-0860(A)  & 07-11-05 & PAH2 & 11.25 &  0.59 &       63 &  0.32 &  0.30 &      106 &  0.34 &  0.33 &       81 &    145.1 $\pm$    26.5 &    131.1 $\pm$     3.2\\
ESO209-G012 & VISIR &  080.B-0860(A)  & 07-11-05 & SIV & 10.49 &  0.16 &       61 &  0.32 &  0.30 &      132 &  0.31 &  0.30 &      176 &    129.9 $\pm$    13.1 &    131.7 $\pm$     6.1\\
ESO253-G003 & TRECS &  GS-2004A-Q-14  & 04-10-27 & N & 10.36 &  2.64 &      716 &  0.42 &  0.41 &      153 &  0.45 &  0.40 &      124 &    176.7 $\pm$     3.9 &    167.1 $\pm$     3.8\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-25 & ARIII &  8.99 &  0.14 &      690 &  0.32 &  0.28 &       65 &  0.43 &  0.34 &       98 &     34.8 $\pm$     3.2 &     20.3 $\pm$     2.1\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-30 & NEII & 12.81 &  0.21 &      721 &  0.39 &  0.37 &       39 &  0.37 &  0.35 &      152 &     58.1 $\pm$     4.9 &     64.6 $\pm$     9.6\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 08-02-26 & NEII & 12.81 &  0.21 &      724 &  0.37 &  0.35 &      150 &  0.40 &  0.37 &      129 &     61.2 $\pm$    17.9 &     55.5 $\pm$    12.8\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-30 & PAH1 &  8.59 &  0.42 &      724 &  0.33 &  0.29 &      113 &  0.38 &  0.31 &       86 &     28.0 $\pm$     2.3 &     23.1 $\pm$     1.8\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 08-02-26 & PAH1 &  8.59 &  0.42 &      724 &  0.35 &  0.28 &      110 &  0.31 &  0.26 &       91 &     31.7 $\pm$     1.1 &     37.6 $\pm$     1.3\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-30 & PAH2 & 11.25 &  0.59 &      724 &  0.32 &  0.30 &      111 &  0.41 &  0.35 &       64 &     42.8 $\pm$     3.6 &     29.9 $\pm$     3.6\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 08-02-26 & PAH2 & 11.25 &  0.59 &      724 &  0.40 &  0.36 &        9 &  0.33 &  0.30 &       80 &     43.8 $\pm$     3.5 &     61.6 $\pm$     3.6\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-25 & SIC & 11.85 &  2.34 &      717 &  0.36 &  0.34 &       75 &  0.38 &  0.34 &       94 &     52.3 $\pm$     5.6 &     47.6 $\pm$     2.0\\
ESO263-G013 & VISIR &  080.B-0860(A)  & 07-12-25 & SIV & 10.49 &  0.16 &      706 &  0.32 &  0.30 &       61 &  0.33 &  0.30 &      129 &     38.8 $\pm$     5.3 &     37.6 $\pm$     5.2\\
ESO286-IG019 & TRECS &  GS-2008B-C-2  & 08-09-11 & Qa & 18.30 &  0.76 &      926 &  0.57 &  0.55 &      170 &  0.60 &  0.59 &      155 &    449.4 $\pm$    10.1 &    397.5 $\pm$     9.9\\
ESO297-G018 & VISIR &  080.B-0860(A)  & 07-10-09 & NEII & 12.81 &  0.21 &       62 &  0.37 &  0.34 &      109 &  $\dots$  &  $\dots$  &  $\dots$  &     31.3 $\pm$     4.2 &     31.2 $\pm$     4.2\\
ESO297-G018 & VISIR &  080.B-0860(A)  & 07-10-09 & PAH1 &  8.59 &  0.42 &       62 &  0.35 &  0.32 &      107 &  $\dots$  &  $\dots$  &  $\dots$  &     23.2 $\pm$     1.6 &     23.1 $\pm$     1.6\\
ESO297-G018 & VISIR &  080.B-0860(A)  & 07-10-09 & PAH2 & 11.25 &  0.59 &       63 &  0.35 &  0.32 &      116 &  $\dots$  &  $\dots$  &  $\dots$  &     25.7 $\pm$     1.4 &     25.6 $\pm$     1.4\\
ESO297-G018 & VISIR &  080.B-0860(A)  & 07-10-09 & SIV & 10.49 &  0.16 &       61 &  0.35 &  0.32 &      110 &  $\dots$  &  $\dots$  &  $\dots$  &     26.3 $\pm$     2.0 &     26.2 $\pm$     2.0\\
ESO323-G032 & VISIR &  080.B-0860(A)  & 08-02-15 & NEII & 12.81 &  0.21 &      117 &  0.41 &  0.39 &      131 &  $\dots$  &  $\dots$  &  $\dots$  &     56.7 $\pm$     4.8 &     56.2 $\pm$     4.8\\
ESO323-G032 & VISIR &  080.B-0860(A)  & 08-02-15 & PAH1 &  8.59 &  0.42 &      118 &  0.41 &  0.36 &      106 &  $\dots$  &  $\dots$  &  $\dots$  &     10.9 $\pm$     2.1 &     10.8 $\pm$     2.1\\
ESO323-G032 & VISIR &  080.B-0860(A)  & 08-02-15 & PAH2 & 11.25 &  0.59 &      118 &  0.38 &  0.37 &       53 &  $\dots$  &  $\dots$  &  $\dots$  &     30.7 $\pm$     2.3 &     31.0 $\pm$     2.3\\
ESO323-G032 & VISIR &  080.B-0860(A)  & 08-02-15 & SIV & 10.49 &  0.16 &      117 &  0.34 &  0.31 &      110 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    33.9   &  $\le$    33.9  \\
ESO323-G077 & VISIR &  083.B-0239(B)  & 09-05-10 & ARIII &  8.99 &  0.14 &       60 &  0.32 &  0.29 &       75 &  0.43 &  0.37 &       89 &    300.9 $\pm$     9.6 &    180.8 $\pm$    46.6\\
ESO323-G077 & VISIR &  084.B-0366(E)  & 10-03-10 & PAH1 &  8.59 &  0.42 &      362 &  0.26 &  0.24 &      130 &  0.34 &  0.32 &      117 &    275.2 $\pm$    15.5 &    146.5 $\pm$    33.6\\
ESO323-G077 & VISIR &  083.B-0239(B)  & 09-05-10 & PAH2\_2 & 11.88 &  0.37 &       62 &  0.39 &  0.35 &       89 &  0.41 &  0.37 &       56 &    383.4 $\pm$    13.6 &    355.2 $\pm$    21.8\\
ESO323-G077 & VISIR &  084.B-0366(E)  & 10-03-10 & PAH2\_2 & 11.88 &  0.37 &      543 &  0.33 &  0.33 &      124 &  0.40 &  0.38 &      101 &    378.7 $\pm$    13.7 &    279.5 $\pm$    61.4\\
ESO362-G018 & VISIR &  084.B-0606(A)  & 09-11-12 & NEII\_1 & 12.27 &  0.18 &      540 &  0.38 &  0.37 &       18 &  0.38 &  0.37 &      164 &    157.5 $\pm$    10.3 &    155.8 $\pm$    10.6\\
ESO362-G018 & VISIR &  084.B-0606(A)  & 09-11-12 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.33 &      177 &  0.33 &  0.32 &       94 &    132.3 $\pm$     4.5 &    138.5 $\pm$    10.3\\
ESO362-G018 & TRECS &  GS-2008B-Q-36  & 08-11-24 & Si2 &  8.74 &  0.39 &      318 &  $\dots$  &  $\dots$  &  $\dots$  &  0.38 &  0.36 &       73 &     57.4 $\pm$     5.3 &  $\le$    73.4  \\
ESO362-G018 & VISIR &  084.B-0606(A)  & 09-11-12 & SIV\_2 & 10.77 &  0.19 &      905 &  0.35 &  0.34 &       54 &  0.38 &  0.35 &      158 &    136.4 $\pm$     4.8 &    118.8 $\pm$     2.8\\
ESO416-G002 & VISIR &  084.B-0606(A)  & 09-09-28 & NEII\_2 & 13.04 &  0.22 &      901 &  0.43 &  0.40 &       98 &  0.47 &  0.35 &       44 &     24.9 $\pm$     2.4 &     27.0 $\pm$     3.4\\
ESO416-G002 & VISIR &  084.B-0606(A)  & 09-09-28 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.45 &  0.42 &       95 &  0.46 &  0.31 &       24 &     18.1 $\pm$     4.3 &     24.2 $\pm$     4.3\\
ESO416-G002 & VISIR &  084.B-0606(A)  & 09-09-28 & SIV\_2 & 10.77 &  0.19 &      362 &  0.47 &  0.39 &      135 &  0.47 &  0.37 &       67 &     24.3 $\pm$     9.4 &     24.2 $\pm$     6.2\\
ESO420-G013 & VISIR &  076.B-0696(A)  & 06-01-19 & NEII & 12.81 &  0.21 &     2587 &  0.39 &  0.38 &       64 &  0.49 &  0.44 &       67 &    285.1 $\pm$     6.1 &    196.2 $\pm$     4.9\\
ESO420-G013 & VISIR &  076.B-0696(A)  & 06-01-19 & NEII\_2 & 13.04 &  0.22 &     3670 &  0.40 &  0.39 &      117 &  0.48 &  0.47 &       26 &    333.8 $\pm$    15.7 &    217.6 $\pm$    10.7\\
ESO420-G013 & VISIR &  076.B-0696(A)  & 06-01-19 & SIC & 11.85 &  2.34 &      543 &  0.38 &  0.35 &       49 &  0.45 &  0.43 &       28 &    201.3 $\pm$    26.1 &    141.8 $\pm$    17.9\\
ESO428-G014 & VISIR &  078.B-0303(A)  & 07-03-01 & ARIII &  8.99 &  0.14 &      699 &  0.33 &  0.29 &      142 &  0.41 &  0.38 &      116 &    115.2 $\pm$     0.6 &     70.0 $\pm$     0.4\\
ESO428-G014 & VISIR &  078.B-0303(A)  & 07-03-01 & PAH2\_2 & 11.88 &  0.37 &      362 &  0.33 &  0.32 &      141 &  0.48 &  0.40 &      129 &    211.8 $\pm$     5.4 &    114.7 $\pm$    12.7\\
ESO428-G014 & VISIR &  078.B-0303(A)  & 07-03-01 & Q1 & 17.65 &  0.83 &      684 &  0.47 &  0.46 &      153 &  0.96 &  0.57 &      139 &    768.6 $\pm$    45.1 &    308.4 $\pm$    11.8\\
ESO428-G014 & VISIR &  078.B-0303(A)  & 07-03-01 & PAH1 &  8.59 &  0.42 &       62 &  0.32 &  0.28 &      136 &  0.40 &  0.37 &      175 &    114.6 $\pm$    13.4 &     71.8 $\pm$    11.3\\
ESO500-G034 & VISIR &  60.A-9244(A)  & 05-01-27 & PAH2 & 11.25 &  0.59 &     1766 &  0.43 &  0.40 &      107 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   190.9   &  $\le$    33.0  \\
ESO506-G027 & VISIR &  084.B-0606(A)  & 10-01-09 & NEII & 12.81 &  0.21 &      180 &  0.38 &  0.34 &       44 &  0.40 &  0.35 &       99 &    179.5 $\pm$    15.1 &    170.7 $\pm$    10.4\\
ESO506-G027 & VISIR &  084.B-0606(A)  & 10-01-09 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.38 &  0.33 &       46 &  0.39 &  0.33 &       85 &    107.7 $\pm$    11.3 &    107.7 $\pm$     5.8\\
ESO506-G027 & VISIR &  084.B-0606(A)  & 10-01-09 & SIV & 10.49 &  0.16 &      179 &  0.34 &  0.29 &       40 &  0.33 &  0.28 &       97 &     50.7 $\pm$     7.2 &     56.6 $\pm$     7.8\\
ESO511-G030 & VISIR &  084.B-0606(A)  & 10-01-27 & NEII & 12.81 &  0.21 &      180 &  0.35 &  0.34 &      164 &  $\dots$  &  $\dots$  &  $\dots$  &     42.8 $\pm$     3.5 &     42.8 $\pm$     3.5\\
ESO511-G030 & VISIR &  084.B-0606(A)  & 10-01-27 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.30 &      158 &  0.45 &  0.32 &       80 &     58.8 $\pm$     8.5 &     40.1 $\pm$     4.2\\
ESO511-G030 & VISIR &  084.B-0606(A)  & 10-01-27 & SIV & 10.49 &  0.16 &      179 &  0.31 &  0.30 &      166 &  0.41 &  0.34 &       80 &     56.4 $\pm$     8.6 &     36.2 $\pm$     1.8\\
ESO548-G081 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_1 & 12.27 &  0.18 &      180 &  0.43 &  0.40 &       10 &  0.61 &  0.43 &      106 &    121.4 $\pm$    12.6 &     72.8 $\pm$     9.7\\
ESO548-G081 & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.33 &      163 &  0.59 &  0.51 &       78 &    113.3 $\pm$    18.2 &     42.6 $\pm$     3.5\\
ESO548-G081 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV\_2 & 10.77 &  0.19 &      362 &  0.37 &  0.34 &      171 &  0.58 &  0.53 &       14 &    114.1 $\pm$    22.8 &     45.3 $\pm$     6.8\\
ESO602-G025 & TRECS &  GS-2009B-C-3  & 09-09-09 & Qa & 18.30 &  0.76 &      926 &  0.59 &  0.58 &      159 &  1.00 &  0.85 &       33 &    132.7 $\pm$     7.5 &     42.9 $\pm$     7.3\\
Fairall0009 & VISIR &  085.B-0251(C)  & 10-07-11 & ARIII &  8.99 &  0.14 &      159 &  0.31 &  0.29 &      158 &  0.38 &  0.32 &      171 &    196.0 $\pm$     8.0 &    145.5 $\pm$    11.6\\
Fairall0009 & VISIR &  075.B-0844(C)  & 05-07-21 & NEII & 12.81 &  0.21 &      358 &  0.44 &  0.39 &       91 &  0.43 &  0.41 &       99 &    301.2 $\pm$    16.1 &    295.4 $\pm$    10.3\\
Fairall0009 & VISIR &  075.B-0844(C)  & 05-07-21 & NEII\_1 & 12.27 &  0.18 &      360 &  0.39 &  0.37 &       97 &  0.39 &  0.38 &      152 &    303.9 $\pm$    16.5 &    281.2 $\pm$     6.5\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-10-07 & PAH1 &  8.59 &  0.42 &      360 &  0.50 &  0.46 &      117 &  0.58 &  0.54 &       30 &    209.1 $\pm$     7.4 &    156.2 $\pm$    11.0\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-10-15 & PAH1 &  8.59 &  0.42 &      360 &  0.30 &  0.27 &      100 &  0.32 &  0.28 &      124 &    187.8 $\pm$     5.9 &    170.9 $\pm$     5.7\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-10-21 & PAH1 &  8.59 &  0.42 &      360 &  0.30 &  0.27 &      147 &  0.46 &  0.43 &       22 &    195.9 $\pm$     9.7 &     85.6 $\pm$     4.4\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-10-25 & PAH1 &  8.59 &  0.42 &      360 &  0.38 &  0.32 &      119 &  0.29 &  0.27 &      141 &    189.4 $\pm$     7.3 &    289.6 $\pm$    15.1\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-11-09 & PAH1 &  8.59 &  0.42 &      362 &  0.27 &  0.26 &      137 &  0.26 &  0.26 &      121 &    185.1 $\pm$     4.1 &    194.4 $\pm$     4.5\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-11-11 & PAH1 &  8.59 &  0.42 &      360 &  0.38 &  0.29 &      101 &  0.29 &  0.26 &      119 &    191.6 $\pm$     7.0 &    279.9 $\pm$    12.7\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-11-22 & PAH1 &  8.59 &  0.42 &      360 &  0.31 &  0.28 &      129 &  0.32 &  0.28 &        1 &    196.7 $\pm$     5.1 &    193.4 $\pm$    15.6\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-11-26 & PAH1 &  8.59 &  0.42 &      360 &  0.26 &  0.25 &      141 &  0.27 &  0.26 &      159 &    188.2 $\pm$     2.6 &    170.3 $\pm$    12.1\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-12-08 & PAH1 &  8.59 &  0.42 &      360 &  0.28 &  0.26 &      108 &  0.32 &  0.29 &      138 &    197.8 $\pm$     7.6 &    149.8 $\pm$    10.7\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-12-13 & PAH1 &  8.59 &  0.42 &      360 &  0.49 &  0.44 &      117 &  0.53 &  0.47 &       11 &    196.4 $\pm$     3.8 &    163.3 $\pm$    13.5\\
Fairall0009 & VISIR &  086.B-0242(A)  & 10-12-24 & PAH1 &  8.59 &  0.42 &      361 &  0.29 &  0.26 &      125 &  0.31 &  0.28 &       14 &    195.2 $\pm$     4.3 &    171.6 $\pm$     6.0\\
Fairall0009 & VISIR &  085.B-0251(C)  & 10-07-11 & PAH2\_2 & 11.88 &  0.37 &      164 &  0.38 &  0.34 &      172 &  0.41 &  0.36 &        2 &    266.9 $\pm$    13.3 &    227.9 $\pm$    12.8\\
Fairall0009 & VISIR &  075.B-0844(C)  & 05-07-21 & SIV & 10.49 &  0.16 &      353 &  0.35 &  0.33 &      107 &  0.41 &  0.37 &      117 &    268.7 $\pm$     0.7 &    203.4 $\pm$    10.7\\
Fairall0009 & VISIR &  085.B-0251(C)  & 10-07-11 & NEII\_2 & 13.04 &  0.22 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  0.38 &  0.36 &       13 &    311.3 $\pm$    48.3 &  $\le$   456.3  \\
Fairall0049 & VISIR &  085.B-0251(C)  & 10-09-01 & ARIII &  8.99 &  0.14 &      135 &  0.54 &  0.50 &      100 &  0.59 &  0.50 &       24 &    314.9 $\pm$    23.0 &    274.4 $\pm$    34.3\\
Fairall0049 & VISIR &  085.B-0251(C)  & 10-09-01 & PAH2\_2 & 11.88 &  0.37 &      141 &  0.46 &  0.45 &       87 &  0.78 &  0.68 &       57 &    523.5 $\pm$    30.6 &    212.2 $\pm$    50.1\\
Fairall0049 & VISIR &  085.B-0251(C)  & 10-09-01 & NEII\_2 & 13.04 &  0.22 &       62 &  $\dots$  &  $\dots$  &  $\dots$  &  0.58 &  0.52 &       51 &    675.3 $\pm$   119.6 &  $\le$  1034.3  \\
Fairall0051 & TRECS &  GS-2007A-DD-7  & 07-06-04 & Qa & 18.30 &  0.76 &      847 &  0.65 &  0.59 &       47 &  0.61 &  0.57 &      179 &    712.5 $\pm$    22.1 &    780.5 $\pm$    22.9\\
FornaxA & VISIR &  384.B-0943(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.39 &  0.37 &        1 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.5   &  $\le$    12.5  \\
FornaxA & TRECS &  GS-2007A-Q-40  & 07-06-29 & Si2 &  8.74 &  0.39 &      608 &  0.47 &  0.44 &       49 &  0.60 &  0.48 &       76 &     13.9 $\pm$     0.4 &      9.6 $\pm$     0.3\\
FornaxA & TRECS &  GS-2007A-Q-40  & 07-09-01 & Si6 & 12.33 &  0.59 &      608 &  0.47 &  0.38 &       69 &  0.60 &  0.47 &       93 &     21.3 $\pm$     0.3 &     13.6 $\pm$     0.2\\
FornaxA & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    26.4   &  $\le$    26.4  \\
H0557-385 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII & 12.81 &  0.21 &      179 &  0.61 &  0.51 &      134 &  0.51 &  0.46 &      155 &    480.3 $\pm$    57.4 &    654.6 $\pm$    56.3\\
H0557-385 & VISIR &  083.B-0452(F)  & 09-09-07 & PAH1 &  8.59 &  0.42 &      235 &  0.44 &  0.36 &      111 &  0.38 &  0.33 &       83 &    330.6 $\pm$    10.8 &    423.3 $\pm$    20.4\\
H0557-385 & VISIR &  083.B-0452(F)  & 09-09-07 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.41 &  0.36 &       99 &  0.43 &  0.36 &       80 &    413.1 $\pm$    59.1 &    385.0 $\pm$    31.9\\
H0557-385 & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.63 &  0.52 &      128 &  0.54 &  0.48 &      151 &    382.4 $\pm$    16.8 &    483.2 $\pm$    87.9\\
H0557-385 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV & 10.49 &  0.16 &      176 &  0.35 &  0.33 &        7 &  0.49 &  0.43 &      135 &    342.2 $\pm$     6.3 &    187.2 $\pm$    23.4\\
H1143-182 & VISIR &  084.B-0606(A)  & 10-01-08 & NEII & 12.81 &  0.21 &      180 &  0.36 &  0.33 &       39 &  0.38 &  0.32 &       76 &     55.7 $\pm$    10.8 &     54.4 $\pm$    10.8\\
H1143-182 & VISIR &  084.B-0606(A)  & 10-01-08 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.37 &  0.31 &       35 &  0.36 &  0.30 &       87 &     44.5 $\pm$     8.6 &     46.3 $\pm$     8.6\\
H1143-182 & VISIR &  084.B-0606(A)  & 10-01-08 & SIV & 10.49 &  0.16 &      179 &  0.32 &  0.28 &       41 &  0.35 &  0.30 &       70 &     58.8 $\pm$     7.7 &     50.8 $\pm$     7.7\\
HydraA & VISIR &  084.B-0974(A)  & 09-11-30 & PAH1 &  8.59 &  0.42 &     4345 &  0.34 &  0.30 &      128 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     2.5   &  $\le$     2.5  \\
IC0883 & COMICS &  o09102  & 09-04-07 & Q17.7 & 17.69 &  0.43 &     3223 &  0.63 &  0.54 &       48 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   496.3   &    302.6 $\pm$     0.0\\
IC1459 & VISIR &  083.B-0536(C)  & 09-06-06 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.34 &  0.32 &       83 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    16.4   &  $\le$    16.4  \\
IC1459 & VISIR &  083.B-0536(C)  & 09-06-06 & PAH2 & 11.25 &  0.59 &      362 &  0.30 &  0.29 &       24 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.2   &  $\le$    12.2  \\
IC1459 & VISIR &  384.B-0943(A)  & 09-12-04 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.39 &  0.38 &       46 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    14.9   &  $\le$    14.9  \\
IC3639 & VISIR &  080.B-0860(A)  & 08-03-22 & NEII\_2 & 13.04 &  0.22 &      722 &  0.38 &  0.35 &      141 &  0.40 &  0.37 &       78 &    556.0 $\pm$    12.8 &    484.1 $\pm$    17.5\\
IC3639 & TRECS &  GS-2004A-Q-14  & 04-03-05 & N & 10.36 &  2.64 &      304 &  0.45 &  0.40 &      137 &  0.42 &  0.39 &      174 &    304.4 $\pm$     8.9 &    326.1 $\pm$     9.0\\
IC3639 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH1 &  8.59 &  0.42 &      724 &  0.36 &  0.34 &      109 &  0.33 &  0.29 &      106 &    138.7 $\pm$     4.1 &    167.0 $\pm$    15.2\\
IC3639 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH2 & 11.25 &  0.59 &      724 &  0.36 &  0.32 &      163 &  0.35 &  0.33 &       97 &    313.6 $\pm$     6.4 &    312.1 $\pm$    15.5\\
IC4329A & VISIR &  083.B-0239(B)  & 09-05-10 & ARIII &  8.99 &  0.14 &       60 &  0.32 &  0.29 &       75 &  0.43 &  0.32 &       47 &    774.7 $\pm$    49.3 &    602.2 $\pm$   146.3\\
IC4329A & VISIR &  084.B-0606(A)  & 10-03-12 & NEII\_1 & 12.27 &  0.18 &      181 &  0.42 &  0.35 &      127 &  0.41 &  0.35 &       66 &   1178.1 $\pm$    31.8 &   1185.9 $\pm$    48.0\\
IC4329A & VISIR &  084.B-0606(A)  & 10-03-12 & PAH2 & 11.25 &  0.59 &      362 &  0.39 &  0.33 &      118 &  0.38 &  0.31 &       70 &   1052.7 $\pm$     9.8 &   1122.9 $\pm$    11.5\\
IC4329A & VISIR &  083.B-0239(B)  & 09-05-10 & PAH2\_2 & 11.88 &  0.37 &       62 &  0.39 &  0.35 &       89 &  0.49 &  0.38 &       59 &   1075.0 $\pm$    63.8 &    867.5 $\pm$   218.6\\
IC4329A & TRECS &  GS-2009A-Q-59  & 09-07-13 & Qa & 18.30 &  0.76 &      608 &  0.80 &  0.77 &       68 &  0.77 &  0.68 &       56 &   2219.8 $\pm$   141.6 &   2597.5 $\pm$   162.8\\
IC4329A & TRECS &  GS-2009A-Q-59  & 09-07-13 & Si2 &  8.74 &  0.39 &      405 &  0.98 &  0.97 &       28 &  0.85 &  0.77 &       57 &    724.2 $\pm$    12.8 &   1053.7 $\pm$    15.3\\
IC4329A & VISIR &  084.B-0606(A)  & 10-03-12 & SIV & 10.49 &  0.16 &      179 &  0.40 &  0.32 &      117 &  0.41 &  0.31 &       70 &    922.1 $\pm$    34.4 &    929.5 $\pm$    23.2\\
IC4518W & TRECS &  GS-2005B-Q-10  & 06-04-10 & N & 10.36 &  2.64 &      608 &  0.55 &  0.51 &       18 &  0.58 &  0.54 &      157 &    115.7 $\pm$     2.2 &    105.4 $\pm$     3.8\\
IC5063 & VISIR &  075.B-0844(C)  & 05-06-10 & NEII\_1 & 12.27 &  0.18 &      180 &  0.43 &  0.42 &       15 &  0.50 &  0.44 &      120 &   1114.1 $\pm$    42.6 &    898.4 $\pm$    41.2\\
IC5063 & VISIR &  077.B-0137(A)  & 06-05-05 & NEII\_1 & 12.27 &  0.18 &      180 &  0.38 &  0.38 &      102 &  0.49 &  0.39 &      107 &   1037.3 $\pm$    62.5 &    771.3 $\pm$    48.5\\
IC5063 & TRECS &  GS-2004A-Q-14  & 04-07-08 & N & 10.36 &  2.64 &      716 &  0.35 &  0.35 &      111 &  0.53 &  0.40 &      103 &    708.7 $\pm$    10.0 &    408.3 $\pm$     8.2\\
IC5063 & TRECS &  GS-2005A-Q-6  & 05-07-09 & N & 10.36 &  2.64 &       32 &  0.44 &  0.37 &      104 &  0.54 &  0.44 &      107 &    688.5 $\pm$    13.4 &    475.0 $\pm$    11.7\\
IC5063 & VISIR &  077.B-0137(A)  & 06-05-05 & PAH2 & 11.25 &  0.59 &      181 &  0.39 &  0.38 &       80 &  0.50 &  0.38 &      109 &    735.7 $\pm$    28.9 &    559.6 $\pm$    29.7\\
IC5063 & VISIR &  075.B-0844(C)  & 05-06-10 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.40 &  0.38 &       32 &  0.45 &  0.39 &      111 &    928.5 $\pm$    22.0 &    806.9 $\pm$    23.4\\
IC5063 & TRECS &  GS-2005A-Q-6  & 05-07-18 & Qa & 18.30 &  0.76 &      304 &  0.57 &  0.54 &       22 &  0.62 &  0.57 &      104 &   2111.7 $\pm$    38.8 &   1849.9 $\pm$    37.3\\
IC5063 & TRECS &  GS-2005A-Q-6  & 05-07-18 & Si2 &  8.74 &  0.39 &      130 &  0.48 &  0.40 &       21 &  0.54 &  0.50 &      114 &    481.0 $\pm$    10.1 &    342.0 $\pm$     9.0\\
IC5063 & VISIR &  075.B-0844(C)  & 05-06-10 & SIV & 10.49 &  0.16 &      353 &  0.41 &  0.39 &       99 &  0.50 &  0.40 &      105 &    670.2 $\pm$    13.6 &    535.6 $\pm$    11.4\\
IC5063 & VISIR &  077.B-0137(A)  & 06-05-05 & SIV & 10.49 &  0.16 &      176 &  0.38 &  0.38 &      160 &  0.55 &  0.42 &      110 &    612.4 $\pm$    18.2 &    380.0 $\pm$    10.0\\
IIIZW035N & VISIR &  084.B-0974(A)  & 09-10-06 & PAH1 &  8.59 &  0.42 &     3967 &  0.46 &  0.40 &       76 &  0.61 &  0.45 &       31 &     48.2 $\pm$     1.3 &     32.3 $\pm$     0.9\\
IRAS00188-0856 & TRECS &  GS-2009B-C-3  & 09-09-09 & Qa & 18.30 &  0.76 &     1853 &  0.71 &  0.64 &       76 &  0.63 &  0.59 &      147 &     73.9 $\pm$     1.3 &     89.1 $\pm$     9.8\\
IRAS01003-2238 & TRECS &  GS-2008B-C-2  & 08-09-11 & Qa & 18.30 &  0.76 &     1853 &  0.63 &  0.57 &       92 &  0.59 &  0.57 &       80 &    325.3 $\pm$     6.7 &    346.1 $\pm$    30.9\\
IRAS04103-2838 & TRECS &  GS-2008B-C-2  & 08-09-11 & Qa & 18.30 &  0.76 &      926 &  0.64 &  0.55 &       33 &  0.69 &  0.57 &       77 &    281.9 $\pm$    12.1 &    250.0 $\pm$    12.0\\
IRAS05189-2524 & TRECS &  GS-2004A-Q-14  & 04-03-11 & N & 10.36 &  2.64 &      716 &  0.41 &  0.39 &       86 &  0.47 &  0.41 &       95 &    426.8 $\pm$     6.8 &    353.0 $\pm$     6.2\\
IRAS05189-2524 & VISIR &  086.B-0919(A)  & 10-11-22 & ARIII &  8.99 &  0.14 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  0.43 &  0.41 &       94 &    413.6 $\pm$    18.5 &  $\le$   469.0  \\
IRAS05189-2524 & VISIR &  086.B-0919(A)  & 10-11-25 & PAH2\_2 & 11.88 &  0.37 &      115 &  $\dots$  &  $\dots$  &  $\dots$  &  0.43 &  0.41 &       88 &    670.4 $\pm$   220.7 &  $\le$  1332.5  \\
IRAS08572+3915 & COMICS &  o07146  & 08-01-24 & Q17.7 & 17.69 &  0.43 &     1922 &  0.63 &  0.50 &       22 &  0.66 &  0.60 &       14 &    610.8 $\pm$    45.1 &    491.8 $\pm$    49.7\\
IRAS09149-6206 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH1 &  8.59 &  0.42 &      117 &  0.50 &  0.40 &       88 &  0.28 &  0.26 &       85 &    334.9 $\pm$    16.3 &    939.4 $\pm$    56.2\\
IRAS09149-6206 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.49 &  0.40 &       83 &  0.34 &  0.33 &       68 &    486.5 $\pm$    16.2 &    833.2 $\pm$    32.8\\
IRAS11095-0238 & COMICS &  o09102  & 09-04-07 & N8.8 &  8.75 &  0.38 &       61 &  0.72 &  0.55 &      138 &  0.53 &  0.42 &       17 &     61.3 $\pm$    16.3 &    113.3 $\pm$    12.8\\
IRAS13349+2438 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH1 &  8.59 &  0.42 &      117 &  0.50 &  0.40 &       88 &  0.43 &  0.40 &        4 &    388.3 $\pm$    17.2 &    470.6 $\pm$    30.2\\
IRAS13349+2438 & VISIR &  083.B-0452(F)  & 09-06-08 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.49 &  0.40 &       83 &  0.43 &  0.41 &       30 &    512.7 $\pm$    10.7 &    582.5 $\pm$    70.7\\
IRAS15250+3609 & COMICS &  o09102  & 09-04-07 & N8.8 &  8.75 &  0.38 &       21 &  0.72 &  0.55 &      138 &  0.82 &  0.54 &      142 &    157.0 $\pm$     7.1 &    136.6 $\pm$    11.8\\
IRAS15250+3609 & COMICS &  o09102  & 09-04-07 & Q17.7 & 17.69 &  0.43 &     3626 &  0.60 &  0.54 &      114 &  1.00 &  0.54 &       64 &    280.1 $\pm$    47.7 &    182.5 $\pm$    17.4\\
IZW001 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     1605 &  0.63 &  0.38 &      137 &  0.70 &  0.47 &      130 &    477.2 $\pm$    22.3 &    333.6 $\pm$    24.1\\
IZW001 & VISIR &  086.B-0919(A)  & 10-10-20 & ARIII &  8.99 &  0.14 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  0.32 &  0.28 &       10 &    303.6 $\pm$    27.3 &  $\le$   385.6  \\
IZW001 & VISIR &  086.B-0919(A)  & 10-10-17 & PAH2\_2 & 11.88 &  0.37 &      115 &  0.45 &  0.43 &       21 &  0.54 &  0.46 &       59 &    445.8 $\pm$    50.7 &    341.5 $\pm$    26.0\\
LEDA013946 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII & 12.81 &  0.21 &     1076 &  0.39 &  0.37 &      175 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    14.8   &  $\le$    14.8  \\
LEDA013946 & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.39 &  0.37 &        1 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    16.0   &  $\le$    16.0  \\
LEDA013946 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV & 10.49 &  0.16 &      529 &  0.35 &  0.33 &        7 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.1   &  $\le$    12.1  \\
LEDA170194 & VISIR &  084.B-0606(A)  & 10-01-09 & NEII & 12.81 &  0.21 &      360 &  0.38 &  0.34 &       44 &  0.35 &  0.29 &       30 &     44.4 $\pm$     6.9 &     55.2 $\pm$    11.5\\
LEDA170194 & VISIR &  084.B-0606(A)  & 10-01-09 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.38 &  0.33 &       46 &  0.37 &  0.36 &       46 &     40.9 $\pm$     6.0 &     37.8 $\pm$     6.0\\
LEDA170194 & VISIR &  084.B-0606(A)  & 10-01-09 & SIV & 10.49 &  0.16 &      179 &  0.34 &  0.29 &       40 &  0.35 &  0.30 &       64 &     39.0 $\pm$    11.0 &     40.8 $\pm$     4.1\\
LEDA178130 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII & 12.81 &  0.21 &     1255 &  0.39 &  0.37 &      175 &  0.52 &  0.48 &      137 &     67.0 $\pm$     3.8 &     39.5 $\pm$     4.8\\
LEDA178130 & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.39 &  0.37 &        1 &  0.49 &  0.47 &      128 &     63.5 $\pm$     2.9 &     40.0 $\pm$     4.4\\
LEDA178130 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV & 10.49 &  0.16 &      529 &  0.71 &  0.63 &      138 &  0.68 &  0.56 &       53 &     49.9 $\pm$     6.7 &     57.6 $\pm$     6.7\\
LEDA549777 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_2 & 13.04 &  0.22 &     1983 &  0.64 &  0.55 &      137 &  0.66 &  0.47 &      123 &     32.7 $\pm$     4.0 &     32.9 $\pm$     4.6\\
M051A & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-5 & 11.60 &  0.55 &      518 &  0.58 &  0.47 &       57 &  0.85 &  0.79 &       59 &     35.0 $\pm$     2.5 &     14.3 $\pm$     2.4\\
M051A & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      517 &  0.61 &  0.47 &       63 &  0.82 &  0.77 &       44 &     37.2 $\pm$     2.5 &     16.8 $\pm$     2.5\\
M081 & MICHELLE &  GN-2011A-Q-55  & 11-02-04 & Qa & 18.10 &  0.95 &      324 &  0.58 &  0.54 &       32 &  0.66 &  0.59 &       17 &    330.9 $\pm$    29.5 &    263.9 $\pm$    29.4\\
M081 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-2 &  8.80 &  0.45 &      311 &  0.50 &  0.44 &       35 &  0.46 &  0.43 &       30 &     67.9 $\pm$     2.3 &     72.4 $\pm$     2.3\\
M081 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-4 & 10.30 &  0.50 &      309 &  0.50 &  0.44 &       44 &  0.53 &  0.51 &      145 &    188.5 $\pm$     4.9 &    154.8 $\pm$     4.5\\
M081 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-6 & 12.50 &  0.60 &      329 &  0.47 &  0.43 &       42 &  0.50 &  0.48 &      171 &    168.1 $\pm$     3.5 &    138.7 $\pm$     3.4\\
M081 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-5 & 11.60 &  0.55 &      155 &  0.45 &  0.41 &       31 &  0.52 &  0.48 &       27 &    170.2 $\pm$     4.1 &    127.1 $\pm$     3.8\\
M081 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      141 &  0.44 &  0.41 &       59 &  0.52 &  0.46 &       30 &    156.0 $\pm$     4.2 &    116.8 $\pm$     4.1\\
M087 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &      401 &  0.45 &  0.38 &       12 &  $\dots$  &  $\dots$  &  $\dots$  &     20.5 $\pm$     1.8 &     20.4 $\pm$     1.8\\
M087 & VISIR &  085.B-0639(C)  & 11-05-18 & PAH1 &  8.59 &  0.42 &      540 &  0.35 &  0.31 &      153 &  0.32 &  0.29 &      142 &     11.9 $\pm$     3.0 &     15.5 $\pm$     3.1\\
M087 & VISIR &  077.B-0728(A)  & 06-05-17 & PAH2\_2 & 11.88 &  0.37 &     1986 &  0.32 &  0.31 &      115 &  0.36 &  0.33 &       47 &     21.6 $\pm$     2.9 &     17.6 $\pm$     2.3\\
M087 & VISIR &  076.B-0599(A)  & 06-03-09 & Q2 & 18.72 &  0.88 &     1881 &  0.50 &  0.47 &      103 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    46.4   &  $\le$    46.4  \\
M087 & VISIR &  076.B-0599(A)  & 06-03-13 & Q2 & 18.72 &  0.88 &     2052 &  0.52 &  0.50 &      104 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    45.6   &  $\le$    45.6  \\
M087 & VISIR &  085.B-0639(C)  & 11-05-18 & SIV\_2 & 10.77 &  0.19 &      905 &  0.44 &  0.34 &      154 &  0.34 &  0.28 &      110 &     15.0 $\pm$     2.0 &     25.4 $\pm$     3.4\\
MCG-01-05-047 & VISIR &  382.A-0604(A)  & 08-09-15 & B10.7 & 10.65 &  1.37 &      181 &  0.36 &  0.33 &      147 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    25.9   &  $\le$    25.9  \\
MCG-01-05-047 & VISIR &  382.A-0604(A)  & 08-09-15 & B11.7 & 11.52 &  0.85 &      180 &  0.35 &  0.33 &      138 &  0.44 &  0.37 &       88 &     35.9 $\pm$     9.5 &     24.1 $\pm$     9.5\\
MCG-01-05-047 & VISIR &  382.A-0604(A)  & 08-09-15 & B12.4 & 12.47 &  0.99 &      362 &  0.37 &  0.35 &      137 &  0.38 &  0.34 &        5 &     62.6 $\pm$     6.9 &     62.3 $\pm$     4.2\\
MCG-01-05-047 & VISIR &  382.A-0604(A)  & 08-09-15 & B9.7 &  9.82 &  0.84 &      362 &  0.35 &  0.32 &      140 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    31.4   &  $\le$    31.4  \\
MCG-01-05-047 & VISIR &  382.A-0604(A)  & 08-09-15 & J7.9 &  7.76 &  0.55 &      360 &  0.27 &  0.26 &      153 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    23.2   &  $\le$    23.2  \\
MCG-01-13-025 & VISIR &  084.B-0606(A)  & 09-11-16 & NEII\_1 & 12.27 &  0.18 &      180 &  0.35 &  0.33 &      109 &  0.53 &  0.34 &       17 &     32.6 $\pm$    18.1 &     21.0 $\pm$    18.1\\
MCG-01-13-025 & VISIR &  084.B-0606(A)  & 09-11-16 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.31 &      101 &  0.44 &  0.38 &       37 &     42.4 $\pm$     4.0 &     26.9 $\pm$     2.2\\
MCG-01-13-025 & VISIR &  084.B-0606(A)  & 09-11-16 & SIV & 10.49 &  0.16 &      176 &  0.30 &  0.29 &      141 &  0.37 &  0.32 &      107 &     37.0 $\pm$     8.6 &     24.9 $\pm$     0.5\\
MCG-01-24-012 & VISIR &  084.B-0606(A)  & 09-11-17 & NEII\_1 & 12.27 &  0.18 &      180 &  0.35 &  0.33 &       39 &  0.40 &  0.36 &      175 &    146.0 $\pm$    20.9 &    118.2 $\pm$    11.1\\
MCG-01-24-012 & VISIR &  084.B-0606(A)  & 09-11-17 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.31 &       31 &  0.33 &  0.31 &      100 &     94.9 $\pm$    15.3 &     92.0 $\pm$     3.4\\
MCG-01-24-012 & VISIR &  084.B-0606(A)  & 09-11-17 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.29 &       65 &  0.30 &  0.24 &       89 &     47.4 $\pm$    12.9 &     60.5 $\pm$    12.9\\
MCG-02-08-014 & VISIR &  382.A-0604(A)  & 09-08-13 & B10.7 & 10.65 &  1.37 &      115 &  0.34 &  0.31 &       96 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    18.9   &  $\le$    18.9  \\
MCG-02-08-014 & VISIR &  382.A-0604(A)  & 09-08-13 & B11.7 & 11.52 &  0.85 &      112 &  0.36 &  0.33 &      102 &  $\dots$  &  $\dots$  &  $\dots$  &     27.6 $\pm$     1.7 &     27.6 $\pm$     1.7\\
MCG-02-08-014 & VISIR &  382.A-0604(A)  & 09-08-13 & B12.4 & 12.47 &  0.99 &      176 &  0.38 &  0.33 &      102 &  0.41 &  0.35 &       79 &     43.6 $\pm$     7.7 &     36.2 $\pm$     7.7\\
MCG-02-08-014 & VISIR &  382.A-0604(A)  & 09-08-13 & B9.7 &  9.82 &  0.84 &      176 &  0.35 &  0.33 &       96 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    30.1   &  $\le$    30.1  \\
MCG-02-08-014 & VISIR &  382.A-0604(A)  & 09-08-13 & J7.9 &  7.76 &  0.55 &      338 &  0.34 &  0.29 &      152 &  $\dots$  &  $\dots$  &  $\dots$  &     33.9 $\pm$     2.1 &     33.5 $\pm$     2.1\\
MCG-02-08-039 & TRECS &  GS-2007A-DD-7  & 07-07-02 & Qa & 18.30 &  0.76 &      282 &  0.58 &  0.52 &       73 &  0.61 &  0.52 &       68 &    334.1 $\pm$    23.9 &    321.9 $\pm$    23.9\\
MCG-02-08-039 & TRECS &  GS-2007A-DD-7  & 07-09-14 & Qa & 18.30 &  0.76 &      564 &  0.65 &  0.64 &        5 &  0.69 &  0.67 &       44 &    390.8 $\pm$    18.7 &    351.8 $\pm$    30.0\\
MCG-03-34-064 & VISIR &  077.B-0137(A)  & 06-04-09 & NEII\_1 & 12.27 &  0.18 &      180 &  0.37 &  0.33 &       83 &  0.51 &  0.40 &       44 &    898.6 $\pm$    25.8 &    530.6 $\pm$    38.2\\
MCG-03-34-064 & VISIR &  076.B-0696(A)  & 06-01-18 & NEII\_2 & 13.04 &  0.22 &     3532 &  0.46 &  0.39 &       25 &  0.55 &  0.42 &       45 &   1130.1 $\pm$    26.2 &    890.5 $\pm$    73.9\\
MCG-03-34-064 & VISIR &  077.B-0137(A)  & 06-04-09 & PAH2 & 11.25 &  0.59 &      181 &  0.35 &  0.32 &       88 &  0.52 &  0.37 &       58 &    740.5 $\pm$    34.0 &    427.9 $\pm$    39.2\\
MCG-03-34-064 & VISIR &  077.B-0137(A)  & 06-04-09 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.29 &       94 &  0.48 &  0.34 &       58 &    585.1 $\pm$    16.6 &    324.4 $\pm$    41.0\\
MCG-05-23-016 & VISIR &  078.B-0303(A)  & 07-01-30 & ARIII &  8.99 &  0.14 &      699 &  0.36 &  0.31 &       67 &  0.30 &  0.28 &       72 &    348.6 $\pm$     6.0 &    414.0 $\pm$    13.1\\
MCG-05-23-016 & VISIR &  076.B-0599(A)  & 06-03-12 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.35 &  0.34 &       55 &  0.35 &  0.34 &      104 &    572.0 $\pm$     9.3 &    572.5 $\pm$    10.3\\
MCG-05-23-016 & VISIR &  078.B-0303(A)  & 07-01-30 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.38 &  0.35 &       50 &  0.35 &  0.33 &       70 &    638.2 $\pm$    16.5 &    706.8 $\pm$    36.9\\
MCG-05-23-016 & VISIR &  078.B-0303(A)  & 07-01-30 & Q1 & 17.65 &  0.83 &      684 &  0.47 &  0.45 &       78 &  0.48 &  0.46 &       52 &   1456.7 $\pm$    60.6 &   1391.1 $\pm$    89.3\\
MCG-05-23-016 & VISIR &  076.B-0599(A)  & 05-12-18 & Q2 & 18.72 &  0.88 &      855 &  0.49 &  0.46 &      104 &  0.50 &  0.48 &      106 &   1456.6 $\pm$    42.4 &   1386.9 $\pm$    31.9\\
MCG-05-23-016 & VISIR &  078.B-0303(A)  & 07-01-30 & PAH1 &  8.59 &  0.42 &       30 &  0.38 &  0.33 &       35 &  0.44 &  0.38 &       21 &    340.1 $\pm$    28.4 &    259.2 $\pm$    42.1\\
MCG-06-30-015 & VISIR &  077.B-0137(A)  & 06-04-14 & NEII\_1 & 12.27 &  0.18 &      180 &  0.35 &  0.33 &       94 &  0.39 &  0.35 &      124 &    371.0 $\pm$    10.3 &    315.1 $\pm$    10.6\\
MCG-06-30-015 & VISIR &  084.B-0366(E)  & 10-03-10 & PAH1 &  8.59 &  0.42 &      362 &  0.26 &  0.24 &      130 &  0.32 &  0.31 &       87 &    239.4 $\pm$    21.0 &    141.0 $\pm$    33.5\\
MCG-06-30-015 & VISIR &  077.B-0137(A)  & 06-04-14 & PAH2 & 11.25 &  0.59 &      181 &  0.33 &  0.31 &       97 &  0.38 &  0.32 &      103 &    357.5 $\pm$    19.1 &    290.1 $\pm$     8.5\\
MCG-06-30-015 & VISIR &  084.B-0366(E)  & 10-03-10 & PAH2\_2 & 11.88 &  0.37 &      362 &  0.33 &  0.33 &      124 &  0.36 &  0.34 &       93 &    346.8 $\pm$    22.3 &    304.1 $\pm$    69.5\\
MCG-06-30-015 & VISIR &  077.B-0137(A)  & 06-04-14 & SIV & 10.49 &  0.16 &      176 &  0.32 &  0.29 &      107 &  0.37 &  0.30 &      112 &    315.0 $\pm$     9.0 &    265.7 $\pm$    14.3\\
MR2251-178 & VISIR &  084.B-0606(A)  & 09-09-20 & NEII\_2 & 13.04 &  0.22 &      360 &  0.37 &  0.35 &      116 &  0.49 &  0.39 &       89 &     90.5 $\pm$    10.7 &     60.0 $\pm$    10.2\\
MR2251-178 & VISIR &  084.B-0606(A)  & 09-09-20 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.33 &  0.32 &       78 &  0.53 &  0.40 &       58 &     90.6 $\pm$     3.3 &     46.6 $\pm$     3.3\\
MR2251-178 & VISIR &  084.B-0606(A)  & 09-09-20 & SIV\_2 & 10.77 &  0.19 &      362 &  0.31 &  0.29 &       53 &  0.55 &  0.38 &       39 &     92.2 $\pm$     2.0 &     36.7 $\pm$     6.6\\
Mrk0003 & MICHELLE &  GN-2009B-Q-61  & 10-02-06 & Si-5 & 11.60 &  0.55 &        4 &  0.48 &  0.41 &      173 &  0.65 &  0.41 &       69 &    518.7 $\pm$    20.9 &    376.7 $\pm$    20.7\\
Mrk0266NE & COMICS &  o09102  & 09-04-07 & N8.8 &  8.75 &  0.38 &      802 &  0.72 &  0.55 &      138 &  1.00 &  1.00 &      127 &     21.9 $\pm$     1.7 &      8.8 $\pm$     0.8\\
Mrk0266SW & COMICS &  o09102  & 09-04-07 & N8.8 &  8.75 &  0.38 &      802 &  0.72 &  0.55 &      138 &  1.00 &  1.00 &       13 &     54.8 $\pm$     5.1 &      5.3 $\pm$     0.5\\
Mrk0304 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     2006 &  0.40 &  0.37 &      168 &  0.58 &  0.54 &        2 &     98.0 $\pm$     7.2 &     47.5 $\pm$     3.3\\
Mrk0509 & VISIR &  077.B-0137(A)  & 06-06-14 & NEII & 12.81 &  0.21 &      179 &  0.42 &  0.40 &      103 &  0.39 &  0.37 &      100 &    256.4 $\pm$    13.5 &    300.8 $\pm$    18.0\\
Mrk0509 & VISIR &  077.B-0137(A)  & 06-06-14 & PAH2 & 11.25 &  0.59 &      181 &  0.42 &  0.38 &      113 &  0.39 &  0.34 &       95 &    232.6 $\pm$     8.3 &    282.4 $\pm$    22.9\\
Mrk0509 & TRECS &  GS-2010B-Q-71  & 10-08-19 & Qa & 18.30 &  0.76 &      318 &  0.56 &  0.54 &        4 &  0.63 &  0.52 &       61 &    462.7 $\pm$    25.3 &    430.2 $\pm$    24.8\\
Mrk0509 & TRECS &  GS-2008B-Q-46  & 08-11-09 & Si2 &  8.74 &  0.39 &      463 &  0.39 &  0.33 &      118 &  0.39 &  0.34 &      134 &    150.1 $\pm$     3.0 &    144.1 $\pm$     3.0\\
Mrk0509 & TRECS &  GS-2010B-Q-71  & 10-08-19 & Si2 &  8.74 &  0.39 &      144 &  0.43 &  0.41 &      142 &  0.53 &  0.42 &       82 &    158.6 $\pm$     4.2 &    120.0 $\pm$     4.0\\
Mrk0509 & TRECS &  GS-2008B-Q-46  & 08-11-09 & Si5 & 11.66 &  0.57 &      289 &  0.44 &  0.39 &      120 &  0.45 &  0.41 &      109 &    233.4 $\pm$     4.1 &    216.5 $\pm$     4.0\\
Mrk0509 & VISIR &  077.B-0137(A)  & 06-06-14 & SIV & 10.49 &  0.16 &      176 &  0.50 &  0.45 &      116 &  0.40 &  0.35 &      109 &    206.0 $\pm$    11.0 &    335.9 $\pm$    25.3\\
Mrk0520 & VISIR &  084.B-0606(A)  & 09-09-19 & NEII & 12.81 &  0.21 &      897 &  0.38 &  0.36 &      135 &  0.45 &  0.42 &      165 &    111.6 $\pm$     7.2 &     77.8 $\pm$     2.9\\
Mrk0520 & VISIR &  084.B-0606(A)  & 09-09-19 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.37 &  0.34 &      171 &  0.44 &  0.42 &       26 &     89.8 $\pm$     4.2 &     63.0 $\pm$     9.3\\
Mrk0520 & VISIR &  084.B-0606(A)  & 09-09-19 & SIV & 10.49 &  0.16 &      529 &  0.39 &  0.36 &      155 &  0.42 &  0.38 &       23 &     58.0 $\pm$     8.9 &     51.0 $\pm$     6.8\\
Mrk0573 & TRECS &  GS-2003B-DD-4  & 03-12-07 & N & 10.36 &  2.64 &      434 &  $\dots$  &  $\dots$  &  $\dots$  &  0.56 &  0.54 &      136 &    194.2 $\pm$    33.8 &  $\le$   294.6  \\
Mrk0573 & TRECS &  GS-2003B-DD-4  & 03-12-07 & Qa & 18.30 &  0.76 &      434 &  $\dots$  &  $\dots$  &  $\dots$  &  0.71 &  0.62 &      106 &    271.5 $\pm$    50.2 &  $\le$   426.3  \\
Mrk0590 & VISIR &  077.B-0137(A)  & 06-08-17 & NEII & 12.81 &  0.21 &      179 &  0.35 &  0.34 &      103 &  0.37 &  0.32 &      107 &    109.2 $\pm$     8.5 &    106.6 $\pm$     4.4\\
Mrk0590 & VISIR &  077.B-0137(A)  & 06-08-17 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.30 &       90 &  0.34 &  0.32 &      152 &     86.3 $\pm$     6.1 &     77.0 $\pm$     3.3\\
Mrk0590 & VISIR &  077.B-0137(A)  & 06-08-17 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.29 &       99 &  0.31 &  0.29 &      138 &     79.0 $\pm$     1.3 &     73.7 $\pm$    14.1\\
Mrk0841 & VISIR &  084.B-0606(A)  & 10-04-01 & NEII & 12.81 &  0.21 &      360 &  0.37 &  0.34 &      120 &  0.40 &  0.37 &      131 &    193.2 $\pm$     2.5 &    163.0 $\pm$     4.4\\
Mrk0841 & VISIR &  084.B-0606(A)  & 10-04-01 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.34 &  0.31 &      149 &  0.37 &  0.36 &       10 &    163.6 $\pm$    10.4 &    133.4 $\pm$     1.1\\
Mrk0841 & VISIR &  084.B-0606(A)  & 10-04-01 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.29 &      158 &  0.34 &  0.32 &      143 &    128.4 $\pm$     8.4 &    106.5 $\pm$     6.1\\
Mrk0897 & TRECS &  GS-2004A-Q-14  & 04-07-30 & N & 10.36 &  2.64 &      716 &  0.41 &  0.37 &      171 &  1.00 &  1.00 &      139 &     28.0 $\pm$     1.2 &      6.3 $\pm$     1.1\\
Mrk0915 & TRECS &  GS-2007A-DD-7  & 07-06-28 & Qa & 18.30 &  0.76 &      847 &  0.57 &  0.53 &       99 &  0.64 &  0.57 &       14 &    201.4 $\pm$    16.0 &    169.6 $\pm$    15.8\\
Mrk0926 & VISIR &  084.B-0606(A)  & 09-09-20 & NEII & 12.81 &  0.21 &      358 &  0.36 &  0.33 &       92 &  0.47 &  0.41 &       85 &    132.5 $\pm$     0.6 &     82.5 $\pm$     0.9\\
Mrk0926 & VISIR &  084.B-0606(A)  & 09-09-20 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.33 &  0.32 &       78 &  0.42 &  0.36 &       59 &    125.7 $\pm$     0.9 &     86.0 $\pm$     1.1\\
Mrk0926 & VISIR &  084.B-0606(A)  & 09-09-20 & SIV\_2 & 10.77 &  0.19 &      362 &  0.31 &  0.29 &       53 &  0.46 &  0.39 &       56 &    113.6 $\pm$     3.9 &     58.1 $\pm$     1.8\\
Mrk0937 & VISIR &  077.B-0137(A)  & 06-07-13 & NEII & 12.81 &  0.21 &      717 &  0.42 &  0.34 &      120 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    21.2   &  $\le$    21.2  \\
Mrk0937 & VISIR &  077.B-0137(A)  & 06-07-10 & SIV & 10.49 &  0.16 &      176 &  0.30 &  0.29 &       83 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.0   &  $\le$    13.0  \\
Mrk1014 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     1605 &  0.41 &  0.38 &      162 &  0.58 &  0.50 &       63 &    101.5 $\pm$     8.2 &     56.0 $\pm$    10.8\\
Mrk1018 & VISIR &  382.A-0604(A)  & 09-08-13 & B10.7 & 10.65 &  1.37 &      115 &  0.34 &  0.31 &       96 &  0.31 &  0.30 &      104 &     57.2 $\pm$     8.8 &     61.5 $\pm$     3.6\\
Mrk1018 & VISIR &  382.A-0604(A)  & 09-08-13 & B11.7 & 11.52 &  0.85 &      112 &  0.36 &  0.33 &      102 &  0.35 &  0.30 &      103 &     62.7 $\pm$     6.8 &     69.0 $\pm$     5.7\\
Mrk1018 & VISIR &  382.A-0604(A)  & 09-08-13 & B12.4 & 12.47 &  0.99 &      176 &  0.38 &  0.33 &      102 &  0.36 &  0.33 &      106 &     60.8 $\pm$     7.0 &     64.4 $\pm$     7.0\\
Mrk1018 & VISIR &  382.A-0604(A)  & 09-08-13 & B9.7 &  9.82 &  0.84 &      176 &  0.35 &  0.33 &       96 &  0.32 &  0.27 &       77 &     51.7 $\pm$     2.5 &     69.3 $\pm$    12.1\\
Mrk1018 & VISIR &  382.A-0604(A)  & 09-08-13 & J7.9 &  7.76 &  0.55 &      338 &  0.34 &  0.29 &      152 &  0.34 &  0.27 &       77 &     38.7 $\pm$     8.6 &     41.9 $\pm$     8.6\\
Mrk1239 & VISIR &  60.A-9244(A)  & 05-01-28 & PAH2 & 11.25 &  0.59 &     1059 &  0.38 &  0.37 &      116 &  0.39 &  0.36 &      149 &    695.2 $\pm$    21.7 &    660.2 $\pm$    55.4\\
Mrk1239 & VISIR &  077.B-0728(A)  & 06-04-28 & PAH2\_2 & 11.88 &  0.37 &      543 &  0.32 &  0.31 &       82 &  0.35 &  0.32 &       85 &    606.0 $\pm$    19.6 &    542.5 $\pm$    30.2\\
Mrk1239 & VISIR &  077.B-0728(A)  & 06-05-16 & Q2 & 18.72 &  0.88 &      993 &  0.48 &  0.47 &      131 &  0.48 &  0.46 &      109 &    918.1 $\pm$    39.3 &    914.7 $\pm$    38.5\\
NGC0034 & TRECS &  GS-2008B-Q-63  & 08-11-10 & Si5 & 11.66 &  0.57 &     2085 &  0.41 &  0.38 &      159 &  0.71 &  0.61 &      173 &    218.8 $\pm$     3.2 &     57.8 $\pm$     2.6\\
NGC0235A & VISIR &  084.B-0606(A)  & 09-09-30 & NEII & 12.81 &  0.21 &      179 &  0.39 &  0.37 &      175 &  0.56 &  0.43 &       69 &     91.4 $\pm$    13.6 &     54.9 $\pm$    13.6\\
NGC0235A & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.35 &       49 &  0.59 &  0.45 &       85 &     63.4 $\pm$     8.3 &     31.1 $\pm$     8.2\\
NGC0235A & VISIR &  084.B-0606(A)  & 09-09-30 & SIV & 10.49 &  0.16 &      176 &  0.35 &  0.33 &        7 &  0.51 &  0.41 &      151 &     38.8 $\pm$     7.8 &     21.9 $\pm$     7.8\\
NGC0253 & VISIR &  074.A-9016(A)  & 04-12-01 & PAH2 & 11.25 &  0.59 &     1413 &  0.36 &  0.35 &       60 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  1523.6   &  $\le$   919.1  \\
NGC0253 & VISIR &  074.A-9016(A)  & 04-12-01 & PAH2\_2 & 11.88 &  0.37 &     1413 &  0.37 &  0.35 &       68 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  1238.2   &  $\le$   453.0  \\
NGC0253 & VISIR &  076.B-0656(A)  & 05-10-09 & Q2 & 18.72 &  0.88 &     3118 &  0.53 &  0.51 &      175 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  4748.0   &  $\le$  2093.3  \\
NGC0253 & VISIR &  075.B-0182(A)  & 05-07-20 & SIV\_1 &  9.82 &  0.18 &     1448 &  0.52 &  0.41 &       30 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  1200.3   &  $\le$   500.9  \\
NGC0424 & TRECS &  GS-2003B-Q-44  & 03-12-02 & N & 10.36 &  2.64 &      608 &  0.34 &  0.33 &       96 &  0.45 &  0.36 &       79 &    792.2 $\pm$    12.4 &    545.6 $\pm$    11.0\\
NGC0454E & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_1 & 12.27 &  0.18 &      721 &  0.43 &  0.40 &       10 &  0.49 &  0.41 &      115 &    152.4 $\pm$    12.5 &    122.1 $\pm$     5.7\\
NGC0454E & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.35 &       49 &  0.48 &  0.37 &      121 &     98.1 $\pm$    10.5 &     72.7 $\pm$     4.8\\
NGC0454E & VISIR &  084.B-0606(A)  & 09-09-30 & SIV\_2 & 10.77 &  0.19 &     1267 &  0.37 &  0.34 &      171 &  0.46 &  0.38 &      125 &     97.0 $\pm$     7.0 &     67.7 $\pm$     2.6\\
NGC0526A & VISIR &  075.B-0844(C)  & 05-07-20 & NEII\_1 & 12.27 &  0.18 &      543 &  0.53 &  0.36 &      148 &  0.39 &  0.36 &      142 &    236.4 $\pm$    17.4 &    331.8 $\pm$    34.3\\
NGC0526A & VISIR &  075.B-0844(C)  & 05-07-20 & SIV & 10.49 &  0.16 &      717 &  0.56 &  0.42 &      148 &  0.34 &  0.32 &      123 &    180.6 $\pm$     3.3 &    394.6 $\pm$    14.2\\
NGC0612 & VISIR &  084.B-0606(A)  & 09-09-28 & NEII & 12.81 &  0.21 &      179 &  0.46 &  0.43 &       82 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    55.2   &  $\le$    55.2  \\
NGC0612 & VISIR &  084.B-0606(A)  & 09-09-28 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.45 &  0.42 &       95 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    26.4   &  $\le$    26.4  \\
NGC0612 & VISIR &  084.B-0606(A)  & 09-09-28 & SIV & 10.49 &  0.16 &      176 &  0.45 &  0.38 &      132 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    30.9   &  $\le$    30.9  \\
NGC0613 & TRECS &  GS-2010B-Q-3  & 10-08-19 & N & 10.36 &  2.64 &      318 &  0.37 &  0.36 &       96 &  0.41 &  0.37 &      146 &     22.3 $\pm$     2.3 &     19.3 $\pm$     2.3\\
NGC0676 & VISIR &  083.B-0536(C)  & 09-07-06 & NEII\_1 & 12.27 &  0.18 &      360 &  0.33 &  0.32 &      102 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    17.8   &  $\le$    17.8  \\
NGC0676 & VISIR &  083.B-0536(C)  & 09-07-06 & PAH2 & 11.25 &  0.59 &      181 &  0.31 &  0.29 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    11.0   &  $\le$    11.0  \\
NGC0676 & VISIR &  086.B-0349(C)  & 10-12-23 & PAH2 & 11.25 &  0.59 &      905 &  0.34 &  0.32 &      141 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    20.8   &     14.9 $\pm$     0.0\\
NGC0676 & VISIR &  086.B-0349(C)  & 10-12-25 & PAH2 & 11.25 &  0.59 &      543 &  0.31 &  0.30 &       97 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    21.0   &     20.7 $\pm$     0.0\\
NGC0676 & VISIR &  086.B-0349(C)  & 10-12-23 & PAH2\_2 & 11.88 &  0.37 &      905 &  0.34 &  0.33 &      130 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    16.5   &     23.4 $\pm$     0.0\\
NGC0676 & VISIR &  086.B-0349(C)  & 10-12-25 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.34 &  0.32 &      137 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.6   &  $\le$    10.6  \\
NGC0788 & VISIR &  382.A-0604(A)  & 08-09-19 & B10.7 & 10.65 &  1.37 &      115 &  0.50 &  0.48 &       24 &  0.47 &  0.45 &        4 &    109.1 $\pm$     9.1 &    126.5 $\pm$     9.1\\
NGC0788 & VISIR &  382.A-0604(A)  & 08-09-19 & B11.7 & 11.52 &  0.85 &      114 &  0.47 &  0.43 &       23 &  0.49 &  0.47 &       72 &    130.9 $\pm$     8.9 &    115.7 $\pm$     8.9\\
NGC0788 & VISIR &  382.A-0604(A)  & 08-09-19 & B12.4 & 12.47 &  0.99 &      176 &  0.41 &  0.40 &      155 &  0.49 &  0.46 &       67 &    140.2 $\pm$    13.5 &    106.3 $\pm$     6.6\\
NGC0788 & VISIR &  382.A-0604(A)  & 08-09-19 & B9.7 &  9.82 &  0.84 &      176 &  0.62 &  0.58 &       29 &  0.45 &  0.40 &       43 &     87.4 $\pm$    17.2 &    176.6 $\pm$    42.5\\
NGC0788 & VISIR &  382.A-0604(A)  & 08-09-19 & J7.9 &  7.76 &  0.55 &      338 &  0.35 &  0.31 &       50 &  0.33 &  0.28 &        5 &     65.6 $\pm$     9.2 &     77.5 $\pm$    10.5\\
NGC0985 & VISIR &  382.A-0604(A)  & 08-09-19 & B10.7 & 10.65 &  1.37 &      115 &  0.41 &  0.39 &       32 &  0.44 &  0.36 &       96 &    164.7 $\pm$    29.6 &    179.8 $\pm$    34.0\\
NGC0985 & VISIR &  382.A-0604(A)  & 08-09-19 & B11.7 & 11.52 &  0.85 &      114 &  0.42 &  0.39 &      165 &  0.37 &  0.33 &       91 &    177.9 $\pm$    10.9 &    238.6 $\pm$    18.1\\
NGC0985 & VISIR &  382.A-0604(A)  & 08-09-19 & B12.4 & 12.47 &  0.99 &      176 &  0.41 &  0.40 &      155 &  0.38 &  0.35 &       93 &    180.1 $\pm$    21.3 &    228.4 $\pm$    11.5\\
NGC0985 & VISIR &  382.A-0604(A)  & 08-09-19 & B9.7 &  9.82 &  0.84 &      176 &  0.39 &  0.36 &       91 &  0.54 &  0.46 &       86 &    172.3 $\pm$    14.0 &     97.5 $\pm$    13.8\\
NGC0985 & VISIR &  382.A-0604(A)  & 08-09-19 & J7.9 &  7.76 &  0.55 &      338 &  0.62 &  0.57 &        9 &  0.40 &  0.40 &       34 &     92.3 $\pm$     7.6 &    220.9 $\pm$    47.3\\
NGC1052 & VISIR &  382.A-0604(A)  & 09-09-06 & B10.7 & 10.65 &  1.37 &      724 &  0.36 &  0.34 &      116 &  0.43 &  0.37 &       75 &    133.7 $\pm$    22.8 &    104.9 $\pm$    12.6\\
NGC1052 & VISIR &  382.A-0604(A)  & 09-09-06 & B11.7 & 11.52 &  0.85 &      360 &  0.43 &  0.40 &      115 &  0.44 &  0.40 &       88 &    154.1 $\pm$    13.2 &    147.4 $\pm$     5.7\\
NGC1052 & VISIR &  382.A-0604(A)  & 09-09-06 & B12.4 & 12.47 &  0.99 &      362 &  0.41 &  0.37 &      108 &  0.51 &  0.42 &       82 &    181.2 $\pm$    19.8 &    128.0 $\pm$     8.6\\
NGC1052 & VISIR &  382.A-0604(A)  & 09-09-06 & B9.7 &  9.82 &  0.84 &      724 &  0.36 &  0.35 &      133 &  0.39 &  0.35 &      167 &    114.7 $\pm$    22.9 &    105.7 $\pm$    12.9\\
NGC1052 & VISIR &  382.A-0604(A)  & 09-09-06 & J7.9 &  7.76 &  0.55 &     1442 &  0.45 &  0.39 &      111 &  0.52 &  0.39 &      154 &     58.8 $\pm$     9.4 &     51.6 $\pm$     5.7\\
NGC1052 & VISIR &  384.B-0943(A)  & 09-10-22 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.66 &  0.52 &      122 &  0.40 &  0.36 &       61 &    133.9 $\pm$     4.2 &    319.8 $\pm$    11.7\\
NGC1052 & VISIR &  086.B-0349(D)  & 10-10-21 & Q2 & 18.72 &  0.88 &      496 &  0.53 &  0.49 &      131 &  0.50 &  0.49 &      118 &    339.0 $\pm$    33.8 &    352.0 $\pm$    15.7\\
NGC1052 & TRECS &  GS-2007B-Q-203  & 07-08-20 & Qa & 18.30 &  0.76 &      926 &  0.53 &  0.53 &       47 &  0.55 &  0.52 &       37 &    355.7 $\pm$     9.1 &    348.5 $\pm$     9.1\\
NGC1052 & TRECS &  GS-2007B-Q-203  & 07-08-17 & Si2 &  8.74 &  0.39 &      926 &  0.62 &  0.56 &       16 &  0.75 &  0.62 &       17 &     63.6 $\pm$     1.6 &     47.2 $\pm$     1.5\\
NGC1052 & VISIR &  086.B-0349(B)  & 10-10-21 & PAH1 &  8.59 &  0.42 &      112 &  0.34 &  0.31 &      138 &  0.45 &  0.39 &      115 &     62.4 $\pm$    14.4 &     37.0 $\pm$     5.3\\
NGC1068 & VISIR &  076.B-0743(F)  & 05-11-15 & ARIII &  8.99 &  0.14 &      690 &  0.36 &  0.34 &       99 &  0.66 &  0.40 &      173 &  17753.2 $\pm$   469.0 &   5690.6 $\pm$   454.3\\
NGC1068 & VISIR &  076.B-0743(F)  & 05-11-15 & NEII & 12.81 &  0.21 &      721 &  0.40 &  0.39 &      119 &  0.70 &  0.40 &      174 &  36540.5 $\pm$  1317.6 &  14429.6 $\pm$  1078.7\\
NGC1068 & VISIR &  60.A-9242(A)  & 04-09-29 & NEII\_1 & 12.27 &  0.18 &     3575 &  0.41 &  0.37 &      109 &  0.67 &  0.40 &      173 &  31801.9 $\pm$   822.7 &  12536.8 $\pm$   773.8\\
NGC1068 & VISIR &  076.B-0743(F)  & 05-11-15 & NEII\_2 & 13.04 &  0.22 &      724 &  0.38 &  0.35 &       97 &  0.72 &  0.41 &      173 &  35152.8 $\pm$  1403.4 &  12177.2 $\pm$  1015.0\\
NGC1068 & VISIR &  076.B-0743(F)  & 05-11-15 & PAH1 &  8.59 &  0.42 &      721 &  0.39 &  0.37 &      113 &  0.65 &  0.43 &      173 &  18523.9 $\pm$   657.0 &   6714.5 $\pm$   462.7\\
NGC1068 & VISIR & 076.B-0743(F) & 05-11-22 & PAH2 & 11.25 &  0.59 &      724 &  0.36 &  0.34 &       31 &  0.77 &  0.49 &      178 &  29233.0 $\pm$   653.8 &   9203.2 $\pm$   614.8\\
NGC1068 & VISIR & 382.B-0732(A) & 08-08-24 & Q1 & 17.65 &  0.83 &      171 &  0.52 &  0.49 &       97 &  0.90 &  0.57 &      179 &  57602.3 $\pm$  1243.6 &  20126.2 $\pm$   368.2\\
NGC1068 & VISIR & 60.A-9242(A) & 04-09-27 & Q2 & 18.72 &  0.88 &     1828 &  0.51 &  0.51 &      157 &  0.96 &  0.68 &      173 &  66926.4 $\pm$  2030.0 &  18783.9 $\pm$  1401.1\\
NGC1068 & VISIR & 382.B-0732(A) & 08-08-24 & Q3 & 19.50 &  0.40 &      174 &  0.54 &  0.52 &      135 &  0.93 &  0.62 &        0 &  57472.4 $\pm$  1662.9 &  19609.0 $\pm$   696.2\\
NGC1068 & VISIR & 076.B-0743(F) & 05-11-15 & SIC & 11.85 &  2.34 &      358 &  0.35 &  0.31 &       99 &  0.74 &  0.47 &      173 &  31758.4 $\pm$  1789.8 &  10104.6 $\pm$   966.9\\
NGC1068 & VISIR & 076.B-0743(F) & 05-11-22 & SIV\_2 & 10.77 &  0.19 &      724 &  0.34 &  0.32 &       67 &  0.76 &  0.47 &        0 &  26832.0 $\pm$   773.3 &   8279.0 $\pm$   648.5\\
NGC1097 & VISIR &  077.B-0137(A)  & 06-08-07 & NEII\_1 & 12.27 &  0.18 &     2524 &  0.34 &  0.32 &      118 &  0.43 &  0.39 &      169 &     27.9 $\pm$     3.1 &     18.7 $\pm$     1.8\\
NGC1097 & VISIR &  085.B-0639(C)  & 10-07-12 & PAH1 &  8.59 &  0.42 &      360 &  0.35 &  0.31 &       89 &  $\dots$  &  $\dots$  &  $\dots$  &     14.7 $\pm$     0.8 &     14.6 $\pm$     0.8\\
NGC1097 & VISIR &  083.B-0536(A)  & 09-07-15 & PAH2 & 11.25 &  0.59 &     1993 &  0.43 &  0.38 &       73 &  0.53 &  0.45 &       77 &     29.1 $\pm$     7.5 &     19.6 $\pm$     4.2\\
NGC1097 & VISIR &  076.B-0656(A)  & 05-10-09 & PAH2 & 11.25 &  0.59 &      883 &  0.39 &  0.36 &      164 &  0.61 &  0.54 &       92 &     30.3 $\pm$     5.1 &     13.0 $\pm$     5.1\\
NGC1097 & VISIR &  077.B-0728(A)  & 06-09-04 & PAH2\_2 & 11.88 &  0.37 &     2527 &  0.34 &  0.32 &       77 &  0.40 &  0.34 &       81 &     17.5 $\pm$     0.9 &     16.4 $\pm$     0.5\\
NGC1097 & VISIR &  076.B-0656(A)  & 05-10-09 & PAH2\_2 & 11.88 &  0.37 &      883 &  0.43 &  0.41 &      103 &  0.52 &  0.40 &       22 &     22.4 $\pm$     3.7 &     18.4 $\pm$     3.7\\
NGC1097 & VISIR &  077.B-0728(A)  & 06-09-05 & Q2 & 18.72 &  0.88 &     1987 &  0.48 &  0.47 &       77 &  0.55 &  0.49 &      135 &     54.2 $\pm$     9.0 &     45.2 $\pm$     9.0\\
NGC1097 & TRECS &  GS-2005B-Q-29  & 05-09-16 & Qa & 18.30 &  0.76 &      912 &  0.55 &  0.52 &      120 &  0.52 &  0.48 &       55 &     47.4 $\pm$    11.2 &     54.1 $\pm$    11.3\\
NGC1097 & TRECS &  GS-2005B-Q-29  & 05-09-17 & Si5 & 11.66 &  0.57 &      456 &  0.43 &  0.41 &       99 &  0.48 &  0.46 &       66 &     26.5 $\pm$     1.9 &     20.7 $\pm$     1.9\\
NGC1097 & VISIR &  085.B-0639(C)  & 10-07-12 & SIV\_2 & 10.77 &  0.19 &      724 &  0.40 &  0.35 &       85 &  0.47 &  0.38 &       88 &     26.8 $\pm$     9.0 &     21.0 $\pm$     1.1\\
NGC1144 & VISIR &  382.A-0604(A)  & 09-08-20 & B10.7 & 10.65 &  1.37 &      115 &  0.39 &  0.34 &       77 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    26.5   &  $\le$    26.5  \\
NGC1144 & VISIR &  382.A-0604(A)  & 09-08-20 & B11.7 & 11.52 &  0.85 &      112 &  0.42 &  0.34 &       79 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    26.0   &  $\le$    26.0  \\
NGC1144 & VISIR &  382.A-0604(A)  & 09-09-10 & B12.4 & 12.47 &  0.99 &      529 &  0.36 &  0.34 &      126 &  0.46 &  0.42 &       86 &     39.8 $\pm$    11.5 &     23.5 $\pm$     6.1\\
NGC1144 & VISIR &  382.A-0604(A)  & 09-09-10 & B9.7 &  9.82 &  0.84 &      529 &  0.32 &  0.30 &      119 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    11.3   &  $\le$    11.3  \\
NGC1144 & VISIR &  382.A-0604(A)  & 09-08-20 & J7.9 &  7.76 &  0.55 &      338 &  0.32 &  0.31 &       54 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    26.7   &  $\le$    26.7  \\
NGC1144 & VISIR &  084.B-0606(A)  & 09-10-06 & NEII & 12.81 &  0.21 &      358 &  0.38 &  0.36 &       99 &  $\dots$  &  $\dots$  &  $\dots$  &     44.2 $\pm$     3.3 &     44.2 $\pm$     3.3\\
NGC1144 & VISIR &  084.B-0606(A)  & 09-10-06 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.39 &  0.37 &       59 &  0.39 &  0.30 &      107 &     23.1 $\pm$     1.0 &     28.0 $\pm$     2.8\\
NGC1144 & VISIR &  084.B-0606(A)  & 09-10-06 & SIV & 10.49 &  0.16 &      353 &  0.40 &  0.36 &       42 &  $\dots$  &  $\dots$  &  $\dots$  &     11.3 $\pm$     1.0 &     11.3 $\pm$     1.0\\
NGC1194 & VISIR &  382.A-0604(A)  & 09-08-20 & B10.7 & 10.65 &  1.37 &      115 &  0.39 &  0.34 &       77 &  0.36 &  0.34 &       76 &    127.3 $\pm$     5.1 &    136.2 $\pm$    11.7\\
NGC1194 & VISIR &  382.A-0604(A)  & 09-08-20 & B11.7 & 11.52 &  0.85 &      112 &  0.42 &  0.34 &       79 &  0.39 &  0.36 &       83 &    190.4 $\pm$    14.0 &    198.8 $\pm$    10.7\\
NGC1194 & VISIR &  382.A-0604(A)  & 09-08-20 & B12.4 & 12.47 &  0.99 &      176 &  0.42 &  0.35 &       80 &  0.40 &  0.35 &       96 &    265.3 $\pm$    24.3 &    274.1 $\pm$    10.5\\
NGC1194 & VISIR &  382.A-0604(A)  & 09-08-20 & B9.7 &  9.82 &  0.84 &      176 &  0.43 &  0.33 &       80 &  0.37 &  0.34 &       80 &    109.2 $\pm$    12.4 &    125.6 $\pm$     5.3\\
NGC1194 & VISIR &  382.A-0604(A)  & 09-08-20 & J7.9 &  7.76 &  0.55 &      338 &  0.32 &  0.31 &       54 &  0.32 &  0.30 &      178 &    169.1 $\pm$    18.0 &    172.0 $\pm$    21.1\\
NGC1275 & COMICS &  o09108  & 09-07-14 & N11.7 & 11.74 &  0.53 &      401 &  0.65 &  0.40 &       84 &  0.73 &  0.62 &       68 &    918.7 $\pm$    54.0 &    534.0 $\pm$    55.3\\
NGC1275 & COMICS &  o09108  & 09-07-14 & NeII & 12.81 &  0.10 &      401 &  1.00 &  0.86 &      103 &  1.00 &  0.76 &       70 &   1208.4 $\pm$    60.9 &   1346.2 $\pm$   114.8\\
NGC1275 & MICHELLE &  GN-2006B-Q-19  & 06-09-10 & Si-2 &  8.80 &  0.45 &      414 &  0.36 &  0.32 &       39 &  0.43 &  0.35 &       25 &    313.6 $\pm$     4.7 &    242.8 $\pm$     4.2\\
NGC1275 & MICHELLE &  GN-2006B-Q-19  & 06-09-10 & Si-6 & 12.50 &  0.60 &      376 &  0.42 &  0.38 &       48 &  0.43 &  0.37 &       25 &    886.4 $\pm$    11.4 &    892.7 $\pm$    11.4\\
NGC1365 & VISIR &  074.A-9016(A)  & 04-12-01 & NEII & 12.81 &  0.21 &      897 &  0.34 &  0.34 &       86 &  0.61 &  0.39 &       99 &    597.7 $\pm$    16.7 &    289.4 $\pm$    15.3\\
NGC1365 & VISIR &  074.A-9016(A)  & 04-12-02 & NEII & 12.81 &  0.21 &     2667 &  0.39 &  0.36 &       89 &  0.52 &  0.40 &       48 &    640.1 $\pm$    20.3 &    392.0 $\pm$    30.4\\
NGC1365 & VISIR &  084.B-0606(A)  & 09-09-28 & NEII\_1 & 12.27 &  0.18 &      180 &  0.43 &  0.40 &      101 &  0.48 &  0.40 &       97 &    490.9 $\pm$    27.0 &    439.4 $\pm$    37.4\\
NGC1365 & VISIR &  084.B-0606(A)  & 09-09-28 & NEII\_2 & 13.04 &  0.22 &      180 &  0.43 &  0.40 &       98 &  0.48 &  0.40 &      101 &    501.5 $\pm$    11.1 &    445.7 $\pm$     9.3\\
NGC1365 & VISIR &  084.B-0606(A)  & 09-09-28 & PAH2 & 11.25 &  0.59 &      181 &  0.42 &  0.41 &      140 &  0.42 &  0.38 &       91 &    422.6 $\pm$     7.8 &    452.1 $\pm$    10.8\\
NGC1386 & TRECS &  GS-2003B-DD-4  & 03-12-06 & N & 10.36 &  2.64 &      434 &  $\dots$  &  $\dots$  &  $\dots$  &  0.54 &  0.38 &        2 &    256.8 $\pm$    44.7 &  $\le$   391.1  \\
NGC1386 & VISIR &  085.B-0639(C)  & 10-07-18 & PAH1 &  8.59 &  0.42 &       62 &  0.64 &  0.46 &       87 &  0.75 &  0.68 &      117 &    208.0 $\pm$    12.1 &     89.0 $\pm$     7.0\\
NGC1386 & VISIR &  077.B-0728(A)  & 06-08-17 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.39 &  0.33 &      115 &  0.50 &  0.35 &        1 &    377.2 $\pm$    11.7 &    210.9 $\pm$    10.6\\
NGC1386 & VISIR &  077.B-0728(A)  & 06-08-09 & Q2 & 18.72 &  0.88 &      993 &  0.56 &  0.54 &       65 &  0.67 &  0.52 &        0 &    648.0 $\pm$   145.0 &    428.9 $\pm$    83.9\\
NGC1386 & VISIR &  077.B-0728(A)  & 06-08-16 & Q2 & 18.72 &  0.88 &      993 &  0.56 &  0.52 &      138 &  0.71 &  0.56 &      177 &    778.7 $\pm$    43.2 &    426.8 $\pm$    10.8\\
NGC1386 & TRECS &  GS-2003B-DD-4  & 03-12-06 & Qa & 18.30 &  0.76 &      434 &  $\dots$  &  $\dots$  &  $\dots$  &  0.70 &  0.51 &      178 &    373.2 $\pm$    68.8 &  $\le$   594.2  \\
NGC1386 & VISIR &  085.B-0639(C)  & 10-07-18 & SIV\_2 & 10.77 &  0.19 &      188 &  0.76 &  0.63 &       99 &  0.80 &  0.71 &       92 &    302.5 $\pm$    15.4 &    208.0 $\pm$    28.0\\
NGC1433 & VISIR &  384.B-0943(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.39 &  0.37 &        1 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.8   &  $\le$    12.8  \\
NGC1433 & TRECS &  GS-2005B-DD-6  & 05-09-18 & Si2 &  8.74 &  0.39 &      304 &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     4.7   &  $\le$     4.7  \\
NGC1553 & VISIR &  384.B-0943(A)  & 09-10-22 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.66 &  0.52 &      122 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    24.7   &  $\le$    24.7  \\
NGC1566 & VISIR &  083.B-0536(A)  & 09-09-07 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.35 &  0.34 &      112 &  0.56 &  0.44 &      126 &    104.1 $\pm$    10.6 &     53.0 $\pm$    12.5\\
NGC1566 & VISIR &  086.B-0349(C)  & 10-11-22 & PAH1 &  8.59 &  0.42 &      180 &  0.27 &  0.25 &      151 &  0.34 &  0.33 &      178 &     40.2 $\pm$     6.2 &     22.3 $\pm$     2.2\\
NGC1566 & VISIR &  083.B-0536(A)  & 09-09-07 & PAH2 & 11.25 &  0.59 &      362 &  0.43 &  0.35 &       98 &  0.58 &  0.46 &      131 &    105.4 $\pm$     9.8 &     59.4 $\pm$     6.2\\
NGC1566 & VISIR &  077.B-0728(A)  & 06-09-05 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.34 &  0.32 &      128 &  0.35 &  0.32 &       46 &     57.0 $\pm$     2.4 &     56.8 $\pm$     6.7\\
NGC1566 & VISIR &  077.B-0728(A)  & 06-09-05 & Q2 & 18.72 &  0.88 &     1159 &  0.48 &  0.47 &       77 &  0.57 &  0.52 &      144 &    147.1 $\pm$    16.2 &    113.2 $\pm$     6.1\\
NGC1566 & TRECS &  GS-2005B-DD-6  & 05-09-18 & Qa & 18.30 &  0.76 &      304 &  $\dots$  &  $\dots$  &  $\dots$  &  0.57 &  0.53 &      150 &    140.7 $\pm$    34.5 &  $\le$   244.2  \\
NGC1566 & TRECS &  GS-2005B-DD-6  & 05-09-18 & Si2 &  8.74 &  0.39 &      304 &  $\dots$  &  $\dots$  &  $\dots$  &  0.52 &  0.47 &      173 &     36.6 $\pm$     3.7 &  $\le$    47.0  \\
NGC1566 & VISIR &  086.B-0349(C)  & 10-11-22 & SIV\_2 & 10.77 &  0.19 &      181 &  0.31 &  0.30 &       69 &  0.36 &  0.34 &      145 &     61.5 $\pm$     1.2 &     47.9 $\pm$     1.1\\
NGC1614 & VISIR &  60.A-9244(A)  & 04-10-02 & PAH2 & 11.25 &  0.59 &     2088 &  0.51 &  0.50 &       90 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   731.4   &  $\le$   200.2  \\
NGC1614 & COMICS &  o07146  & 08-01-24 & Q17.7 & 17.69 &  0.43 &      961 &  0.73 &  0.65 &      162 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  2572.9   &  $\le$  1194.4  \\
NGC1614 & VISIR &  078.B-0173(B)  & 06-10-04 & Q2 & 18.72 &  0.88 &     2079 &  0.49 &  0.48 &      102 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$  2666.3   &  $\le$   654.2  \\
NGC1614 & TRECS &  GS-2006B-Q-9  & 06-09-16 & Si2 &  8.74 &  0.39 &      868 &  0.39 &  0.33 &      136 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   420.3   &  $\le$    65.5  \\
NGC1614 & TRECS &  GS-2006B-Q-9  & 06-09-30 & Si2 &  8.74 &  0.39 &      868 &  0.46 &  0.44 &        1 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   397.7   &  $\le$    89.9  \\
NGC1667 & VISIR &  083.B-0536(A)  & 09-09-07 & NEII\_1 & 12.27 &  0.18 &     1803 &  0.41 &  0.37 &      104 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.4   &  $\le$    13.3  \\
NGC1667 & TRECS &  GS-2004A-Q-14  & 04-10-27 & N & 10.36 &  2.64 &      716 &  0.42 &  0.41 &      153 &  0.52 &  0.43 &       53 &      6.0 $\pm$     1.4 &      4.6 $\pm$     1.4\\
NGC1667 & VISIR &  083.B-0536(A)  & 09-09-07 & PAH2 & 11.25 &  0.59 &      362 &  0.43 &  0.35 &       98 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    21.2   &  $\le$    21.2  \\
NGC1808 & VISIR &  384.B-0943(A)  & 09-10-22 & PAH2\_2 & 11.88 &  0.37 &      722 &  0.66 &  0.52 &      122 &  0.64 &  0.54 &      130 &    411.0 $\pm$    10.5 &    328.8 $\pm$     9.4\\
NGC2110 & VISIR &  078.B-0303(A)  & 06-10-10 & ARIII &  8.99 &  0.14 &      690 &  0.31 &  0.29 &      138 &  0.35 &  0.30 &       90 &    174.0 $\pm$     4.5 &    150.0 $\pm$     9.3\\
NGC2110 & VISIR &  086.B-0479(A)  & 10-10-20 & NEII & 12.81 &  0.21 &     1973 &  0.34 &  0.34 &      128 &  0.36 &  0.35 &      132 &    388.9 $\pm$     6.9 &    357.5 $\pm$    10.5\\
NGC2110 & VISIR &  086.B-0479(A)  & 10-10-20 & NEII\_1 & 12.27 &  0.18 &     1983 &  0.33 &  0.33 &       98 &  0.37 &  0.36 &       93 &    364.7 $\pm$     6.9 &    308.0 $\pm$    11.2\\
NGC2110 & VISIR &  078.B-0303(A)  & 06-10-10 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.38 &  0.35 &      139 &  0.35 &  0.33 &       64 &    295.6 $\pm$     8.1 &    331.8 $\pm$     7.9\\
NGC2110 & VISIR &  078.B-0303(A)  & 06-10-10 & Q1 & 17.65 &  0.83 &      662 &  0.49 &  0.46 &      132 &  0.48 &  0.47 &       82 &    520.9 $\pm$    41.7 &    517.6 $\pm$    10.8\\
NGC2110 & VISIR &  078.B-0303(A)  & 06-10-10 & PAH1 &  8.59 &  0.42 &       62 &  0.35 &  0.31 &      123 &  0.40 &  0.31 &      115 &    162.7 $\pm$    10.3 &    143.4 $\pm$    11.4\\
NGC2110 & MICHELLE &  GN-2007A-Q-49  & 07-03-18 & N\_prime & 11.20 &  1.20 &      188 &  0.65 &  0.53 &       12 &  0.53 &  0.49 &      168 &    312.1 $\pm$     5.6 &    417.3 $\pm$     6.4\\
NGC2623 & COMICS &  o07146  & 08-01-24 & Q17.7 & 17.69 &  0.43 &     2403 &  0.63 &  0.53 &      115 &  0.99 &  0.88 &       51 &    484.4 $\pm$    42.7 &    183.4 $\pm$    12.9\\
NGC2992 & VISIR &  076.B-0468(A)  & 06-02-16 & NEII & 12.81 &  0.21 &     1267 &  0.35 &  0.32 &      103 &  0.38 &  0.38 &       66 &    361.3 $\pm$    12.5 &    277.9 $\pm$     8.9\\
NGC2992 & VISIR &  076.B-0468(A)  & 06-02-17 & NEII & 12.81 &  0.21 &     1267 &  0.36 &  0.35 &      147 &  0.40 &  0.38 &       97 &    364.7 $\pm$    10.1 &    294.9 $\pm$    11.3\\
NGC2992 & VISIR &  076.B-0468(A)  & 06-02-16 & NEII\_1 & 12.27 &  0.18 &     1263 &  0.33 &  0.31 &       99 &  0.36 &  0.34 &       12 &    277.7 $\pm$    12.9 &    236.2 $\pm$    13.6\\
NGC2992 & VISIR &  076.B-0468(A)  & 06-02-17 & NEII\_1 & 12.27 &  0.18 &     1267 &  0.35 &  0.34 &      147 &  0.36 &  0.35 &      118 &    283.0 $\pm$     6.3 &    271.6 $\pm$     6.9\\
NGC2992 & VISIR &  084.B-0606(A)  & 09-11-30 & NEII\_1 & 12.27 &  0.18 &      181 &  0.39 &  0.36 &       64 &  0.46 &  0.39 &       12 &    193.1 $\pm$    15.9 &    146.1 $\pm$    12.5\\
NGC2992 & VISIR &  084.B-0606(A)  & 09-12-02 & NEII\_1 & 12.27 &  0.18 &      181 &  0.41 &  0.36 &      111 &  0.41 &  0.37 &       33 &    166.0 $\pm$     3.0 &    155.7 $\pm$     9.0\\
NGC2992 & VISIR &  084.B-0606(A)  & 09-12-02 & NEII\_2 & 13.04 &  0.22 &      181 &  0.39 &  0.34 &      100 &  0.42 &  0.39 &       48 &    223.2 $\pm$     5.0 &    180.2 $\pm$    17.9\\
NGC2992 & VISIR &  084.B-0606(A)  & 09-11-30 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.31 &      110 &  0.42 &  0.39 &       28 &    146.5 $\pm$    15.6 &     92.4 $\pm$     9.6\\
NGC2992 & VISIR &  084.B-0606(A)  & 09-12-02 & PAH2 & 11.25 &  0.59 &      181 &  0.39 &  0.33 &       99 &  0.39 &  0.37 &       44 &    141.2 $\pm$    13.3 &    125.4 $\pm$     7.4\\
NGC2992 & VISIR &  60.A-9244(A)  & 04-12-22 & PAH2 & 11.25 &  0.59 &     2119 &  0.41 &  0.37 &       98 &  0.39 &  0.36 &       97 &    289.6 $\pm$    14.6 &    312.6 $\pm$    14.6\\
NGC2992 & VISIR &  60.A-9244(A)  & 05-02-01 & PAH2 & 11.25 &  0.59 &      883 &  0.41 &  0.38 &      151 &  0.40 &  0.38 &       12 &    300.7 $\pm$    33.3 &    318.7 $\pm$    22.7\\
NGC2992 & MICHELLE &  GN-2006A-Q-11  & 06-05-12 & N\_prime & 11.20 &  1.20 &      188 &  0.40 &  0.34 &      174 &  0.49 &  0.41 &        5 &    229.8 $\pm$     4.0 &    161.2 $\pm$     3.5\\
NGC2992 & MICHELLE &  GN-2006A-Q-11  & 06-05-12 & Qa & 18.10 &  0.95 &      163 &  0.53 &  0.51 &      154 &  0.60 &  0.52 &       19 &    631.8 $\pm$    21.6 &    541.9 $\pm$    20.5\\
NGC3081 & VISIR &  080.B-0860(A)  & 07-12-30 & NEII\_2 & 13.04 &  0.22 &       62 &  0.37 &  0.37 &      147 &  0.52 &  0.29 &      124 &    202.8 $\pm$    36.9 &    179.1 $\pm$    36.9\\
NGC3081 & VISIR &  080.B-0860(A)  & 07-12-30 & PAH1 &  8.59 &  0.42 &       62 &  0.33 &  0.29 &      113 &  0.43 &  0.29 &      122 &     84.6 $\pm$     9.6 &     64.8 $\pm$     9.6\\
NGC3081 & VISIR &  080.B-0860(A)  & 07-12-30 & PAH2 & 11.25 &  0.59 &       62 &  0.32 &  0.30 &      111 &  0.41 &  0.30 &      128 &    155.1 $\pm$    15.8 &    117.5 $\pm$    15.8\\
NGC3081 & TRECS &  GS-2005A-Q-6  & 06-01-25 & Qa & 18.30 &  0.76 &      304 &  0.62 &  0.57 &      153 &  1.00 &  0.65 &      170 &    466.4 $\pm$    18.7 &    239.6 $\pm$    18.3\\
NGC3081 & TRECS &  GS-2005A-Q-6  & 06-01-25 & Si2 &  8.74 &  0.39 &      130 &  0.38 &  0.35 &      167 &  0.42 &  0.38 &       74 &     92.0 $\pm$     3.2 &     76.5 $\pm$     3.1\\
NGC3081 & VISIR &  080.B-0860(A)  & 07-12-30 & SIV & 10.49 &  0.16 &       62 &  0.35 &  0.30 &       99 &  0.42 &  0.28 &      130 &    147.2 $\pm$    23.9 &    112.0 $\pm$    23.9\\
NGC3094 & TRECS &  GS-2008A-Q-55  & 08-03-02 & N & 10.36 &  2.64 &      318 &  0.41 &  0.40 &       72 &  0.42 &  0.37 &        7 &    372.9 $\pm$     6.9 &    393.5 $\pm$     7.1\\
NGC3094 & TRECS &  GS-2008A-Q-55  & 08-06-06 & N & 10.36 &  2.64 &      318 &  0.75 &  0.63 &      125 &  0.75 &  0.65 &      134 &    367.0 $\pm$     7.3 &    353.6 $\pm$     7.2\\
NGC3094 & TRECS &  GS-2008A-Q-55  & 09-01-08 & N & 10.36 &  2.64 &      318 &  0.61 &  0.53 &       59 &  0.58 &  0.50 &       27 &    372.4 $\pm$     6.6 &    415.7 $\pm$     7.0\\
NGC3147 & MICHELLE &  GN-2010A-C-7  & 10-02-05 & Si-5 & 11.60 &  0.55 &      259 &  0.54 &  0.48 &      135 &  0.68 &  0.50 &      149 &     21.4 $\pm$     2.7 &     16.1 $\pm$     2.7\\
NGC3147 & MICHELLE &  GN-2010A-C-7  & 10-02-05 & Si-6 & 12.50 &  0.60 &      282 &  0.54 &  0.53 &      153 &  0.70 &  0.54 &      156 &     22.3 $\pm$     3.2 &     16.8 $\pm$     3.2\\
NGC3166 & TRECS &  GS-2007B-Q-203  & 07-12-02 & Si2 &  8.74 &  0.39 &      926 &  0.57 &  0.43 &       38 &  $\dots$  &  $\dots$  &  $\dots$  &      4.6 $\pm$     0.3 &      4.5 $\pm$     0.3\\
NGC3169 & VISIR &  384.B-0943(A)  & 10-01-09 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.34 &  0.32 &      121 &  0.63 &  0.47 &       67 &     20.2 $\pm$     4.3 &      7.7 $\pm$     4.6\\
NGC3169 & TRECS &  GS-2007B-Q-203  & 07-12-03 & Si2 &  8.74 &  0.39 &      926 &  0.70 &  0.58 &       54 &  1.00 &  0.64 &       45 &     13.1 $\pm$     1.4 &      8.8 $\pm$     1.4\\
NGC3169 & TRECS &  GS-2007B-Q-203  & 07-12-06 & Si2 &  8.74 &  0.39 &      926 &  0.50 &  0.41 &       42 &  1.00 &  0.61 &       38 &     13.4 $\pm$     1.0 &      4.7 $\pm$     1.0\\
NGC3185 & VISIR &  084.B-0974(A)  & 10-01-30 & PAH1 &  8.59 &  0.42 &     1922 &  0.51 &  0.41 &       94 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    19.0   &  $\le$    19.0  \\
NGC3227 & VISIR &  080.B-0240(A)  & 08-03-22 & ARIII &  8.99 &  0.14 &      353 &  0.41 &  0.28 &      103 &  0.34 &  0.32 &       46 &    181.8 $\pm$     4.5 &    185.2 $\pm$     7.0\\
NGC3227 & VISIR &  084.B-0366(E)  & 10-03-11 & PAH1 &  8.59 &  0.42 &      362 &  0.26 &  0.24 &       61 &  0.35 &  0.31 &      146 &    149.3 $\pm$     9.3 &     90.5 $\pm$     9.7\\
NGC3227 & VISIR &  080.B-0240(A)  & 08-03-22 & PAH2\_2 & 11.88 &  0.37 &      236 &  0.36 &  0.32 &      111 &  0.39 &  0.38 &      143 &    318.8 $\pm$     4.7 &    248.0 $\pm$     6.6\\
NGC3227 & VISIR &  084.B-0366(E)  & 10-03-11 & PAH2\_2 & 11.88 &  0.37 &      362 &  0.32 &  0.31 &       18 &  0.38 &  0.34 &      179 &    302.2 $\pm$    26.2 &    236.7 $\pm$    14.3\\
NGC3227 & VISIR &  080.B-0240(A)  & 08-03-22 & Q1 & 17.65 &  0.83 &     1382 &  0.50 &  0.44 &      104 &  0.54 &  0.51 &       96 &    976.9 $\pm$    49.3 &    771.8 $\pm$    47.4\\
NGC3227 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.37 &  0.31 &      113 &  0.50 &  0.48 &      110 &    341.9 $\pm$    39.5 &    172.8 $\pm$     4.7\\
NGC3227 & VISIR &  080.B-0240(A)  & 08-03-22 & PAH1 &  8.59 &  0.42 &       62 &  0.32 &  0.27 &       97 &  0.38 &  0.32 &      117 &    151.8 $\pm$    27.7 &    111.2 $\pm$    16.4\\
NGC3227 & MICHELLE &  GN-2006A-Q-30  & 06-04-07 & N\_prime & 11.20 &  1.20 &      376 &  0.57 &  0.48 &       28 &  0.51 &  0.47 &      173 &    332.3 $\pm$     6.8 &    371.5 $\pm$     7.1\\
NGC3281 & VISIR &  080.B-0860(A)  & 08-02-07 & NEII\_2 & 13.04 &  0.22 &      540 &  0.36 &  0.34 &      106 &  0.43 &  0.37 &      163 &   1013.0 $\pm$    16.6 &    797.0 $\pm$    18.5\\
NGC3281 & TRECS &  GS-2003B-DD-4  & 04-01-30 & N & 10.36 &  2.64 &      260 &  0.36 &  0.35 &      110 &  0.47 &  0.43 &      175 &    466.6 $\pm$     6.9 &    297.9 $\pm$     6.0\\
NGC3281 & VISIR &  080.B-0860(A)  & 08-02-07 & PAH1 &  8.59 &  0.42 &      543 &  0.31 &  0.25 &      108 &  0.34 &  0.31 &      174 &    421.3 $\pm$    11.7 &    329.4 $\pm$    23.5\\
NGC3281 & VISIR &  080.B-0860(A)  & 08-02-07 & PAH2 & 11.25 &  0.59 &      543 &  0.33 &  0.30 &       95 &  0.38 &  0.32 &      171 &    456.5 $\pm$     7.6 &    361.9 $\pm$    20.8\\
NGC3281 & TRECS &  GS-2003B-DD-4  & 04-01-30 & Qa & 18.30 &  0.76 &      456 &  0.62 &  0.58 &      160 &  0.71 &  0.66 &      156 &   1146.4 $\pm$    33.7 &    870.4 $\pm$    32.9\\
NGC3281 & TRECS &  GS-2008A-Q-55  & 08-03-28 & Si2 &  8.74 &  0.39 &      318 &  0.54 &  0.51 &      148 &  0.55 &  0.49 &       11 &    382.9 $\pm$     8.3 &    394.7 $\pm$     8.4\\
NGC3281 & TRECS &  GS-2008A-Q-55  & 08-04-10 & Si2 &  8.74 &  0.39 &      318 &  0.46 &  0.37 &       36 &  0.49 &  0.42 &       23 &    400.4 $\pm$     8.5 &    329.9 $\pm$     7.8\\
NGC3281 & VISIR &  080.B-0860(A)  & 08-03-20 & SIC & 11.85 &  2.34 &      540 &  0.35 &  0.31 &      100 &  0.39 &  0.37 &      179 &    651.3 $\pm$     8.1 &    486.4 $\pm$    13.5\\
NGC3281 & VISIR &  080.B-0860(A)  & 08-03-20 & SIV & 10.49 &  0.16 &      538 &  0.31 &  0.28 &      113 &  0.36 &  0.35 &      137 &    275.2 $\pm$     8.8 &    192.6 $\pm$    13.9\\
NGC3312 & VISIR &  083.B-0536(C)  & 09-07-15 & PAH2 & 11.25 &  0.59 &      724 &  0.40 &  0.38 &      161 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.4   &      8.4 $\pm$     0.0\\
NGC3312 & VISIR &  086.B-0349(C)  & 10-12-29 & PAH2\_2 & 11.88 &  0.37 &     1986 &  0.30 &  0.30 &       64 &  0.34 &  0.29 &       84 &      7.7 $\pm$     1.0 &      7.2 $\pm$     1.0\\
NGC3368 & VISIR &  384.B-0943(A)  & 10-02-23 & PAH2\_2 & 11.88 &  0.37 &      905 &  0.41 &  0.34 &      126 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.3   &  $\le$    13.3  \\
NGC3379 & VISIR &  084.B-0974(A)  & 10-01-29 & PAH1 &  8.59 &  0.42 &     1986 &  0.30 &  0.26 &       42 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     2.0   &  $\le$     2.0  \\
NGC3393 & VISIR &  080.B-0860(A)  & 08-03-22 & NEII\_2 & 13.04 &  0.22 &       62 &  0.38 &  0.35 &      141 &  0.57 &  0.31 &       66 &     95.5 $\pm$    23.3 &     71.0 $\pm$    23.3\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-02-26 & PAH1 &  8.59 &  0.42 &       62 &  0.35 &  0.28 &      110 &  0.36 &  0.28 &      104 &     23.8 $\pm$     6.9 &     21.1 $\pm$     6.9\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH1 &  8.59 &  0.42 &       62 &  0.36 &  0.34 &      109 &  0.27 &  0.19 &      138 &     13.8 $\pm$     6.9 &     32.4 $\pm$     6.9\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-02-26 & PAH2 & 11.25 &  0.59 &       63 &  0.40 &  0.36 &        9 &  0.42 &  0.30 &      170 &     36.9 $\pm$    10.5 &     41.0 $\pm$    10.5\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH2 & 11.25 &  0.59 &       62 &  0.36 &  0.32 &      163 &  0.45 &  0.36 &       45 &     40.3 $\pm$    11.0 &     28.6 $\pm$    11.0\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-02-26 & SIV & 10.49 &  0.16 &       61 &  0.35 &  0.34 &      172 &  0.41 &  0.30 &        4 &     39.8 $\pm$    13.2 &     38.7 $\pm$    13.2\\
NGC3393 & VISIR &  080.B-0860(A)  & 08-03-22 & SIV & 10.49 &  0.16 &       62 &  0.34 &  0.32 &      148 &  0.45 &  0.25 &       37 &     32.8 $\pm$    12.7 &     27.7 $\pm$    12.7\\
NGC3486 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      259 &  0.53 &  0.50 &      173 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.2   &  $\le$    10.2  \\
NGC3486 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-5 & 11.60 &  0.55 &      362 &  0.42 &  0.41 &      124 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     4.7   &  $\le$     4.7  \\
NGC3486 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      376 &  0.43 &  0.42 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.1   &  $\le$     6.1  \\
NGC3521 & VISIR &  384.B-0943(A)  & 10-01-09 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.34 &  0.32 &      121 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     9.1   &  $\le$     9.1  \\
NGC3607 & VISIR &  084.B-0974(A)  & 10-01-31 & PAH1 &  8.59 &  0.42 &     1986 &  0.48 &  0.37 &      141 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.4   &  $\le$     8.4  \\
NGC3623 & VISIR &  384.B-0943(A)  & 10-02-23 & PAH2\_2 & 11.88 &  0.37 &      905 &  0.40 &  0.34 &       12 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    15.2   &  $\le$    15.2  \\
NGC3627 & VISIR &  084.B-0974(A)  & 10-01-30 & PAH1 &  8.59 &  0.42 &     1398 &  0.51 &  0.41 &       94 &  1.00 &  1.00 &       35 &     93.5 $\pm$    11.7 &     10.3 $\pm$     0.8\\
NGC3628 & VISIR &  084.B-0974(A)  & 10-02-23 & PAH1 &  8.59 &  0.42 &     2166 &  0.39 &  0.30 &      133 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    50.1   &  $\le$     6.3  \\
NGC3660 & TRECS &  GS-2004A-Q-14  & 04-03-05 & N & 10.36 &  2.64 &      716 &  0.45 &  0.40 &      137 &  0.64 &  0.51 &       97 &     26.3 $\pm$     1.8 &     14.1 $\pm$     1.7\\
NGC3690E & MICHELLE &  GN-2003B-Q-72  & 03-12-13 & Si-1 &  7.70 &  0.35 &      300 &  0.65 &  0.58 &      105 &  0.98 &  0.93 &       73 &    649.4 $\pm$    16.5 &    266.2 $\pm$    14.9\\
NGC3690E & MICHELLE &  GN-2003B-Q-72  & 03-12-13 & Si-5 & 11.60 &  0.55 &      322 &  0.54 &  0.45 &      107 &  0.82 &  0.80 &      102 &    408.0 $\pm$     8.4 &    151.6 $\pm$     7.0\\
NGC3690W & MICHELLE &  GN-2003B-Q-72  & 03-12-13 & Si-1 &  7.70 &  0.35 &      300 &  0.65 &  0.58 &      105 &  1.00 &  0.99 &      142 &    745.5 $\pm$    18.1 &    283.2 $\pm$    16.2\\
NGC3690W & MICHELLE &  GN-2003B-Q-72  & 03-12-13 & Si-5 & 11.60 &  0.55 &      322 &  0.54 &  0.45 &      107 &  0.99 &  0.81 &      157 &   1184.8 $\pm$    20.8 &    360.8 $\pm$    15.6\\
NGC3718 & MICHELLE &  GN-2008A-Q-43  & 08-07-11 & N\_prime & 11.20 &  1.20 &      940 &  0.42 &  0.37 &       91 &  0.48 &  0.44 &      104 &     19.7 $\pm$     0.2 &     14.4 $\pm$     0.8\\
NGC3783 & VISIR &  080.B-0240(A)  & 08-03-20 & ARIII &  8.99 &  0.14 &      228 &  0.33 &  0.27 &       87 &  0.34 &  0.31 &       70 &    370.4 $\pm$     5.5 &    306.9 $\pm$     4.6\\
NGC3783 & VISIR &  075.B-0844(C)  & 05-04-17 & NEII\_1 & 12.27 &  0.18 &      180 &  0.34 &  0.32 &       99 &  0.37 &  0.35 &      160 &    708.8 $\pm$    32.6 &    592.4 $\pm$    32.5\\
NGC3783 & VISIR &  083.B-0452(F)  & 09-05-19 & PAH1 &  8.59 &  0.42 &      118 &  0.27 &  0.24 &       71 &  0.31 &  0.27 &       88 &    387.7 $\pm$    14.1 &    309.4 $\pm$    19.6\\
NGC3783 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH1 &  8.59 &  0.42 &      117 &  0.26 &  0.25 &       76 &  0.29 &  0.27 &      127 &    396.7 $\pm$    12.8 &    329.5 $\pm$    13.8\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-01-01 & PAH1 &  8.59 &  0.42 &      721 &  0.30 &  0.27 &      134 &  0.38 &  0.34 &        5 &    343.0 $\pm$     5.4 &    241.4 $\pm$     6.8\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-01-11 & PAH1 &  8.59 &  0.42 &      362 &  0.45 &  0.36 &       42 &  0.43 &  0.35 &      112 &    369.6 $\pm$    12.8 &    404.0 $\pm$    27.5\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-02-24 & PAH1 &  8.59 &  0.42 &      360 &  0.37 &  0.32 &       27 &  0.37 &  0.34 &      129 &    348.2 $\pm$    10.8 &    324.5 $\pm$    26.3\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-10 & PAH1 &  8.59 &  0.42 &      362 &  0.62 &  0.52 &      108 &  0.46 &  0.44 &      108 &    353.9 $\pm$     7.0 &    549.4 $\pm$    47.8\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-13 & PAH1 &  8.59 &  0.42 &      360 &  0.35 &  0.27 &      128 &  0.26 &  0.25 &      114 &    372.4 $\pm$    10.4 &    552.4 $\pm$    21.4\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-14 & PAH1 &  8.59 &  0.42 &      362 &  0.47 &  0.40 &       77 &  0.50 &  0.42 &      104 &    335.0 $\pm$    10.5 &    290.6 $\pm$    11.1\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-18 & PAH1 &  8.59 &  0.42 &      362 &  0.40 &  0.34 &      121 &  0.50 &  0.43 &       56 &    407.6 $\pm$    12.4 &    262.8 $\pm$    34.7\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-23 & PAH1 &  8.59 &  0.42 &      362 &  0.42 &  0.34 &       81 &  0.44 &  0.33 &       99 &    373.5 $\pm$    14.0 &    369.5 $\pm$    39.8\\
NGC3783 & VISIR &  086.B-0242(A)  & 11-03-27 & PAH1 &  8.59 &  0.42 &      362 &  0.29 &  0.27 &       84 &  0.37 &  0.33 &      107 &    384.9 $\pm$    12.3 &    239.0 $\pm$    11.6\\
NGC3783 & VISIR &  60.A-9244(A)  & 05-01-28 & PAH2 & 11.25 &  0.59 &     1059 &  0.38 &  0.37 &      116 &  0.40 &  0.35 &      173 &    721.5 $\pm$    11.6 &    688.3 $\pm$    63.4\\
NGC3783 & VISIR &  075.B-0844(C)  & 05-04-17 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.35 &  0.30 &       97 &  0.37 &  0.34 &      139 &    617.9 $\pm$    36.2 &    521.1 $\pm$    18.6\\
NGC3783 & VISIR &  077.B-0728(A)  & 06-04-29 & PAH2\_2 & 11.88 &  0.37 &      543 &  0.33 &  0.31 &      104 &  0.34 &  0.34 &      140 &    653.1 $\pm$    14.0 &    590.8 $\pm$    38.9\\
NGC3783 & VISIR &  080.B-0240(A)  & 08-03-20 & PAH2\_2 & 11.88 &  0.37 &      236 &  0.33 &  0.32 &      112 &  0.36 &  0.34 &       85 &    622.9 $\pm$    22.4 &    543.3 $\pm$    77.0\\
NGC3783 & VISIR &  083.B-0452(F)  & 09-05-19 & PAH2\_2 & 11.88 &  0.37 &      236 &  0.34 &  0.32 &       51 &  0.35 &  0.34 &       98 &    732.5 $\pm$    14.1 &    665.6 $\pm$    13.8\\
NGC3783 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.33 &  0.31 &       69 &  0.35 &  0.34 &      137 &    693.6 $\pm$    17.6 &    604.9 $\pm$    23.1\\
NGC3783 & VISIR &  080.B-0240(A)  & 08-03-20 & Q1 & 17.65 &  0.83 &      342 &  0.48 &  0.44 &       81 &  0.50 &  0.47 &       53 &   1470.4 $\pm$   106.6 &   1254.8 $\pm$    14.1\\
NGC3783 & VISIR &  076.B-0599(A)  & 06-03-13 & Q2 & 18.72 &  0.88 &      684 &  0.52 &  0.50 &      104 &  0.52 &  0.51 &       82 &   1439.2 $\pm$    75.0 &   1401.7 $\pm$    58.7\\
NGC3783 & VISIR &  075.B-0844(C)  & 05-04-17 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.28 &       91 &  0.34 &  0.32 &      121 &    557.6 $\pm$    30.6 &    456.2 $\pm$    32.6\\
NGC3982 & MICHELLE &  GN-2010A-C-7  & 10-02-05 & Si-5 & 11.60 &  0.55 &      518 &  0.44 &  0.43 &      162 &  0.48 &  0.46 &       13 &     24.9 $\pm$     1.3 &     21.4 $\pm$     1.3\\
NGC3982 & MICHELLE &  GN-2010A-C-7  & 10-02-05 & Si-6 & 12.50 &  0.60 &      517 &  0.45 &  0.42 &      117 &  0.50 &  0.48 &       68 &     30.2 $\pm$     1.9 &     23.9 $\pm$     1.9\\
NGC3998 & COMICS &  o00001  & 05-12-21 & N11.7 & 11.74 &  0.53 &     1604 &  0.35 &  0.34 &       86 &  0.62 &  0.52 &      104 &     95.0 $\pm$     4.7 &     34.5 $\pm$     3.7\\
NGC3998 & COMICS &  o00001  & 05-12-21 & UIR8.6 &  8.59 &  0.21 &     2006 &  0.70 &  0.56 &       29 &  0.74 &  0.66 &      163 &     33.1 $\pm$     9.1 &     31.7 $\pm$     5.5\\
NGC3998 & MICHELLE &  GN-2011A-Q-55  & 11-01-23 & Qa & 18.10 &  0.95 &      324 &  0.58 &  0.51 &       36 &  0.58 &  0.51 &       33 &    153.4 $\pm$    15.2 &    155.8 $\pm$    15.2\\
NGC3998 & MICHELLE &  GN-2006A-Q-30  & 06-06-12 & Si-2 &  8.80 &  0.45 &      414 &  $\dots$  &  $\dots$  &  $\dots$  &  0.93 &  0.83 &       58 &     33.9 $\pm$     4.3 &  $\le$    46.7  \\
NGC3998 & MICHELLE &  GN-2011A-Q-55  & 11-01-23 & Si-2 &  8.80 &  0.45 &      311 &  $\dots$  &  $\dots$  &  $\dots$  &  0.42 &  0.32 &       36 &     26.5 $\pm$     3.2 &  $\le$    36.1  \\
NGC3998 & MICHELLE &  GN-2006A-Q-30  & 06-06-12 & Si-4 & 10.30 &  0.50 &      353 &  $\dots$  &  $\dots$  &  $\dots$  &  0.76 &  0.68 &      156 &     70.3 $\pm$     8.3 &  $\le$    95.3  \\
NGC3998 & MICHELLE &  GN-2011A-Q-55  & 11-01-23 & Si-4 & 10.30 &  0.50 &      309 &  $\dots$  &  $\dots$  &  $\dots$  &  0.49 &  0.43 &       26 &     59.5 $\pm$     6.4 &  $\le$    78.6  \\
NGC3998 & MICHELLE &  GN-2006A-Q-30  & 06-06-12 & Si-6 & 12.50 &  0.60 &      376 &  $\dots$  &  $\dots$  &  $\dots$  &  0.56 &  0.47 &      152 &     71.0 $\pm$     7.6 &  $\le$    93.8  \\
NGC4051 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      155 &  0.46 &  0.40 &      150 &  0.47 &  0.42 &      133 &    464.0 $\pm$    10.2 &    438.1 $\pm$     9.9\\
NGC4074 & VISIR &  084.B-0606(A)  & 10-01-27 & NEII & 12.81 &  0.21 &     1983 &  0.34 &  0.33 &       30 &  0.41 &  0.40 &        8 &     80.3 $\pm$     2.5 &     56.2 $\pm$     1.5\\
NGC4111 & MICHELLE &  GN-2008A-Q-43  & 08-06-12 & N\_prime & 11.20 &  1.20 &      470 &  0.52 &  0.49 &      121 &  1.00 &  1.00 &       11 &     12.1 $\pm$     0.5 &      3.3 $\pm$     0.5\\
NGC4138 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      259 &  0.46 &  0.40 &      150 &  0.52 &  0.44 &      146 &     21.0 $\pm$     2.1 &     16.8 $\pm$     2.1\\
NGC4151 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH1 &  8.59 &  0.42 &      117 &  0.65 &  0.48 &       21 &  0.52 &  0.45 &       20 &    816.6 $\pm$    33.5 &   1123.4 $\pm$    58.3\\
NGC4151 & VISIR &  084.B-0366(E)  & 10-03-29 & PAH1 &  8.59 &  0.42 &      360 &  0.62 &  0.47 &       34 &  0.46 &  0.37 &       26 &    872.8 $\pm$    20.1 &   1476.7 $\pm$    67.7\\
NGC4151 & VISIR &  083.B-0452(F)  & 09-06-07 & PAH2\_2 & 11.88 &  0.37 &      117 &  0.59 &  0.47 &       21 &  0.65 &  0.51 &       15 &   1301.5 $\pm$    70.7 &   1095.9 $\pm$    53.9\\
NGC4151 & VISIR &  084.B-0366(E)  & 10-03-29 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.55 &  0.39 &       32 &  0.54 &  0.44 &       31 &   1398.7 $\pm$    32.3 &   1259.3 $\pm$   124.4\\
NGC4151 & MICHELLE &  GN-2006B-Q-18  & 07-03-18 & Si-5 & 11.60 &  0.55 &       12 &  0.46 &  0.41 &      151 &  0.51 &  0.50 &      117 &   1528.2 $\pm$    33.0 &   1130.6 $\pm$    30.1\\
NGC4235 & VISIR &  083.B-0536(A)  & 09-06-08 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.55 &  0.46 &       80 &  0.43 &  0.36 &      148 &     36.0 $\pm$     5.4 &     57.6 $\pm$     1.0\\
NGC4235 & VISIR &  085.B-0639(C)  & 10-04-14 & PAH1 &  8.59 &  0.42 &      362 &  0.33 &  0.32 &       28 &  0.34 &  0.28 &       43 &     32.6 $\pm$     3.8 &     34.3 $\pm$     6.4\\
NGC4235 & VISIR &  083.B-0536(A)  & 09-06-08 & PAH2 & 11.25 &  0.59 &      362 &  0.47 &  0.39 &       89 &  0.41 &  0.39 &        9 &     39.8 $\pm$     5.5 &     46.9 $\pm$     4.1\\
NGC4235 & VISIR &  085.B-0639(D)  & 10-05-12 & Q2 & 18.72 &  0.88 &     1987 &  0.46 &  0.46 &       72 &  0.47 &  0.45 &       97 &     58.2 $\pm$     7.0 &     58.7 $\pm$     2.1\\
NGC4235 & VISIR &  085.B-0639(C)  & 10-04-14 & SIV\_2 & 10.77 &  0.19 &      541 &  0.38 &  0.34 &       22 &  0.36 &  0.31 &       12 &     43.1 $\pm$     5.3 &     49.4 $\pm$     7.6\\
NGC4258 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-2 &  8.80 &  0.45 &      311 &  0.40 &  0.37 &       30 &  0.42 &  0.37 &       30 &     69.4 $\pm$     2.0 &     70.3 $\pm$     2.1\\
NGC4258 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-4 & 10.30 &  0.50 &      309 &  0.40 &  0.36 &       17 &  0.49 &  0.44 &        1 &    108.7 $\pm$     4.8 &     98.1 $\pm$     4.5\\
NGC4258 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      155 &  0.47 &  0.40 &      137 &  0.42 &  0.37 &      124 &    128.3 $\pm$     3.5 &    154.7 $\pm$     3.6\\
NGC4258 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-5 & 11.60 &  0.55 &      155 &  0.50 &  0.48 &      145 &  0.46 &  0.44 &      153 &    141.6 $\pm$     3.2 &    165.9 $\pm$     3.3\\
NGC4258 & MICHELLE &  GN-2011A-Q-55  & 11-02-03 & Si-6 & 12.50 &  0.60 &      329 &  0.41 &  0.38 &       18 &  0.42 &  0.40 &       88 &    133.2 $\pm$     2.4 &    126.7 $\pm$     2.3\\
NGC4258 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      141 &  0.46 &  0.44 &      149 &  0.50 &  0.48 &      141 &    139.0 $\pm$     4.8 &    118.5 $\pm$     4.7\\
NGC4261 & COMICS &  o05405  & 05-04-30 & N11.7 & 11.74 &  0.53 &     1943 &  0.46 &  0.39 &       78 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.3   &  $\le$     6.3  \\
NGC4261 & COMICS &  o05405  & 05-04-30 & N8.8 &  8.75 &  0.38 &      484 &  0.44 &  0.35 &       79 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.1   &  $\le$     7.1  \\
NGC4261 & VISIR &  083.B-0536(C)  & 09-06-16 & NEII\_1 & 12.27 &  0.18 &     3245 &  0.39 &  0.37 &       67 &  $\dots$  &  $\dots$  &  $\dots$  &     12.1 $\pm$     1.2 &     12.1 $\pm$     1.2\\
NGC4261 & VISIR &  085.B-0639(C)  & 10-05-28 & PAH1 &  8.59 &  0.42 &      722 &  0.36 &  0.33 &       85 &  $\dots$  &  $\dots$  &  $\dots$  &      4.6 $\pm$     0.4 &      4.6 $\pm$     0.4\\
NGC4261 & VISIR &  083.B-0536(C)  & 09-06-18 & PAH2 & 11.25 &  0.59 &      543 &  0.33 &  0.30 &       71 &  $\dots$  &  $\dots$  &  $\dots$  &      9.7 $\pm$     1.3 &      9.7 $\pm$     1.3\\
NGC4261 & VISIR &  384.B-0943(A)  & 10-02-22 & PAH2\_2 & 11.88 &  0.37 &      906 &  0.36 &  0.32 &      167 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.2   &  $\le$     6.2  \\
NGC4261 & VISIR &  085.B-0639(D)  & 10-05-12 & Q2 & 18.72 &  0.88 &     1987 &  0.46 &  0.46 &       72 &  $\dots$  &  $\dots$  &  $\dots$  &     22.0 $\pm$     1.0 &     21.9 $\pm$     1.0\\
NGC4261 & TRECS &  GS-2007B-Q-203  & 08-01-03 & Si2 &  8.74 &  0.39 &      926 &  0.38 &  0.34 &       48 &  $\dots$  &  $\dots$  &  $\dots$  &      3.5 $\pm$     0.3 &      3.5 $\pm$     0.3\\
NGC4261 & VISIR &  077.B-0135(A)  & 06-06-18 & SIC & 11.85 &  2.34 &     5382 &  0.53 &  0.44 &       96 &  $\dots$  &  $\dots$  &  $\dots$  &     15.2 $\pm$     1.7 &     15.0 $\pm$     1.7\\
NGC4261 & VISIR &  085.B-0639(C)  & 10-05-25 & SIV\_2 & 10.77 &  0.19 &     1986 &  0.36 &  0.35 &       76 &  $\dots$  &  $\dots$  &  $\dots$  &      8.4 $\pm$     0.6 &      8.4 $\pm$     0.6\\
NGC4278 & MICHELLE &  GN-2008A-Q-43  & 08-06-16 & N\_prime & 11.20 &  1.20 &      470 &  0.40 &  0.39 &       63 &  $\dots$  &  $\dots$  &  $\dots$  &      2.2 $\pm$     0.3 &      2.2 $\pm$     0.3\\
NGC4303 & VISIR &  077.B-0137(A)  & 06-04-15 & NEII\_1 & 12.27 &  0.18 &     2524 &  0.37 &  0.33 &      136 &  $\dots$  &  $\dots$  &  $\dots$  &      6.1 $\pm$     0.5 &      6.1 $\pm$     0.5\\
NGC4374 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &     1403 &  0.45 &  0.38 &       12 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     3.6   &  $\le$     3.6  \\
NGC4374 & VISIR &  384.B-0943(A)  & 10-02-22 & PAH2\_2 & 11.88 &  0.37 &      906 &  0.36 &  0.32 &      167 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.5   &  $\le$    10.5  \\
NGC4374 & TRECS &  GS-2007B-Q-203  & 08-02-20 & Si2 &  8.74 &  0.39 &      926 &  0.50 &  0.41 &       54 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.4   &  $\le$     6.4  \\
NGC4374 & TRECS &  GS-2007B-Q-203  & 08-04-10 & Si2 &  8.74 &  0.39 &      926 &  0.36 &  0.34 &       60 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     3.9   &  $\le$     3.9  \\
NGC4374 & TRECS &  GS-2007B-Q-215  & 08-05-03 & Si2 &  8.74 &  0.39 &      347 &  0.64 &  0.55 &       83 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.1   &  $\le$    12.1  \\
NGC4374 & TRECS &  GS-2007B-Q-215  & 08-06-13 & Si2 &  8.74 &  0.39 &      347 &  0.53 &  0.48 &      101 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     9.0   &  $\le$     9.0  \\
NGC4388 & VISIR &  080.B-0860(A)  & 08-03-21 & NEII\_2 & 13.04 &  0.22 &       62 &  0.38 &  0.36 &      103 &  0.52 &  0.47 &      102 &    425.6 $\pm$    97.6 &    256.2 $\pm$    52.0\\
NGC4388 & VISIR &  080.B-0860(A)  & 08-03-21 & PAH1 &  8.59 &  0.42 &       62 &  0.38 &  0.37 &       91 &  0.56 &  0.49 &       82 &    144.2 $\pm$    10.4 &     77.8 $\pm$    12.1\\
NGC4388 & VISIR &  080.B-0860(A)  & 08-03-21 & PAH2 & 11.25 &  0.59 &       62 &  0.36 &  0.31 &      110 &  0.46 &  0.39 &       78 &    194.4 $\pm$    17.8 &    125.9 $\pm$    15.4\\
NGC4388 & VISIR &  080.B-0860(A)  & 08-03-21 & SIV & 10.49 &  0.16 &       62 &  0.36 &  0.34 &      125 &  0.50 &  0.36 &       18 &    155.2 $\pm$    26.2 &    103.8 $\pm$    26.0\\
NGC4388 & MICHELLE &  GN-2006A-Q-11  & 06-05-12 & N\_prime & 11.20 &  1.20 &      141 &  0.44 &  0.36 &      177 &  0.50 &  0.44 &       15 &    252.6 $\pm$     5.1 &    185.1 $\pm$     4.7\\
NGC4388 & MICHELLE &  GN-2006A-Q-11  & 06-05-12 & Qa & 18.10 &  0.95 &      108 &  0.55 &  0.52 &      158 &  0.62 &  0.56 &       19 &    950.6 $\pm$    27.3 &    762.7 $\pm$    25.5\\
NGC4395 & MICHELLE &  GN-2010A-C-7  & 10-02-05 & Si-6 & 12.50 &  0.60 &       70 &  0.42 &  0.40 &       69 &  0.56 &  0.51 &      101 &      9.7 $\pm$     1.7 &      5.9 $\pm$     1.7\\
NGC4418 & VISIR &  076.B-0696(A)  & 06-01-18 & NEII & 12.81 &  0.21 &     3670 &  0.51 &  0.41 &       80 &  0.56 &  0.46 &       64 &   1711.1 $\pm$    66.6 &   1345.5 $\pm$    81.0\\
NGC4418 & VISIR &  076.B-0696(A)  & 06-01-18 & NEII\_2 & 13.04 &  0.22 &     3532 &  0.74 &  0.42 &       42 &  0.55 &  0.47 &       62 &   1728.0 $\pm$    38.0 &   1864.2 $\pm$    62.8\\
NGC4418 & TRECS &  GS-2004A-C-2  & 04-05-07 & N & 10.36 &  2.64 &       18 &  0.65 &  0.61 &      160 &  0.71 &  0.61 &      144 &    403.9 $\pm$    15.5 &    369.5 $\pm$    15.3\\
NGC4418 & TRECS &  GS-2004A-C-2  & 04-05-08 & N & 10.36 &  2.64 &       18 &  0.47 &  0.41 &       22 &  0.44 &  0.38 &      160 &    517.5 $\pm$    12.6 &    593.6 $\pm$    13.0\\
NGC4418 & VISIR &  60.A-9244(A)  & 05-01-29 & PAH2 & 11.25 &  0.59 &      906 &  0.33 &  0.32 &      125 &  0.44 &  0.38 &      120 &    130.5 $\pm$     4.2 &     79.4 $\pm$     2.8\\
NGC4418 & VISIR &  60.A-9244(A)  & 05-01-31 & PAH2 & 11.25 &  0.59 &      906 &  0.42 &  0.39 &        1 &  0.45 &  0.42 &      115 &    112.7 $\pm$     7.0 &     98.3 $\pm$     3.3\\
NGC4418 & VISIR &  077.B-0060(A)  & 06-04-07 & PAH2 & 11.25 &  0.59 &     1059 &  0.40 &  0.35 &       93 &  0.53 &  0.48 &       48 &    121.4 $\pm$    18.7 &     69.0 $\pm$    15.4\\
NGC4418 & VISIR &  077.B-0060(A)  & 06-04-07 & Q2 & 18.72 &  0.88 &     1386 &  0.52 &  0.49 &       84 &  0.55 &  0.54 &      115 &   1949.5 $\pm$    90.2 &   1646.0 $\pm$    34.7\\
NGC4418 & TRECS &  GS-2004A-C-2  & 04-05-07 & Si6 & 12.33 &  0.59 &      108 &  0.48 &  0.40 &        2 &  0.60 &  0.52 &      171 &    899.8 $\pm$    18.5 &    554.7 $\pm$    15.7\\
NGC4438 & TRECS &  GS-2007B-Q-203  & 08-02-20 & Si2 &  8.74 &  0.39 &      926 &  0.54 &  0.47 &       51 &  $\dots$  &  $\dots$  &  $\dots$  &      8.5 $\pm$     0.5 &      8.5 $\pm$     0.5\\
NGC4438 & TRECS &  GS-2007B-Q-203  & 08-07-03 & Si2 &  8.74 &  0.39 &      926 &  0.47 &  0.45 &      130 &  $\dots$  &  $\dots$  &  $\dots$  &      8.0 $\pm$     0.3 &      8.0 $\pm$     0.3\\
NGC4457 & TRECS &  GS-2007B-Q-203  & 08-02-20 & Si2 &  8.74 &  0.39 &      926 &  0.49 &  0.41 &       55 &  1.00 &  1.00 &      170 &     20.4 $\pm$     0.8 &      4.8 $\pm$     0.7\\
NGC4457 & TRECS &  GS-2007B-Q-203  & 08-03-27 & Si2 &  8.74 &  0.39 &      926 &  0.40 &  0.33 &       63 &  1.00 &  0.78 &       36 &     15.9 $\pm$     1.4 &      4.9 $\pm$     1.4\\
NGC4472 & VISIR &  077.B-0137(A)  & 06-04-18 & NEII\_1 & 12.27 &  0.18 &     2524 &  0.35 &  0.35 &       60 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.8   &  $\le$     7.8  \\
NGC4501 & TRECS &  GS-2004A-Q-14  & 04-03-05 & N & 10.36 &  2.64 &      716 &  0.45 &  0.40 &      137 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     2.7   &      2.7 $\pm$     0.0\\
NGC4501 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      518 &  0.51 &  0.45 &       73 &  $\dots$  &  $\dots$  &  $\dots$  &      3.7 $\pm$     0.4 &      3.7 $\pm$     0.4\\
NGC4507 & VISIR &  077.B-0137(A)  & 06-04-15 & NEII\_1 & 12.27 &  0.18 &      180 &  0.37 &  0.33 &      136 &  0.35 &  0.35 &      145 &    622.8 $\pm$    16.0 &    621.0 $\pm$    15.3\\
NGC4507 & VISIR &  077.B-0137(A)  & 06-04-15 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.32 &      135 &  0.35 &  0.32 &       99 &    585.7 $\pm$    13.8 &    617.9 $\pm$    29.1\\
NGC4507 & VISIR &  077.B-0137(A)  & 06-04-15 & SIV & 10.49 &  0.16 &      176 &  0.37 &  0.32 &      137 &  0.33 &  0.31 &      105 &    518.9 $\pm$    25.6 &    544.8 $\pm$    80.9\\
NGC4579 & VISIR &  075.B-0844(C)  & 05-04-30 & NEII\_1 & 12.27 &  0.18 &      540 &  0.35 &  0.33 &       82 &  0.38 &  0.36 &       68 &     64.1 $\pm$    15.7 &     52.9 $\pm$     4.4\\
NGC4579 & VISIR &  075.B-0844(C)  & 05-04-30 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.33 &  0.32 &       70 &  0.36 &  0.35 &      177 &     68.6 $\pm$    13.2 &     56.7 $\pm$     6.2\\
NGC4579 & VISIR &  085.B-0639(D)  & 10-05-12 & Q2 & 18.72 &  0.88 &      828 &  0.47 &  0.46 &      139 &  0.46 &  0.44 &       45 &    101.1 $\pm$    11.5 &    110.1 $\pm$     8.9\\
NGC4579 & VISIR &  075.B-0844(C)  & 05-04-30 & SIV & 10.49 &  0.16 &      176 &  0.31 &  0.30 &      126 &  0.34 &  0.31 &       96 &     64.8 $\pm$    15.3 &     61.9 $\pm$     2.3\\
NGC4579 & VISIR &  085.B-0639(C)  & 11-05-07 & SIV\_2 & 10.77 &  0.19 &      361 &  0.45 &  0.35 &      153 &  0.41 &  0.32 &       11 &     71.3 $\pm$     8.2 &     86.5 $\pm$     2.2\\
NGC4579 & VISIR &  075.B-0844(C)  & 05-04-30 & PAH2 & 11.25 &  0.59 &      173 &  0.44 &  0.34 &      137 &  0.33 &  0.30 &        3 &     71.5 $\pm$     6.8 &    104.0 $\pm$    11.9\\
NGC4579 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-5 & 11.60 &  0.55 &      155 &  0.40 &  0.37 &       78 &  0.60 &  0.48 &       41 &     77.4 $\pm$     2.8 &     39.8 $\pm$     2.7\\
NGC4579 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      141 &  0.41 &  0.39 &       35 &  0.53 &  0.45 &       36 &     71.6 $\pm$     3.2 &     48.6 $\pm$     3.2\\
NGC4579 & VISIR &  083.B-0536(B)  & 09-05-04 & PAH1 &  8.59 &  0.42 &     1035 &  0.50 &  0.45 &       63 &  $\dots$  &  $\dots$  &  $\dots$  &     25.0 $\pm$     8.2 &     21.6 $\pm$     7.1\\
NGC4593 & VISIR &  080.B-0240(A)  & 08-04-01 & ARIII &  8.99 &  0.14 &      228 &  0.28 &  0.28 &      109 &  0.37 &  0.30 &      122 &    191.5 $\pm$     2.4 &    129.8 $\pm$     7.5\\
NGC4593 & VISIR &  384.B-0143(A)  & 10-03-05 & NEII & 12.81 &  0.21 &      141 &  0.38 &  0.34 &       77 &  0.42 &  0.38 &      115 &    276.4 $\pm$    59.1 &    225.6 $\pm$    27.0\\
NGC4593 & VISIR &  385.B-0051(A)  & 10-04-23 & NEII & 12.81 &  0.21 &      140 &  0.37 &  0.35 &       18 &  0.42 &  0.37 &       71 &    254.7 $\pm$    29.7 &    216.9 $\pm$     6.4\\
NGC4593 & VISIR &  385.B-0051(A)  & 10-06-16 & NEII & 12.81 &  0.21 &      140 &  0.39 &  0.36 &      124 &  0.37 &  0.36 &      111 &    275.6 $\pm$    25.3 &    289.0 $\pm$    17.1\\
NGC4593 & VISIR &  075.B-0844(C)  & 05-04-30 & NEII\_1 & 12.27 &  0.18 &      360 &  0.35 &  0.33 &       82 &  0.39 &  0.34 &      112 &    373.8 $\pm$     9.2 &    311.4 $\pm$    37.3\\
NGC4593 & VISIR &  385.B-0051(A)  & 10-04-23 & PAH1 &  8.59 &  0.42 &      141 &  0.28 &  0.26 &      177 &  0.33 &  0.29 &       77 &    145.9 $\pm$     5.3 &    111.1 $\pm$     3.5\\
NGC4593 & VISIR &  075.B-0844(C)  & 05-04-30 & PAH2\_2 & 11.88 &  0.37 &      361 &  0.33 &  0.32 &       70 &  0.37 &  0.31 &      107 &    340.1 $\pm$    12.9 &    309.7 $\pm$    11.0\\
NGC4593 & VISIR &  080.B-0240(A)  & 08-04-01 & PAH2\_2 & 11.88 &  0.37 &      235 &  0.33 &  0.31 &      154 &  0.38 &  0.34 &      118 &    287.2 $\pm$     7.4 &    228.9 $\pm$     6.7\\
NGC4593 & VISIR &  384.B-0143(A)  & 10-03-05 & PAH2\_2 & 11.88 &  0.37 &      141 &  0.35 &  0.32 &       73 &  0.39 &  0.37 &      131 &    243.0 $\pm$     9.7 &    188.6 $\pm$     3.9\\
NGC4593 & VISIR &  385.B-0051(A)  & 10-04-23 & PAH2\_2 & 11.88 &  0.37 &      141 &  0.34 &  0.31 &       12 &  0.38 &  0.35 &       67 &    238.5 $\pm$    16.3 &    192.3 $\pm$     6.5\\
NGC4593 & VISIR &  385.B-0051(A)  & 10-06-16 & PAH2\_2 & 11.88 &  0.37 &      282 &  0.39 &  0.35 &      138 &  0.36 &  0.35 &       83 &    252.5 $\pm$     3.0 &    277.0 $\pm$     3.5\\
NGC4593 & VISIR &  080.B-0240(A)  & 08-04-01 & Q1 & 17.65 &  0.83 &     1368 &  0.46 &  0.44 &       94 &  0.52 &  0.47 &      111 &    429.3 $\pm$    10.7 &    352.3 $\pm$     7.8\\
NGC4593 & VISIR &  075.B-0844(C)  & 05-04-30 & SIV & 10.49 &  0.16 &      353 &  0.31 &  0.30 &      126 &  0.36 &  0.29 &      111 &    344.4 $\pm$     5.2 &    312.8 $\pm$    11.1\\
NGC4594 & VISIR &  083.B-0536(C)  & 09-06-18 & NEII\_1 & 12.27 &  0.18 &      901 &  0.34 &  0.33 &       59 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    10.8   &  $\le$    10.8  \\
NGC4594 & VISIR &  083.B-0536(C)  & 09-06-18 & PAH2 & 11.25 &  0.59 &      362 &  0.33 &  0.30 &       71 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.7   &  $\le$     6.7  \\
NGC4594 & VISIR &  076.B-0599(A)  & 06-03-22 & PAH2\_2 & 11.88 &  0.37 &      722 &  0.52 &  0.37 &       96 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    22.0   &  $\le$    22.0  \\
NGC4594 & VISIR &  384.B-0943(A)  & 10-02-22 & PAH2\_2 & 11.88 &  0.37 &     1812 &  0.38 &  0.33 &        5 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     9.1   &  $\le$     9.1  \\
NGC4594 & TRECS &  GS-2007B-Q-203  & 08-02-20 & Si2 &  8.74 &  0.39 &      926 &  0.49 &  0.41 &       55 &  $\dots$  &  $\dots$  &  $\dots$  &      3.7 $\pm$     0.4 &      3.7 $\pm$     0.4\\
NGC4594 & TRECS &  GS-2007B-Q-203  & 08-03-27 & Si2 &  8.74 &  0.39 &      926 &  0.48 &  0.44 &       34 &  $\dots$  &  $\dots$  &  $\dots$  &      4.6 $\pm$     0.5 &      4.6 $\pm$     0.5\\
NGC4594 & TRECS &  GS-2007B-Q-203  & 08-04-10 & Si2 &  8.74 &  0.39 &      926 &  0.46 &  0.37 &       36 &  $\dots$  &  $\dots$  &  $\dots$  &      3.6 $\pm$     0.3 &      3.6 $\pm$     0.3\\
NGC4594 & TRECS &  GS-2007B-Q-203  & 08-05-02 & Si2 &  8.74 &  0.39 &      926 &  0.37 &  0.33 &       26 &  $\dots$  &  $\dots$  &  $\dots$  &      3.0 $\pm$     0.3 &      3.0 $\pm$     0.3\\
NGC4636 & VISIR &  384.B-0943(A)  & 10-02-23 & PAH2\_2 & 11.88 &  0.37 &      905 &  0.40 &  0.34 &       12 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    16.3   &  $\le$    16.3  \\
NGC4636 & VISIR &  384.B-0943(A)  & 10-03-24 & PAH2\_2 & 11.88 &  0.37 &      906 &  0.56 &  0.51 &       94 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    28.6   &  $\le$    28.6  \\
NGC4636 & VISIR &  384.B-0943(A)  & 10-04-01 & PAH2\_2 & 11.88 &  0.37 &      902 &  0.32 &  0.31 &      170 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.9   &  $\le$     7.9  \\
NGC4698 & VISIR &  077.B-0137(A)  & 06-04-18 & NEII\_1 & 12.27 &  0.18 &     2524 &  0.35 &  0.35 &       60 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.6   &  $\le$     7.6  \\
NGC4736 & MICHELLE &  GN-2007A-Q-93  & 07-04-15 & N\_prime & 11.20 &  1.20 &      611 &  0.55 &  0.53 &      140 &  1.00 &  1.00 &      164 &     23.5 $\pm$     0.6 &      7.0 $\pm$     0.5\\
NGC4736 & MICHELLE &  GN-2007A-Q-93  & 07-04-16 & Qa & 18.10 &  0.95 &      608 &  0.81 &  0.72 &       10 &  1.00 &  0.87 &       48 &     87.6 $\pm$    19.0 &     57.1 $\pm$    19.0\\
NGC4746 & VISIR &  60.A-9244(A)  & 05-01-31 & PAH2 & 11.25 &  0.59 &     1766 &  0.37 &  0.34 &      175 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.8   &  $\le$     7.8  \\
NGC4785 & VISIR &  60.A-9244(A)  & 05-01-28 & PAH2 & 11.25 &  0.59 &     1766 &  0.38 &  0.37 &      116 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.0   &  $\le$    13.0  \\
NGC4941 & VISIR &  077.B-0137(A)  & 06-04-19 & NEII\_1 & 12.27 &  0.18 &     1622 &  0.36 &  0.35 &      100 &  0.39 &  0.33 &      121 &     76.1 $\pm$     4.3 &     75.2 $\pm$     3.3\\
NGC4941 & VISIR &  085.B-0639(C)  & 10-04-02 & PAH1 &  8.59 &  0.42 &      118 &  0.34 &  0.30 &      148 &  0.28 &  0.26 &      103 &     36.9 $\pm$     9.0 &     47.8 $\pm$     5.9\\
NGC4941 & VISIR &  083.B-0536(A)  & 09-05-12 & PAH2 & 11.25 &  0.59 &      724 &  0.32 &  0.31 &      176 &  0.37 &  0.31 &      111 &     66.0 $\pm$     4.1 &     57.3 $\pm$     2.0\\
NGC4941 & VISIR &  085.B-0639(D)  & 10-04-02 & Q2 & 18.72 &  0.88 &      684 &  0.51 &  0.48 &      122 &  0.53 &  0.48 &      140 &    232.0 $\pm$    17.1 &    216.4 $\pm$    14.9\\
NGC4941 & VISIR &  085.B-0639(C)  & 10-04-02 & SIV\_2 & 10.77 &  0.19 &      541 &  0.37 &  0.33 &      153 &  0.35 &  0.30 &      113 &     65.4 $\pm$    12.1 &     79.3 $\pm$     8.5\\
NGC4945 & VISIR &  077.B-0060(B)  & 06-04-18 & PAH2 & 11.25 &  0.59 &      529 &  0.42 &  0.35 &      121 &  1.00 &  0.71 &       60 &     63.2 $\pm$     7.9 &     13.1 $\pm$     7.7\\
NGC4945 & VISIR &  077.B-0060(B)  & 06-04-18 & Q2 & 18.72 &  0.88 &     1396 &  0.54 &  0.49 &       46 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   221.3   &  $\le$    98.3  \\
NGC4945 & TRECS &  GS-2006A-Q-62  & 06-03-17 & Qa & 18.30 &  0.76 &      260 &  0.62 &  0.57 &      136 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   126.6   &  $\le$    95.0  \\
NGC4945 & TRECS &  GS-2006A-Q-62  & 06-03-17 & Si2 &  8.74 &  0.39 &      260 &  0.44 &  0.39 &      138 &  1.00 &  0.78 &       44 &    107.6 $\pm$     5.6 &     23.4 $\pm$     5.5\\
NGC4945 & VISIR &  077.B-0060(B)  & 06-04-18 & PAH1 &  8.59 &  0.42 &      345 &  0.32 &  0.30 &       34 &  1.00 &  0.89 &       44 &    170.8 $\pm$    14.5 &     18.0 $\pm$    13.9\\
NGC4992 & VISIR &  080.B-0860(A)  & 08-03-21 & NEII & 12.81 &  0.21 &      101 &  0.33 &  0.32 &       78 &  0.43 &  0.36 &      142 &     80.3 $\pm$    15.8 &     55.7 $\pm$    15.8\\
NGC4992 & VISIR &  080.B-0860(A)  & 08-03-21 & PAH1 &  8.59 &  0.42 &      102 &  0.38 &  0.37 &       91 &  0.47 &  0.37 &       71 &     55.6 $\pm$     7.3 &     45.0 $\pm$     7.3\\
NGC4992 & VISIR &  080.B-0860(A)  & 08-03-21 & PAH2 & 11.25 &  0.59 &      102 &  0.36 &  0.31 &      110 &  0.47 &  0.30 &      175 &     35.4 $\pm$     8.1 &     27.8 $\pm$     8.1\\
NGC4992 & VISIR &  080.B-0860(A)  & 08-03-21 & SIV & 10.49 &  0.16 &      101 &  0.36 &  0.34 &      125 &  $\dots$  &  $\dots$  &  $\dots$  &     33.0 $\pm$     3.6 &     33.0 $\pm$     3.6\\
NGC5005 & MICHELLE &  GN-2008A-Q-43  & 08-06-12 & N\_prime & 11.20 &  1.20 &      470 &  0.70 &  0.55 &       52 &  1.00 &  0.98 &       82 &     15.5 $\pm$     1.6 &      6.1 $\pm$     1.6\\
NGC5033 & MICHELLE &  GN-2008A-Q-43  & 08-06-16 & N\_prime & 11.20 &  1.20 &      470 &  0.37 &  0.36 &       72 &  0.42 &  0.39 &       87 &     16.2 $\pm$     0.7 &     13.4 $\pm$     0.7\\
NGC5033 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      518 &  0.51 &  0.45 &       73 &  0.57 &  0.46 &       16 &     17.7 $\pm$     2.0 &     15.9 $\pm$     2.0\\
NGC5135 & VISIR &  081.B-0182(A)  & 08-04-20 & B11.7 & 11.52 &  0.85 &     2163 &  0.44 &  0.38 &      132 &  0.43 &  0.38 &      138 &     95.4 $\pm$     6.5 &     87.7 $\pm$    23.6\\
NGC5135 & VISIR &  076.B-0696(A)  & 06-01-19 & NEII & 12.81 &  0.21 &     7072 &  0.51 &  0.46 &       84 &  0.45 &  0.40 &      110 &    156.8 $\pm$     3.4 &    196.0 $\pm$    17.0\\
NGC5135 & VISIR &  077.B-0137(A)  & 06-04-09 & NEII\_1 & 12.27 &  0.18 &     2524 &  0.37 &  0.33 &       83 &  0.36 &  0.34 &       15 &    121.9 $\pm$     2.7 &    120.5 $\pm$     5.9\\
NGC5135 & VISIR &  081.B-0182(A)  & 08-05-13 & NEII\_1 & 12.27 &  0.18 &     2070 &  0.37 &  0.36 &      157 &  0.48 &  0.44 &       70 &    140.5 $\pm$    11.3 &     85.6 $\pm$    15.5\\
NGC5135 & VISIR &  076.B-0696(A)  & 06-01-19 & NEII\_2 & 13.04 &  0.22 &     3670 &  0.44 &  0.40 &      122 &  0.52 &  0.47 &        5 &    142.9 $\pm$     5.1 &    104.6 $\pm$     4.4\\
NGC5135 & VISIR &  081.B-0182(A)  & 08-05-13 & NEII\_2 & 13.04 &  0.22 &     2070 &  0.40 &  0.38 &      140 &  0.50 &  0.46 &       37 &    179.0 $\pm$     9.4 &    114.0 $\pm$     7.7\\
NGC5135 & TRECS &  GS-2005B-Q-10  & 06-03-04 & N & 10.36 &  2.64 &      608 &  $\dots$  &  $\dots$  &  $\dots$  &  0.42 &  0.40 &       67 &     65.2 $\pm$    11.4 &  $\le$    98.2  \\
NGC5135 & VISIR &  081.B-0182(A)  & 08-04-20 & SIV & 10.49 &  0.16 &     1624 &  0.45 &  0.39 &      135 &  0.42 &  0.36 &       91 &     59.1 $\pm$     7.4 &     68.7 $\pm$    15.6\\
NGC5135 & VISIR &  077.B-0137(A)  & 06-04-09 & SIV & 10.49 &  0.16 &       84 &  0.31 &  0.29 &       94 &  0.40 &  0.39 &       67 &     89.9 $\pm$    18.9 &     35.4 $\pm$    18.9\\
NGC5252 & VISIR &  084.B-0606(A)  & 10-02-21 & NEII & 12.81 &  0.21 &      724 &  0.39 &  0.34 &       99 &  0.40 &  0.37 &      165 &     85.5 $\pm$    13.1 &     75.7 $\pm$     6.0\\
NGC5252 & VISIR &  084.B-0606(A)  & 10-02-21 & PAH2\_2 & 11.88 &  0.37 &      362 &  0.38 &  0.31 &       95 &  0.35 &  0.33 &      117 &     88.6 $\pm$     6.4 &     93.6 $\pm$     8.5\\
NGC5252 & VISIR &  084.B-0606(A)  & 10-02-21 & SIV & 10.49 &  0.16 &      360 &  0.31 &  0.29 &      155 &  0.35 &  0.32 &      152 &     90.3 $\pm$     3.8 &     72.3 $\pm$     3.7\\
NGC5258 & VISIR &  60.A-9244(A)  & 05-02-02 & PAH2 & 11.25 &  0.59 &     1766 &  0.37 &  0.36 &       42 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    13.4   &  $\le$    13.4  \\
NGC5273 & MICHELLE &  GN-2010A-C-7  & 10-02-02 & Si-5 & 11.60 &  0.55 &      259 &  0.49 &  0.48 &       87 &  $\dots$  &  $\dots$  &  $\dots$  &     20.1 $\pm$     0.9 &     20.3 $\pm$     0.9\\
NGC5273 & MICHELLE &  GN-2010A-C-7  & 10-02-04 & Si-6 & 12.50 &  0.60 &      282 &  0.41 &  0.39 &       35 &  0.53 &  0.47 &       96 &     27.7 $\pm$     2.7 &     17.6 $\pm$     2.7\\
NGC5347 & MICHELLE &  GN-2006A-Q-11  & 07-03-19 & N\_prime & 11.20 &  1.20 &      188 &  0.68 &  0.42 &      168 &  0.52 &  0.47 &        4 &    238.0 $\pm$     4.9 &    280.8 $\pm$     5.4\\
NGC5347 & MICHELLE &  GN-2006A-Q-11  & 07-03-19 & Qa & 18.10 &  0.95 &      162 &  $\dots$  &  $\dots$  &  $\dots$  &  0.63 &  0.57 &      177 &    871.1 $\pm$   106.7 &  $\le$  1191.3  \\
NGC5363 & VISIR &  083.B-0536(C)  & 09-05-11 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.40 &  0.38 &      147 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    14.1   &  $\le$    14.1  \\
NGC5363 & VISIR &  083.B-0536(C)  & 09-05-11 & PAH2 & 11.25 &  0.59 &      543 &  0.35 &  0.31 &      113 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.5   &  $\le$     6.5  \\
NGC5363 & MICHELLE &  GN-2008A-Q-43  & 08-07-11 & N\_prime & 11.20 &  1.20 &      470 &  0.36 &  0.33 &       28 &  1.00 &  0.78 &       42 &     10.0 $\pm$     1.3 &      1.6 $\pm$     1.2\\
NGC5427 & VISIR &  60.A-9244(A)  & 05-02-03 & PAH2 & 11.25 &  0.59 &     1794 &  0.41 &  0.39 &      136 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    15.0   &  $\le$    15.0  \\
NGC5506 & VISIR &  084.B-0606(A)  & 10-02-23 & NEII\_1 & 12.27 &  0.18 &      181 &  0.34 &  0.33 &      147 &  0.40 &  0.39 &       16 &   1191.8 $\pm$    17.3 &    883.1 $\pm$    45.4\\
NGC5506 & VISIR &  084.B-0606(A)  & 10-02-23 & NEII\_2 & 13.04 &  0.22 &      181 &  0.36 &  0.36 &      115 &  0.41 &  0.39 &       74 &   1392.6 $\pm$    50.8 &   1119.3 $\pm$    44.5\\
NGC5506 & VISIR &  084.B-0606(A)  & 10-02-23 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.32 &       98 &  0.41 &  0.38 &       45 &    871.7 $\pm$    18.3 &    591.5 $\pm$    97.5\\
NGC5506 & VISIR &  60.A-9244(A)  & 05-02-02 & PAH2 & 11.25 &  0.59 &     1589 &  0.37 &  0.36 &       42 &  0.41 &  0.39 &       35 &    823.4 $\pm$    12.7 &    644.8 $\pm$    28.9\\
NGC5506 & VISIR &  076.B-0599(A)  & 06-03-15 & PAH2\_2 & 11.88 &  0.37 &      362 &  0.33 &  0.32 &       26 &  0.38 &  0.34 &       92 &    866.4 $\pm$    23.6 &    727.5 $\pm$    68.8\\
NGC5506 & VISIR &  077.B-0728(A)  & 06-06-06 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.38 &  0.33 &      107 &  0.39 &  0.34 &       80 &    938.6 $\pm$    22.3 &    883.7 $\pm$    23.0\\
NGC5506 & VISIR &  076.B-0599(A)  & 06-03-13 & Q2 & 18.72 &  0.88 &      513 &  0.57 &  0.57 &      104 &  0.66 &  0.60 &      104 &   2125.3 $\pm$   242.6 &   1744.5 $\pm$   230.1\\
NGC5506 & VISIR &  076.B-0599(A)  & 06-03-22 & Q2 & 18.72 &  0.88 &      513 &  0.52 &  0.49 &       81 &  0.54 &  0.49 &      109 &   1746.0 $\pm$   107.7 &   1687.2 $\pm$    43.8\\
NGC5506 & VISIR &  077.B-0728(A)  & 06-06-06 & Q2 & 18.72 &  0.88 &     1026 &  0.50 &  0.47 &       99 &  0.55 &  0.51 &       73 &   1801.2 $\pm$    63.9 &   1519.6 $\pm$    44.0\\
NGC5506 & TRECS &  GS-2004A-C-2  & 04-05-06 & Si6 & 12.33 &  0.59 &      108 &  $\dots$  &  $\dots$  &  $\dots$  &  0.55 &  0.44 &      173 &   1088.7 $\pm$   233.3 &  $\le$  1788.7  \\
NGC5506 & MICHELLE &  GN-2006A-Q-11  & 06-04-06 & N\_prime & 11.20 &  1.20 &      141 &  0.53 &  0.43 &      170 &  0.49 &  0.42 &        1 &    879.5 $\pm$    14.9 &    981.8 $\pm$    15.7\\
NGC5506 & MICHELLE &  GN-2006A-Q-11  & 06-04-06 & Qa & 18.10 &  0.95 &      108 &  0.56 &  0.52 &      158 &  0.60 &  0.56 &        9 &   2084.3 $\pm$    34.2 &   1800.6 $\pm$    32.7\\
NGC5548 & VISIR &  085.B-0251(C)  & 10-06-27 & ARIII &  8.99 &  0.14 &      176 &  0.35 &  0.31 &       14 &  0.81 &  0.65 &       37 &    132.8 $\pm$    16.7 &     27.3 $\pm$    16.5\\
NGC5548 & VISIR &  085.B-0251(C)  & 10-06-27 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.41 &  0.37 &       13 &  0.66 &  0.50 &       13 &    169.7 $\pm$    49.1 &     77.9 $\pm$     8.1\\
NGC5643 & VISIR &  083.B-0239(B)  & 09-05-03 & ARIII &  8.99 &  0.14 &       83 &  0.30 &  0.27 &      137 &  0.39 &  0.33 &       24 &    129.0 $\pm$    16.8 &     80.0 $\pm$    16.7\\
NGC5643 & VISIR &  083.B-0239(B)  & 09-05-03 & PAH2\_2 & 11.88 &  0.37 &       86 &  0.34 &  0.32 &      140 &  0.43 &  0.35 &       57 &    293.6 $\pm$     7.6 &    214.6 $\pm$    18.1\\
NGC5643 & VISIR &  083.B-0239(B)  & 09-05-03 & NEII\_2 & 13.04 &  0.22 &       31 &  $\dots$  &  $\dots$  &  $\dots$  &  0.48 &  0.38 &       60 &    420.1 $\pm$    56.0 &  $\le$   588.1  \\
NGC5728 & VISIR &  084.B-0606(A)  & 10-03-12 & NEII\_1 & 12.27 &  0.18 &     1448 &  0.42 &  0.35 &      127 &  0.49 &  0.41 &       80 &     69.2 $\pm$     2.4 &     49.1 $\pm$     5.2\\
NGC5728 & VISIR &  080.B-0860(A)  & 08-03-21 & NEII\_2 & 13.04 &  0.22 &       62 &  0.37 &  0.34 &      114 &  $\dots$  &  $\dots$  &  $\dots$  &     93.0 $\pm$     7.9 &     92.8 $\pm$     7.9\\
NGC5728 & VISIR &  080.B-0860(A)  & 08-03-21 & PAH1 &  8.59 &  0.42 &       62 &  0.38 &  0.37 &       91 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    38.7   &  $\le$    38.7  \\
NGC5728 & VISIR &  084.B-0606(A)  & 10-03-12 & PAH2 & 11.25 &  0.59 &      362 &  0.39 &  0.33 &      118 &  0.43 &  0.35 &       90 &     24.2 $\pm$     3.3 &     20.8 $\pm$     3.3\\
NGC5728 & TRECS &  GS-2005A-Q-6  & 05-07-09 & Qa & 18.30 &  0.76 &      304 &  0.56 &  0.55 &      132 &  0.70 &  0.67 &      128 &    190.0 $\pm$    33.9 &    122.6 $\pm$    33.8\\
NGC5728 & TRECS &  GS-2005A-Q-6  & 05-07-08 & Si2 &  8.74 &  0.39 &      130 &  0.52 &  0.45 &       45 &  0.75 &  0.65 &      130 &     24.0 $\pm$     3.9 &     12.0 $\pm$     3.9\\
NGC5728 & VISIR &  080.B-0860(A)  & 08-03-21 & SIV & 10.49 &  0.16 &       62 &  0.36 &  0.34 &      125 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    58.8   &  $\le$    58.8  \\
NGC5813 & VISIR &  083.B-0536(A)  & 09-05-11 & NEII\_1 & 12.27 &  0.18 &      180 &  0.40 &  0.38 &      147 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    48.0   &  $\le$    48.0  \\
NGC5813 & VISIR &  083.B-0536(A)  & 09-05-11 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.33 &      162 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    15.4   &  $\le$    15.4  \\
NGC5866 & MICHELLE &  GN-2008A-Q-43  & 08-06-13 & N\_prime & 11.20 &  1.20 &      470 &  0.61 &  0.54 &       33 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.4   &  $\le$     6.4  \\
NGC5953 & TRECS &  GS-2004A-Q-14  & 04-05-03 & N & 10.36 &  2.64 &      716 &  0.40 &  0.37 &      132 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    18.2   &     12.2 $\pm$     0.0\\
NGC5995 & VISIR &  077.B-0137(A)  & 06-04-14 & NEII & 12.81 &  0.21 &      179 &  0.46 &  0.34 &       83 &  0.44 &  0.36 &       91 &    384.6 $\pm$    23.1 &    375.5 $\pm$    26.5\\
NGC5995 & VISIR &  077.B-0137(A)  & 06-04-14 & PAH2 & 11.25 &  0.59 &      181 &  0.39 &  0.30 &       84 &  0.45 &  0.33 &      100 &    326.4 $\pm$    10.1 &    259.1 $\pm$    10.2\\
NGC5995 & VISIR &  085.B-0251(C)  & 10-07-26 & PAH2 & 11.25 &  0.59 &     2174 &  0.33 &  0.31 &      147 &  0.33 &  0.31 &      154 &    314.3 $\pm$    11.0 &    324.0 $\pm$    11.6\\
NGC5995 & VISIR &  085.B-0251(C)  & 10-07-26 & PAH2\_2 & 11.88 &  0.37 &     2166 &  0.37 &  0.33 &      160 &  0.36 &  0.33 &       72 &    323.5 $\pm$     9.5 &    316.3 $\pm$    11.5\\
NGC5995 & VISIR &  077.B-0137(A)  & 06-04-14 & SIV & 10.49 &  0.16 &      176 &  0.48 &  0.31 &       82 &  0.47 &  0.33 &       97 &    270.5 $\pm$    10.1 &    271.9 $\pm$    19.9\\
NGC6221 & TRECS &  GS-2009B-Q-43  & 09-08-28 & Qa & 18.30 &  0.76 &      202 &  0.56 &  0.55 &       43 &  1.00 &  0.62 &        8 &    546.4 $\pm$    48.0 &    190.5 $\pm$    44.0\\
NGC6221 & TRECS &  GS-2009B-Q-43  & 09-08-28 & Si2 &  8.74 &  0.39 &      144 &  0.40 &  0.39 &      165 &  0.56 &  0.48 &       38 &     92.4 $\pm$     8.9 &     57.8 $\pm$     8.9\\
NGC6240N & VISIR &  075.B-0791(A)  & 05-04-19 & PAH2 & 11.25 &  0.59 &     1794 &  0.69 &  0.61 &      159 &  $\dots$  &  $\dots$  &  $\dots$  &     27.8 $\pm$     4.1 &     27.6 $\pm$     6.9\\
NGC6240N & VISIR &  075.B-0791(A)  & 05-04-19 & PAH2\_2 & 11.88 &  0.37 &     1766 &  0.57 &  0.46 &      167 &  $\dots$  &  $\dots$  &  $\dots$  &     29.2 $\pm$     4.3 &     17.3 $\pm$     7.2\\
NGC6240N & VISIR &  075.B-0727(A)  & 05-06-15 & Q2 & 18.72 &  0.88 &     3666 &  0.56 &  0.55 &      122 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    75.1   &  $\le$    75.0  \\
NGC6240S & VISIR &  075.B-0791(A)  & 05-04-19 & PAH2 & 11.25 &  0.59 &     1794 &  0.69 &  0.61 &      159 &  0.64 &  0.48 &      162 &    151.7 $\pm$    12.3 &     99.5 $\pm$     8.4\\
NGC6240S & VISIR &  075.B-0791(A)  & 05-04-19 & PAH2\_2 & 11.88 &  0.37 &     1766 &  0.57 &  0.46 &      167 &  0.95 &  0.72 &      158 &    303.2 $\pm$    16.4 &     92.9 $\pm$     4.8\\
NGC6240S & VISIR &  075.B-0727(A)  & 05-06-15 & Q2 & 18.72 &  0.88 &     3666 &  0.56 &  0.55 &      122 &  0.77 &  0.65 &      168 &    590.2 $\pm$   111.0 &    370.0 $\pm$    72.6\\
NGC6251 & COMICS &  o09108  & 09-05-04 & N11.7 & 11.74 &  0.53 &     2406 &  0.38 &  0.37 &      159 &  0.57 &  0.37 &      145 &     14.3 $\pm$     3.5 &      7.6 $\pm$     3.5\\
NGC6300 & VISIR &  080.B-0860(A)  & 08-03-22 & NEII\_2 & 13.04 &  0.22 &      361 &  0.36 &  0.36 &       61 &  0.50 &  0.41 &      108 &    608.2 $\pm$    12.6 &    385.4 $\pm$     9.0\\
NGC6300 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH1 &  8.59 &  0.42 &      362 &  0.29 &  0.26 &      153 &  0.45 &  0.35 &      111 &    217.8 $\pm$    10.4 &    104.2 $\pm$    12.0\\
NGC6300 & VISIR &  080.B-0860(A)  & 08-03-22 & PAH2 & 11.25 &  0.59 &      362 &  0.36 &  0.35 &       57 &  0.43 &  0.36 &      111 &    266.5 $\pm$    14.9 &    220.0 $\pm$    13.2\\
NGC6300 & VISIR &  080.B-0860(A)  & 08-03-22 & SIV & 10.49 &  0.16 &      721 &  0.31 &  0.30 &      132 &  0.44 &  0.41 &      122 &    153.2 $\pm$     3.3 &     76.1 $\pm$     1.3\\
NGC6810 & TRECS &  GS-2004A-Q-14  & 04-07-08 & N & 10.36 &  2.64 &      716 &  0.35 &  0.35 &      111 &  0.77 &  0.55 &      164 &    244.8 $\pm$     4.4 &     35.3 $\pm$     3.6\\
NGC6814 & VISIR &  080.B-0860(A)  & 07-10-20 & NEII\_2 & 13.04 &  0.22 &      543 &  0.43 &  0.40 &      161 &  0.51 &  0.43 &      100 &     95.6 $\pm$    23.5 &     75.9 $\pm$     5.9\\
NGC6814 & VISIR &  080.B-0860(A)  & 07-10-20 & PAH1 &  8.59 &  0.42 &      543 &  0.53 &  0.51 &      153 &  0.58 &  0.41 &       97 &     54.6 $\pm$     3.8 &     60.3 $\pm$     4.1\\
NGC6814 & VISIR &  080.B-0860(A)  & 07-10-20 & PAH2 & 11.25 &  0.59 &      543 &  0.41 &  0.40 &       48 &  0.49 &  0.39 &       89 &    102.5 $\pm$     6.7 &     85.5 $\pm$     5.9\\
NGC6814 & TRECS &  GS-2009B-Q-43  & 09-08-28 & Qa & 18.30 &  0.76 &      202 &  0.52 &  0.50 &      150 &  0.60 &  0.51 &       68 &    188.4 $\pm$    43.0 &    160.9 $\pm$    42.9\\
NGC6814 & TRECS &  GS-2009B-Q-43  & 09-08-28 & Si2 &  8.74 &  0.39 &      144 &  0.35 &  0.31 &      177 &  0.35 &  0.33 &      107 &     51.6 $\pm$     2.7 &     48.3 $\pm$     2.7\\
NGC6814 & VISIR &  080.B-0860(A)  & 07-10-20 & SIV & 10.49 &  0.16 &      529 &  0.41 &  0.38 &      170 &  0.61 &  0.46 &       99 &     96.9 $\pm$    10.2 &     54.5 $\pm$     6.8\\
NGC6860 & VISIR &  084.B-0606(A)  & 09-09-19 & NEII\_1 & 12.27 &  0.18 &      360 &  0.37 &  0.35 &      169 &  0.37 &  0.36 &       28 &    206.1 $\pm$    12.4 &    200.8 $\pm$    16.3\\
NGC6860 & VISIR &  084.B-0606(A)  & 09-09-19 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.34 &      127 &  0.34 &  0.34 &       14 &    208.7 $\pm$    10.4 &    229.3 $\pm$     7.7\\
NGC6860 & TRECS &  GS-2007A-DD-7  & 07-06-04 & Qa & 18.30 &  0.76 &      847 &  0.57 &  0.52 &        6 &  0.56 &  0.54 &      120 &    304.5 $\pm$    14.1 &    296.3 $\pm$    14.0\\
NGC6860 & TRECS &  GS-2008B-Q-36  & 08-09-17 & Si2 &  8.74 &  0.39 &      318 &  0.47 &  0.43 &      108 &  0.56 &  0.52 &      120 &    144.8 $\pm$     4.4 &     99.0 $\pm$     4.0\\
NGC6860 & VISIR &  084.B-0606(A)  & 09-09-19 & SIV\_2 & 10.77 &  0.19 &      543 &  0.40 &  0.36 &      165 &  0.38 &  0.33 &       34 &    208.6 $\pm$    12.5 &    222.8 $\pm$    16.1\\
NGC6890 & TRECS &  GS-2004A-Q-14  & 04-07-08 & N & 10.36 &  2.64 &      716 &  0.35 &  0.35 &      111 &  0.42 &  0.36 &      101 &     93.0 $\pm$     1.7 &     74.8 $\pm$     1.7\\
NGC7130 & VISIR &  083.B-0592(A)  & 09-07-03 & B11.7 & 11.52 &  0.85 &     2152 &  0.38 &  0.36 &       98 &  0.57 &  0.55 &      133 &    225.1 $\pm$     4.2 &     96.9 $\pm$     5.1\\
NGC7130 & VISIR &  083.B-0592(A)  & 09-07-03 & NEII\_1 & 12.27 &  0.18 &     2070 &  0.36 &  0.34 &       85 &  0.55 &  0.52 &       76 &    278.9 $\pm$    20.7 &    125.7 $\pm$     8.4\\
NGC7130 & VISIR &  083.B-0592(A)  & 09-07-03 & NEII\_2 & 13.04 &  0.22 &     2070 &  0.38 &  0.36 &       81 &  0.59 &  0.56 &      141 &    478.1 $\pm$    15.4 &    186.7 $\pm$     8.9\\
NGC7130 & TRECS &  GS-2004A-Q-14  & 04-07-08 & N & 10.36 &  2.64 &      716 &  0.35 &  0.35 &      111 &  0.59 &  0.57 &      141 &    160.5 $\pm$     3.5 &     58.4 $\pm$     3.2\\
NGC7130 & VISIR &  084.B-0974(A)  & 09-10-11 & PAH1 &  8.59 &  0.42 &     1380 &  0.31 &  0.28 &       75 &  0.70 &  0.66 &       90 &    137.1 $\pm$    10.1 &     26.1 $\pm$     1.3\\
NGC7130 & VISIR &  083.B-0592(A)  & 09-07-03 & SIV & 10.49 &  0.16 &     2172 &  0.40 &  0.35 &       96 &  0.50 &  0.45 &      105 &    105.0 $\pm$     9.3 &     65.5 $\pm$     4.3\\
NGC7130 & VISIR &  084.B-0974(A)  & 09-10-11 & SIV & 10.49 &  0.16 &     1986 &  0.39 &  0.36 &       45 &  0.52 &  0.47 &       31 &    118.6 $\pm$    10.1 &     69.2 $\pm$     3.7\\
NGC7172 & VISIR &  077.B-0137(A)  & 06-07-09 & NEII\_1 & 12.27 &  0.18 &      721 &  0.40 &  0.38 &       86 &  0.47 &  0.44 &       95 &    163.9 $\pm$     9.9 &    116.9 $\pm$     2.9\\
NGC7172 & VISIR &  084.B-0606(A)  & 09-09-20 & NEII\_2 & 13.04 &  0.22 &      180 &  0.37 &  0.35 &      116 &  0.43 &  0.36 &       81 &    190.7 $\pm$    10.9 &    160.9 $\pm$    14.5\\
NGC7172 & VISIR &  084.B-0606(A)  & 09-09-20 & PAH2 & 11.25 &  0.59 &      181 &  0.31 &  0.30 &      100 &  0.41 &  0.34 &       91 &     61.9 $\pm$     5.3 &     40.4 $\pm$     4.6\\
NGC7172 & TRECS &  GS-2004A-C-2  & 04-05-06 & Si6 & 12.33 &  0.59 &      108 &  $\dots$  &  $\dots$  &  $\dots$  &  0.75 &  0.53 &       73 &    164.3 $\pm$    36.2 &  $\le$   272.8  \\
NGC7212 & TRECS &  GS-2007A-DD-7  & 07-06-04 & Qa & 18.30 &  0.76 &      847 &  0.58 &  0.55 &      178 &  0.79 &  0.62 &      176 &    384.4 $\pm$    14.9 &    250.0 $\pm$    14.5\\
NGC7213 & VISIR &  384.B-0887(A)  & 09-09-11 & NEII & 12.81 &  0.21 &     1614 &  0.46 &  0.40 &       71 &  0.60 &  0.50 &      118 &    263.0 $\pm$     8.6 &    164.8 $\pm$    22.9\\
NGC7213 & VISIR &  077.B-0137(A)  & 06-07-14 & NEII\_1 & 12.27 &  0.18 &      180 &  0.33 &  0.32 &       72 &  0.39 &  0.36 &       75 &    254.8 $\pm$    15.0 &    192.7 $\pm$    10.1\\
NGC7213 & VISIR &  083.B-0536(A)  & 09-05-18 & NEII\_1 & 12.27 &  0.18 &      180 &  0.32 &  0.32 &      110 &  0.33 &  0.32 &      113 &    231.2 $\pm$    16.2 &    218.5 $\pm$     5.2\\
NGC7213 & VISIR &  384.B-0887(A)  & 09-09-11 & NEII\_1 & 12.27 &  0.18 &      540 &  0.48 &  0.41 &       67 &  0.68 &  0.54 &      110 &    251.8 $\pm$    22.6 &    139.1 $\pm$    15.6\\
NGC7213 & VISIR &  077.B-0137(A)  & 06-07-14 & PAH2 & 11.25 &  0.59 &      181 &  0.36 &  0.30 &      102 &  0.41 &  0.37 &       69 &    298.3 $\pm$    17.9 &    213.7 $\pm$     9.3\\
NGC7213 & VISIR &  083.B-0536(A)  & 09-05-18 & PAH2 & 11.25 &  0.59 &      181 &  0.30 &  0.29 &      113 &  0.32 &  0.29 &      112 &    232.4 $\pm$     6.4 &    218.4 $\pm$    11.2\\
NGC7213 & VISIR &  085.B-0639(D)  & 10-06-08 & Q2 & 18.72 &  0.88 &      331 &  0.56 &  0.49 &      134 &  0.54 &  0.52 &      102 &    446.9 $\pm$    40.1 &    427.9 $\pm$    28.1\\
NGC7213 & TRECS &  GS-2007A-DD-7  & 07-06-07 & Qa & 18.30 &  0.76 &      847 &  0.60 &  0.56 &        9 &  0.64 &  0.58 &      151 &    391.3 $\pm$    20.9 &    349.9 $\pm$    20.7\\
NGC7213 & TRECS &  GS-2008B-Q-36  & 08-09-17 & Si2 &  8.74 &  0.39 &      318 &  0.39 &  0.35 &        0 &  0.49 &  0.44 &      120 &     93.4 $\pm$     3.5 &     58.5 $\pm$     3.2\\
NGC7213 & TRECS &  GS-2010B-Q-71  & 10-08-20 & Si2 &  8.74 &  0.39 &      144 &  0.62 &  0.50 &       97 &  0.55 &  0.46 &      110 &     86.5 $\pm$     3.7 &    102.7 $\pm$     3.8\\
NGC7213 & TRECS &  GS-2010B-Q-71  & 10-12-17 & Si2 &  8.74 &  0.39 &      144 &  0.54 &  0.50 &       72 &  0.65 &  0.53 &       89 &     82.7 $\pm$     5.3 &     64.3 $\pm$     5.2\\
NGC7213 & VISIR &  077.B-0137(A)  & 06-07-14 & SIV & 10.49 &  0.16 &      176 &  0.32 &  0.29 &       97 &  0.35 &  0.32 &       82 &    248.1 $\pm$    15.8 &    200.8 $\pm$    17.0\\
NGC7314 & VISIR &  075.B-0844(C)  & 05-06-26 & PAH2 & 11.25 &  0.59 &      724 &  0.53 &  0.42 &      126 &  0.68 &  0.64 &       82 &     71.7 $\pm$     4.2 &     36.5 $\pm$     4.1\\
NGC7314 & VISIR &  075.B-0844(C)  & 05-07-20 & PAH2 & 11.25 &  0.59 &      724 &  0.39 &  0.34 &       99 &  0.46 &  0.39 &       74 &     73.1 $\pm$     3.3 &     53.1 $\pm$     3.2\\
NGC7314 & TRECS &  GS-2010B-Q-71  & 10-09-25 & Qa & 18.30 &  0.76 &      810 &  0.58 &  0.55 &       91 &  0.63 &  0.56 &       47 &    195.7 $\pm$    12.0 &    175.6 $\pm$    11.9\\
NGC7314 & TRECS &  GS-2010B-Q-71  & 10-08-20 & Si2 &  8.74 &  0.39 &      318 &  0.46 &  0.41 &       39 &  0.51 &  0.49 &      156 &     44.0 $\pm$     3.3 &     60.7 $\pm$     4.3\\
NGC7314 & VISIR &  075.B-0844(C)  & 05-06-26 & SIV & 10.49 &  0.16 &      706 &  0.53 &  0.43 &      123 &  0.59 &  0.51 &       60 &     76.0 $\pm$     1.2 &     57.4 $\pm$     1.4\\
NGC7314 & VISIR &  075.B-0844(C)  & 05-07-20 & SIV & 10.49 &  0.16 &      721 &  0.39 &  0.36 &      106 &  0.50 &  0.42 &       61 &     75.7 $\pm$     4.9 &     45.1 $\pm$     2.8\\
NGC7469 & VISIR &  077.B-0137(A)  & 06-07-12 & NEII\_1 & 12.27 &  0.18 &      180 &  0.36 &  0.35 &       91 &  0.39 &  0.36 &       83 &    597.1 $\pm$    17.6 &    527.3 $\pm$    20.8\\
NGC7469 & VISIR &  077.B-0137(A)  & 06-07-12 & PAH2 & 11.25 &  0.59 &      181 &  0.35 &  0.33 &      124 &  0.49 &  0.39 &       90 &    499.9 $\pm$    28.1 &    305.9 $\pm$    21.7\\
NGC7469 & VISIR &  077.B-0728(A)  & 06-06-15 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.35 &  0.32 &      111 &  0.39 &  0.35 &      108 &    494.3 $\pm$    15.8 &    412.7 $\pm$    24.1\\
NGC7469 & VISIR &  077.B-0728(A)  & 06-07-14 & PAH2\_2 & 11.88 &  0.37 &      541 &  0.35 &  0.32 &       89 &  0.38 &  0.32 &      116 &    532.0 $\pm$    15.2 &    493.1 $\pm$    16.9\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-08-26 & Q1 & 17.65 &  0.83 &      518 &  0.45 &  0.44 &       87 &  0.47 &  0.44 &       83 &   1070.4 $\pm$    20.3 &   1044.0 $\pm$    42.5\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-09-18 & Q1 & 17.65 &  0.83 &      684 &  0.49 &  0.46 &       92 &  0.52 &  0.52 &      155 &   1130.6 $\pm$   145.7 &    943.7 $\pm$   151.5\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-10-02 & Q1 & 17.65 &  0.83 &      684 &  0.52 &  0.47 &      110 &  0.55 &  0.49 &       87 &   1086.0 $\pm$    31.0 &    965.9 $\pm$    29.1\\
NGC7469 & VISIR &  077.B-0728(A)  & 06-06-15 & Q2 & 18.72 &  0.88 &      993 &  0.49 &  0.47 &      108 &  0.50 &  0.46 &      107 &   1306.2 $\pm$    36.8 &   1304.5 $\pm$    20.3\\
NGC7469 & VISIR &  077.B-0728(A)  & 06-08-06 & Q2 & 18.72 &  0.88 &      993 &  0.47 &  0.46 &       90 &  0.49 &  0.47 &       93 &   1269.3 $\pm$    47.7 &   1217.7 $\pm$    29.2\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-08-26 & Q3 & 19.50 &  0.40 &      522 &  0.51 &  0.48 &       93 &  0.53 &  0.51 &       93 &   1215.3 $\pm$   154.7 &   1122.8 $\pm$    94.3\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-09-18 & Q3 & 19.50 &  0.40 &      523 &  0.54 &  0.49 &       82 &  0.55 &  0.52 &      114 &   1221.1 $\pm$    83.4 &   1112.0 $\pm$    47.9\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-10-02 & Q3 & 19.50 &  0.40 &      519 &  0.56 &  0.50 &      106 &  0.55 &  0.51 &       78 &   1357.0 $\pm$    41.3 &   1365.1 $\pm$    77.0\\
NGC7469 & TRECS &  GS-2009B-Q-43  & 09-09-19 & Qa & 18.30 &  0.76 &      202 &  0.55 &  0.54 &       16 &  0.55 &  0.54 &      171 &   1342.8 $\pm$    43.8 &   1328.1 $\pm$    43.5\\
NGC7469 & TRECS &  GS-2009B-Q-43  & 09-09-19 & Si2 &  8.74 &  0.39 &      144 &  0.40 &  0.38 &       48 &  0.48 &  0.44 &        8 &    260.7 $\pm$     6.1 &    187.7 $\pm$     5.7\\
NGC7469 & VISIR &  077.B-0137(A)  & 06-07-12 & SIV & 10.49 &  0.16 &      176 &  0.34 &  0.31 &      139 &  0.44 &  0.34 &       86 &    448.5 $\pm$    14.1 &    316.5 $\pm$    45.5\\
NGC7469 & VISIR &  382.B-0732(A)  & 08-08-26 & NEII\_2 & 13.04 &  0.22 &       31 &  $\dots$  &  $\dots$  &  $\dots$  &  0.38 &  0.36 &       97 &    696.9 $\pm$    62.9 &  $\le$   885.7  \\
NGC7479 & MICHELLE &  GN-2008A-Q-43  & 08-07-01 & Si-2 &  8.80 &  0.45 &      933 &  0.38 &  0.35 &      145 &  0.38 &  0.33 &       81 &    157.9 $\pm$     1.7 &    166.9 $\pm$     1.8\\
NGC7496 & TRECS &  GS-2010B-Q-71  & 10-09-25 & Qa & 18.30 &  0.76 &      318 &  0.58 &  0.55 &       91 &  0.70 &  0.66 &      113 &    568.1 $\pm$    21.8 &    388.9 $\pm$    21.3\\
NGC7496 & TRECS &  GS-2010B-Q-71  & 10-08-20 & Si2 &  8.74 &  0.39 &      144 &  0.53 &  0.48 &      122 &  0.63 &  0.62 &       40 &     80.3 $\pm$     5.1 &     52.5 $\pm$     5.1\\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-10 & ARIII &  8.99 &  0.14 &      180 &  0.45 &  0.40 &      144 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    33.3   &  $\le$    33.3  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-23 & NEII & 12.81 &  0.21 &      507 &  0.43 &  0.41 &       30 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    68.6   &  $\le$    68.6  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-23 & NEII\_1 & 12.27 &  0.18 &      690 &  0.44 &  0.42 &       64 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    41.7   &  $\le$    41.7  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-23 & NEII\_2 & 13.04 &  0.22 &     1035 &  0.40 &  0.39 &       21 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    47.0   &  $\le$    47.0  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-10 & PAH1 &  8.59 &  0.42 &      172 &  0.47 &  0.43 &      147 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    36.4   &  $\le$    36.4  \\
NGC7552 & VISIR &  075.B-0727(A)  & 05-06-15 & PAH2 & 11.25 &  0.59 &      538 &  0.66 &  0.59 &       17 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    57.5   &  $\le$    57.5  \\
NGC7552 & VISIR &  075.B-0727(A)  & 05-06-15 & PAH2\_2 & 11.88 &  0.37 &      538 &  0.56 &  0.47 &      155 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    60.4   &  $\le$    60.4  \\
NGC7552 & VISIR &  076.B-0656(A)  & 05-10-09 & Q2 & 18.72 &  0.88 &     3638 &  0.55 &  0.52 &      119 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$   100.5   &  $\le$   100.5  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-10 & SIC & 11.85 &  2.34 &      362 &  0.49 &  0.43 &      152 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    44.3   &  $\le$    44.3  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-10 & SIV & 10.49 &  0.16 &      361 &  0.50 &  0.45 &      143 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    44.6   &  $\le$    44.6  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-23 & SIV\_1 &  9.82 &  0.18 &     2870 &  0.41 &  0.38 &      155 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    30.4   &  $\le$    30.4  \\
NGC7552 & VISIR &  075.B-0182(A)  & 05-06-23 & SIV\_2 & 10.77 &  0.19 &      349 &  0.41 &  0.39 &       41 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    38.2   &  $\le$    38.2  \\
NGC7582 & VISIR &  082.B-0299(B)  & 08-08-17 & ARIII &  8.99 &  0.14 &       60 &  0.53 &  0.47 &      117 &  0.52 &  0.48 &       70 &    254.1 $\pm$    12.1 &    246.8 $\pm$    26.4\\
NGC7582 & VISIR &  082.B-0299(B)  & 08-08-23 & ARIII &  8.99 &  0.14 &       60 &  0.30 &  0.29 &      128 &  0.40 &  0.32 &       83 &    230.5 $\pm$    23.3 &    156.4 $\pm$    17.8\\
NGC7582 & VISIR &  60.A-9246(A)  & 04-09-30 & NEII & 12.81 &  0.21 &     3591 &  0.38 &  0.36 &      127 &  0.45 &  0.39 &       94 &    610.3 $\pm$     7.5 &    470.0 $\pm$     6.8\\
NGC7582 & TRECS &  GS-2005A-Q-50  & 05-07-18 & N & 10.36 &  2.64 &       32 &  0.52 &  0.46 &       15 &  0.40 &  0.37 &       61 &    339.2 $\pm$     9.1 &    548.4 $\pm$    10.8\\
NGC7582 & VISIR &  077.B-0728(A)  & 06-08-06 & PAH2\_2 & 11.88 &  0.37 &      722 &  0.35 &  0.33 &       43 &  0.34 &  0.31 &       90 &    386.3 $\pm$     9.6 &    406.7 $\pm$    16.2\\
NGC7582 & VISIR &  082.B-0299(B)  & 08-08-18 & PAH2\_2 & 11.88 &  0.37 &       62 &  0.48 &  0.46 &       68 &  0.49 &  0.40 &       76 &    403.3 $\pm$    71.3 &    448.7 $\pm$    73.3\\
NGC7582 & VISIR &  082.B-0299(B)  & 08-08-23 & PAH2\_2 & 11.88 &  0.37 &       62 &  0.35 &  0.33 &      122 &  0.41 &  0.36 &       84 &    391.2 $\pm$    57.3 &    306.0 $\pm$    16.6\\
NGC7582 & VISIR &  077.B-0728(A)  & 06-06-16 & Q2 & 18.72 &  0.88 &     1026 &  0.48 &  0.46 &      107 &  0.56 &  0.50 &       92 &    568.5 $\pm$    47.7 &    436.8 $\pm$    35.3\\
NGC7582 & VISIR &  082.B-0299(B)  & 08-08-17 & PAH1 &  8.59 &  0.42 &       31 &  0.62 &  0.58 &      122 &  0.52 &  0.42 &       89 &    294.5 $\pm$     9.5 &    504.3 $\pm$    80.4\\
NGC7590 & VISIR &  083.B-0536(C)  & 09-06-05 & NEII\_1 & 12.27 &  0.18 &      901 &  0.36 &  0.35 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    12.0   &  $\le$    12.0  \\
NGC7590 & TRECS &  GS-2005A-Q-50  & 05-07-12 & N & 10.36 &  2.64 &       65 &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    21.2   &  $\le$    21.2  \\
NGC7590 & VISIR &  083.B-0536(C)  & 09-06-05 & PAH2 & 11.25 &  0.59 &      362 &  0.34 &  0.31 &      119 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     7.6   &  $\le$     7.6  \\
NGC7592W & TRECS &  GS-2010B-C-4  & 10-08-31 & Qa & 18.30 &  0.76 &      926 &  0.56 &  0.54 &      168 &  0.71 &  0.63 &       84 &    173.4 $\pm$    21.8 &    117.6 $\pm$    21.7\\
NGC7626 & VISIR &  083.B-0536(C)  & 09-06-05 & NEII\_1 & 12.27 &  0.18 &      721 &  0.36 &  0.35 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    17.4   &  $\le$    17.4  \\
NGC7626 & VISIR &  083.B-0536(C)  & 09-06-05 & PAH2 & 11.25 &  0.59 &      181 &  0.34 &  0.31 &      119 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    15.6   &  $\le$    15.6  \\
NGC7674 & VISIR &  077.B-0137(A)  & 06-07-13 & NEII & 12.81 &  0.21 &     1435 &  0.41 &  0.37 &       99 &  0.48 &  0.42 &      136 &    513.7 $\pm$    21.4 &    374.3 $\pm$    15.2\\
NGC7674 & TRECS &  GS-2007A-DD-7  & 07-07-01 & Qa & 18.30 &  0.76 &      847 &  0.57 &  0.53 &       70 &  0.65 &  0.57 &      131 &   1027.8 $\pm$    18.1 &    840.8 $\pm$    17.1\\
NGC7674 & VISIR &  082.B-0299(B)  & 09-07-03 & ARIII &  8.99 &  0.14 &       62 &  0.30 &  0.28 &        2 &  0.36 &  0.32 &      113 &    212.8 $\pm$    18.9 &    153.6 $\pm$     9.8\\
NGC7674 & VISIR &  082.B-0299(B)  & 09-06-12 & PAH2\_2 & 11.88 &  0.37 &      122 &  0.41 &  0.40 &      132 &  0.41 &  0.38 &      175 &    438.5 $\pm$    24.8 &    426.2 $\pm$    35.9\\
NGC7679 & VISIR &  077.B-0137(A)  & 06-07-10 & NEII\_1 & 12.27 &  0.18 &      180 &  0.34 &  0.32 &      125 &  0.46 &  0.32 &      124 &     35.9 $\pm$     9.5 &     26.9 $\pm$     9.5\\
NGC7679 & VISIR &  077.B-0137(A)  & 06-07-10 & PAH2 & 11.25 &  0.59 &      181 &  0.32 &  0.31 &      128 &  0.41 &  0.40 &      166 &     42.4 $\pm$     5.2 &     24.3 $\pm$     5.2\\
NGC7679 & VISIR &  077.B-0137(A)  & 06-07-10 & SIV & 10.49 &  0.16 &      176 &  0.32 &  0.29 &      115 &  0.31 &  0.27 &       69 &     24.9 $\pm$     5.5 &     27.6 $\pm$     5.5\\
NGC7743 & VISIR &  083.B-0536(A)  & 09-07-06 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.33 &  0.32 &      102 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.3   &  $\le$     8.3  \\
NGC7743 & VISIR &  084.B-0974(A)  & 09-10-04 & PAH1 &  8.59 &  0.42 &     1552 &  0.52 &  0.47 &       26 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.6   &  $\le$     6.6  \\
NGC7743 & VISIR &  083.B-0536(A)  & 09-07-06 & PAH2 & 11.25 &  0.59 &      362 &  0.31 &  0.29 &      117 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.5   &  $\le$     6.5  \\
NGC7743 & VISIR &  084.B-0974(A)  & 09-11-13 & SIV & 10.49 &  0.16 &     2172 &  0.36 &  0.33 &      150 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     4.7   &  $\le$     4.7  \\
PG0026+129 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     2006 &  0.59 &  0.40 &      131 &  0.55 &  0.52 &      106 &     45.3 $\pm$     6.4 &     39.2 $\pm$     6.3\\
PG0052+251 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     1203 &  0.69 &  0.42 &       98 &  0.48 &  0.38 &      129 &     29.0 $\pm$     7.7 &     40.6 $\pm$     7.8\\
PG0844+349 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &     3210 &  0.50 &  0.38 &      102 &  0.74 &  0.44 &      108 &     62.0 $\pm$     4.4 &     35.6 $\pm$     1.2\\
PG2130+099 & COMICS &  o06139  & 06-10-04 & N11.7 & 11.74 &  0.53 &      401 &  0.36 &  0.36 &      165 &  0.48 &  0.46 &      112 &    178.8 $\pm$     9.5 &    106.4 $\pm$     6.5\\
PG2130+099 & VISIR &  075.B-0844(C)  & 05-06-10 & NEII & 12.81 &  0.21 &      721 &  0.43 &  0.42 &       69 &  0.51 &  0.42 &      167 &    187.8 $\pm$     9.2 &    161.8 $\pm$     6.2\\
PG2130+099 & VISIR &  075.B-0844(C)  & 05-06-10 & PAH2 & 11.25 &  0.59 &      724 &  0.44 &  0.41 &       20 &  0.47 &  0.40 &      172 &    159.2 $\pm$     4.3 &    150.4 $\pm$     9.0\\
PG2130+099 & VISIR &  075.B-0844(C)  & 05-06-10 & SIV\_1 &  9.82 &  0.18 &      724 &  0.40 &  0.37 &       65 &  0.43 &  0.37 &      164 &    138.4 $\pm$    14.3 &    132.3 $\pm$     3.1\\
PictorA & VISIR &  084.B-0606(A)  & 09-09-30 & NEII & 12.81 &  0.21 &      358 &  0.61 &  0.51 &      134 &  0.78 &  0.63 &      123 &     84.9 $\pm$    13.2 &     54.5 $\pm$    13.1\\
PictorA & VISIR &  084.B-0606(A)  & 09-09-30 & PAH2\_2 & 11.88 &  0.37 &      180 &  0.63 &  0.52 &      128 &  0.73 &  0.55 &      108 &     80.2 $\pm$     9.9 &     64.2 $\pm$     9.9\\
PictorA & TRECS &  GS-2007A-Q-40  & 07-09-07 & Qa & 18.30 &  0.76 &      282 &  0.55 &  0.49 &       98 &  1.00 &  0.68 &      123 &    127.7 $\pm$    19.6 &     53.0 $\pm$    19.3\\
PictorA & TRECS &  GS-2007A-Q-40  & 07-02-10 & Si2 &  8.74 &  0.39 &      564 &  0.55 &  0.46 &      110 &  0.40 &  0.33 &       98 &     38.3 $\pm$     0.9 &     68.9 $\pm$     1.4\\
PictorA & TRECS &  GS-2008A-Q-58  & 08-03-04 & Si2 &  8.74 &  0.39 &     1694 &  0.47 &  0.38 &      114 &  0.49 &  0.42 &       89 &     41.2 $\pm$     2.9 &     35.1 $\pm$     5.6\\
PictorA & TRECS &  GS-2007A-Q-40  & 07-02-10 & Si6 & 12.33 &  0.59 &      564 &  0.49 &  0.42 &       58 &  0.46 &  0.40 &       91 &     77.4 $\pm$     1.2 &     89.8 $\pm$     4.2\\
PictorA & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.42 &  0.35 &       88 &  0.34 &  0.32 &       83 &     84.8 $\pm$     7.9 &    112.0 $\pm$     4.8\\
PictorA & VISIR &  084.B-0606(A)  & 09-09-30 & SIV & 10.49 &  0.16 &      176 &  0.71 &  0.63 &      138 &  0.67 &  0.58 &      174 &     80.7 $\pm$    10.8 &     91.9 $\pm$    10.8\\
PKS1417-19 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.37 &  0.30 &      111 &  0.49 &  0.42 &       97 &     25.8 $\pm$     6.1 &     15.6 $\pm$     1.2\\
PKS1814-63 & VISIR &  385.B-0981(A)  & 10-07-21 & SIC & 11.85 &  2.34 &     1794 &  0.46 &  0.41 &       44 &  0.56 &  0.44 &       25 &     23.4 $\pm$     3.9 &     18.4 $\pm$     3.5\\
PKS1932-46 & VISIR &  385.B-0981(A)  & 10-07-21 & SIC & 11.85 &  2.34 &     3588 &  0.53 &  0.49 &      103 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     8.3   &  $\le$     8.3  \\
PKS2158-380 & VISIR &  077.B-0135(A)  & 06-06-19 & SIC & 11.85 &  2.34 &     1794 &  0.42 &  0.34 &      104 &  0.43 &  0.36 &      109 &     18.6 $\pm$     2.4 &     16.8 $\pm$     2.4\\
PKS2354-35 & VISIR &  077.B-0135(A)  & 06-06-19 & SIC & 11.85 &  2.34 &     1794 &  0.35 &  0.34 &      134 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$     6.9   &  $\le$     6.9  \\
SuperantennaeS & TRECS &  GS-2004A-Q-14  & 04-07-08 & N & 10.36 &  2.64 &      716 &  0.35 &  0.35 &      111 &  0.46 &  0.45 &      143 &    110.7 $\pm$     1.9 &     64.5 $\pm$     1.7\\
SuperantennaeS & TRECS &  GS-2008B-C-2  & 08-09-11 & Qa & 18.30 &  0.76 &      926 &  0.72 &  0.64 &      179 &  0.76 &  0.68 &      176 &    594.7 $\pm$    16.0 &    524.2 $\pm$    15.3\\
SuperantennaeS & TRECS &  GS-2009B-C-3  & 09-09-08 & Qa & 18.30 &  0.76 &     1013 &  0.68 &  0.61 &      164 &  0.82 &  0.78 &      102 &    583.1 $\pm$     9.7 &    379.2 $\pm$     7.5\\
SuperantennaeS & TRECS &  GS-2009B-C-3  & 09-09-08 & Qa & 18.30 &  0.76 &     1013 &  0.71 &  0.68 &      129 &  0.67 &  0.65 &      170 &    624.4 $\pm$    11.2 &    684.2 $\pm$    11.7\\
UGC05101 & COMICS &  o09102  & 09-04-08 & N8.8 &  8.75 &  0.38 &      242 &  0.82 &  0.73 &      105 &  1.00 &  0.67 &       79 &    225.2 $\pm$    40.4 &    229.4 $\pm$    51.5\\
UGC05101 & COMICS &  o09102  & 09-04-08 & Q17.7 & 17.69 &  0.43 &      805 &  0.74 &  0.63 &       93 &  0.73 &  0.64 &       61 &    232.2 $\pm$    46.5 &    229.5 $\pm$    41.9\\
UGC12348 & TRECS &  GS-2007A-DD-7  & 07-07-01 & Qa & 18.30 &  0.76 &      282 &  0.56 &  0.51 &        8 &  0.61 &  0.53 &       70 &    170.4 $\pm$    15.0 &    150.4 $\pm$    15.0\\
UGC12348 & TRECS &  GS-2007A-DD-7  & 07-07-03 & Qa & 18.30 &  0.76 &      564 &  0.58 &  0.56 &       39 &  0.64 &  0.58 &       74 &    157.0 $\pm$    28.9 &    138.3 $\pm$    32.3\\
Z041-020 & VISIR &  084.B-0606(A)  & 10-01-27 & NEII & 12.81 &  0.21 &      540 &  0.34 &  0.33 &       30 &  $\dots$  &  $\dots$  &  $\dots$  &     29.3 $\pm$     1.6 &     29.3 $\pm$     1.6\\
Z041-020 & VISIR &  084.B-0606(A)  & 10-01-27 & PAH2\_2 & 11.88 &  0.37 &      181 &  0.32 &  0.30 &       31 &  $\dots$  &  $\dots$  &  $\dots$  &     17.4 $\pm$     1.3 &     17.4 $\pm$     1.3\\
Z041-020 & VISIR &  084.B-0606(A)  & 10-01-27 & SIV & 10.49 &  0.16 &      358 &  0.34 &  0.29 &       18 &  $\dots$  &  $\dots$  &  $\dots$  &     13.6 $\pm$     1.1 &     13.4 $\pm$     1.1\\


==> tab_obs_cut.tex <==
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & NEII\_1 & 12.27 &  0.18 &      360 &  0.38 &  0.35 &      126 &  0.36 &  0.35 &      171 &     63.2 $\pm$     5.3 &     64.9 $\pm$     3.6\\
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & NEII\_2 & 13.04 &  0.22 &      543 &  0.36 &  0.36 &      128 &  0.40 &  0.36 &       23 &     62.1 $\pm$    10.2 &     53.5 $\pm$     4.3\\
1H0419-577 & VISIR &  084.B-0606(A)  & 09-11-29 & PAH2 & 11.25 &  0.59 &      181 &  0.37 &  0.33 &      108 &  0.36 &  0.33 &       80 &     67.2 $\pm$    13.0 &     70.7 $\pm$     8.2\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-01-26 & NEII\_1 & 12.27 &  0.18 &     1442 &  0.56 &  0.48 &       95 &  0.51 &  0.41 &        2 &     39.0 $\pm$    15.1 &     53.8 $\pm$     7.2\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-03-23 & NEII\_2 & 13.04 &  0.22 &     1991 &  0.40 &  0.37 &       66 &  0.58 &  0.51 &      166 &     41.1 $\pm$     2.6 &     20.6 $\pm$     2.0\\
1RXSJ112716 & VISIR &  084.B-0606(A)  & 10-01-26 & PAH2 & 11.25 &  0.59 &      362 &  0.42 &  0.39 &       12 &  0.47 &  0.34 &      157 &     36.4 $\pm$     8.9 &     35.6 $\pm$     8.8\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_1 & 12.27 &  0.18 &      540 &  0.43 &  0.40 &       10 &  0.77 &  0.58 &      119 &     26.5 $\pm$    11.2 &     10.0 $\pm$    11.2\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & NEII\_2 & 13.04 &  0.22 &      901 &  0.41 &  0.40 &       16 &  0.71 &  0.60 &       85 &     33.6 $\pm$     7.6 &     13.0 $\pm$     7.6\\
2MASXJ0356565 & VISIR &  084.B-0606(A)  & 09-09-30 & SIV\_2 & 10.77 &  0.19 &      362 &  0.37 &  0.34 &      171 &  0.69 &  0.33 &      120 &     23.8 $\pm$     7.7 &     13.0 $\pm$     7.7\\
2MASXJ0918002 & VISIR &  084.B-0606(A)  & 10-01-05 & PAH2\_2 & 11.88 &  0.37 &     1986 &  0.34 &  0.31 &       94 &  0.42 &  0.31 &       97 &     16.6 $\pm$     0.6 &     13.4 $\pm$     0.7\\
3C029 & VISIR &  078.B-0020(A)  & 06-12-27 & SIC & 11.85 &  2.34 &     1803 &  0.41 &  0.35 &       86 &  $\dots$  &  $\dots$  &  $\dots$  &  $\le$    11.1   &  $\le$    11.1  \\
3C033 & COMICS &  o09108  & 09-07-14 & N11.7 & 11.74 &  0.53 &     3208 &  0.71 &  0.52 &       72 &  1.00 &  0.85 &      121 &     47.4 $\pm$     5.0 &     20.8 $\pm$     3.0\\

